Replicability in High Dimensional Statistics

The replicability crisis is a major issue across nearly all areas of empirical science, calling for the formal study of replicability in statistics. Motivated in this context, [Impagliazzo, Lei, Pitassi, and Sorrell STOC 2022] introduced the notion of replicable learning algorithms, and gave basic procedures for $1$-dimensional tasks including statistical queries. In this work, we study the computational and statistical cost of replicability for several fundamental high dimensional statistical tasks, including multi-hypothesis testing and mean estimation. Our main contribution establishes a computational and statistical equivalence between optimal replicable algorithms and high dimensional isoperimetric tilings. As a consequence, we obtain matching sample complexity upper and lower bounds for replicable mean estimation of distributions with bounded covariance, resolving an open problem of [Bun, Gaboardi, Hopkins, Impagliazzo, Lei, Pitassi, Sivakumar, and Sorrell, STOC2023] and for the $N$-Coin Problem, resolving a problem of [Karbasi, Velegkas, Yang, and Zhou, NeurIPS2023] up to log factors. While our equivalence is computational, allowing us to shave log factors in sample complexity from the best known efficient algorithms, efficient isoperimetric tilings are not known. To circumvent this, we introduce several relaxed paradigms that do allow for sample and computationally efficient algorithms, including allowing pre-processing, adaptivity, and approximate replicability. In these cases we give efficient algorithms matching or beating the best known sample complexity for mean estimation and the coin problem, including a generic procedure that reduces the standard quadratic overhead of replicability to linear in expectation.

==> inputs/lattice-rounding_old_.tex <==
\subsection{Replicable Learning via Isoperimetric Approximate Tiling}
\label{sec:replicability-from-isoperimetry}
% \todo{add circle simplification, reduction from DP using Stability is Stable}\maxh{Let's only do circle simplification after everything else is done. Reduction from DP maybe in related work section?}
In this subsection, we construct a replicable algorithm for mean estimation based on $(\gamma,A)$-isoperimetric approximate tilings whose sample complexity scales the surface-to-volume ratio $A$. When $A=\Theta(N)$, we will see in the following section the algorithm is information theoretically optimal.

% In this subsection, we show that information theoretically optimal high dimension replicable mean estimation can be obtained by rounding scheme based on (approximate) tilings of $\R^N$ with optimal normalized surface area $A = \Theta(N)$.
% Recall the definition of an approximate tiling. 
% \begin{definition}[$A$-Isoperimetric Tiling]
%     \label{def:approximate-isoperimetric-tiling}
%     We say a collection of sets $\mathcal V$ 
%     form an $A$-isoperimetric tiling of the space $\R^N$ if the following are satisfied:
%     \begin{enumerate}
%         \item (Partition) $\mathcal V$ forms a partition of $\R^N$.
%         \item (Bounded Size)
%         For each set $V \in \mathcal V$,
%         $\sup_{x, y \in V} \snorm{2}{x - y} \leq 1$. \snote{Do we want covering radius or just maximum distance? Maximum distance is more natural for the upper bound.}
%         \item (Isoperimetry) For any $u \in \Z^{n}$ and $C_{u} = u + [-10, 10]^{n}$,
%         \begin{equation*}
%             \vol \left( \bigcup_{V \in \mathcal V} \boundary V \cap C_{u} \right) \leq A \; 
%             \vol \lp( C_{\vec u} \rp).
%         \end{equation*}
%         % \item (Efficiency) For all $x \in \bigcup_{v \in \Z^{n}} S_{v}$, there is a polynomial time algorithm computing $v$ for which $x \in S_{v}$.
%         % \chris{do we also want to efficiently decide if $x$ is not in any part? I guess this is probably easy too.}
%     \end{enumerate}
% \end{definition}
% \ApproximateTiling*
% Our algorithm will be based on a \emph{rounding query} with respect to an isoperimetric tiling of $\R^N$.
% \begin{definition}[Tiling Rounding Query]
% Given an approximate tiling $\mathcal V$, we associate with each $V \in \mathcal V$ a canonical point $x_V \in V$.
% A rounding query 
% $\mathcal R: \R^N \mapsto \R^N$
% with respect to $\mathcal V$ does the following: given $u \in \R^N$,
% if $u \in V \in \mathcal V$, the query returns $x_V$. Otherwise, it returns an arbitrary point.
% \end{definition}
Formally, our algorithm is based on access to the membership oracle of an \iat.
For simplicity, unlike in \Cref{def:informal-tiling}, we assume that the membership oracle always returns the right answer on points within the partition.
This is without loss of generality: given a randomized membership oracle that succeeds with probability at least $2/3$, one can always query it $\Theta\lp(\log(1/\delta) \rp)$ times to boost its success probability to $1-\delta$. Since we will only call the oracle once in our algorithm, this incurs a cost of at most $\delta$ in the failure/non-replicable probability and can be safely ignored.
% In fact, we apply at most $1$ membership oracle in our learning algorithms.
% Hence, we will incur a cost of at most $\delta$ in the failure/non-replicable probability of the learning algorithm if we use a randomized membership oracle instead.}
\maxh{Remove below definition (ensure randomized version is defined in previous section).}
\begin{definition}[Deterministic Membership Oracle of Approximate Tiling] \label{def:tiling-membership-oracle}
An algorithm $\innerAlg$ is said to be a membership oracle of an approximate tiling $\{S_v\}$ of $\R^N$ 
if the following hold:
\begin{enumerate}
    \item Suppose $x \in \bigcup_{v} S_v$.
    Then $\innerAlg(x)$ returns $v$ such that $x \in S_v$.
    \item Suppose $x \not \in \bigcup_{v} S_v$. $\innerAlg(x)$ could return an arbitrary vector $u$.
\end{enumerate}
The membership oracle is said to be efficient if the algorithm runs in polynomial time in the bit-complexity of the input $x$.
\end{definition}
Given a $(\rho, A)$-\iat{} $\mathcal V$, we  design an $O(\rho)$-replicable algorithm that learns the mean of any distribution with bounded covariance in $\ell_2$ distance, and shows that the algorithm's sample complexity scales quadratically with the surface area parameter $A$ of $\mathcal V$.
At a high level, this is achieved by first computing an optimal, non-replicable $\ell_2$ mean estimator for bounded covariance distributions, and then use a randomized rounding scheme based on $\mathcal V$ to round the estimator (see \Cref{prop:replicable-rounding} and \Cref{alg:r-rounding}) to ensure replicability.
% subject to a mild smoothness condition 
% on $\mathcal V$. 
% \maxh{I think it makes more sense here to state the $\ell_\infty$-result, then give as a corollary the version for any $\ell_p$-norm. The fact that you prove the result by first doing $\ell_2$ doesn't mean we have to present it this way at the start. In the next subsection we can explain this is our approach. UPDATE: I guess doing $\ell_2$ as a corollary loses a log factor? So maybe not?}\maxh{Maybe also put the algorithm pseudocode up here and refer to it in the theorem statement?}
\begin{theorem}[From Tiling to $\ell_2$ Replicable Mean Estimation]
\label{thm:tiling-to-replicable}
Let  $\eps \in (0, \sqrt{N}]$,
$N \in \mathbb Z_+$,
$A > 0$, 
$\delta < \rho \in (0, 1)$, 
$\mathcal V$ be a $(\rho, A)$-\iat{} of $\R^N$,
% Furthermore, assume that for each $V \in \mathcal V$, the boundary $\partial V$ is piecewise-smooth.
and $\distribution$ be an $N$-dimensional distribution with covariance bounded from above by $I$.
% Let $m:= \Theta
% \lp( N^2/(\eps^2\rho^2) \rp)$, and $u$ be the sample mean computed from $m$
Given access to a membership oracle $\mathcal R$ of $\mathcal V$, there exists a $O(\rho)$-replicable algorithm (\Cref{alg:r-mean-est}) that estimates the mean of $\distribution$ up to error $\eps$ in $\ell_2$ distance with success probability $1 - \delta$.
Moreover, the algorithm 
uses $m:=\bigO{\lp( N + \log(1/\delta) \rp) A^2 N^{-1} \eps^{-2} \rho^{-2}}$ vector samples,\footnote{Note that $A \geq \Omega(N)$ even for optimal tilings, so this does not violate the standard $\Omega(N \eps^{-2})$ lower bound for (non-replicable) mean estimation.}
% It is known that estimating up to $\eps$ $\ell_2$ distance requires at least $\Omega(N \eps^{-2})$ many samples. This term is dominated by $\Theta(A^2\eps^{-2})$ since the optimal isoperimetric tiling has surface area to volume ratio at least $A = \Omega(N)$.}. 
% Hence, the second term in the sample complexity is really a lower order term, 
uses $1$ deterministic membership query, and runs in time $\poly{N m}$.
\end{theorem}
% \maxh{Is it much more work to get the right dependence on $\rho$ and/or $\delta$?}
% We briefly discuss the sample complexity upper bound achieved by the above theorem.
% Recall that the optimal non-replicable mean estimation algorithm uses $\Theta(N \eps^{-2})$ many samples. The above theorem says that the replicable algorithm based on an $A$-isoperimetric Tiling needs to pay an extra multiplicative cost of $A / \rho^{-2}$ in its sample complexity. 
We remark that there are known constructions, i.e., ``randomized foams'' from \cite{kindler2012spherical}, that give isoperimetric tilings of $\R^N$ with surface-area to volume ratio $O(N)$.
Combining the construction with \Cref{thm:tiling-to-replicable} then
immediately gives a replicable algorithm with an optimal \snew{(vector)} sample complexity of $\Theta \lp( N^2 \rho^{-2} \eps^{-2}  \rp)$ (assuming $N \gg \log(1/\delta)$).
% \chris{I guess we are working with vector samples now? Think this should be clarified but maybe makes more sense to talk about vector samples in the lower bound than it does to talk about coordinate samples in the upper bound}
Unfortunately membership queries in such constructions take exponential time, so computational efficiency is lost in this process. 
In the next section, we will discuss other isoperimetrically optimal candidates for sample-optimal mean estimation based on lattices. 
Compared to randomized foams, these constructions have the advantage of having computationally efficient rounding schemes after an initial pre-processing stage, and seem to have greater potential to give a truly computationally efficient sample-optimal algorithm.

% For non-replicable mean estimation, a common algorithm (computing the sample mean) can be used to optimally learn the mean of an unknown distribution under both $\ell_2$ and $\ell_\infty$ distance.
% This is perhaps less obvious for replicable mean estimation. 
We also provide a similar algorithm (\Cref{alg:r-mean-est-infty}) that replicably learns the mean in $\ell_\infty$ distance.
Note that the $N$-coin distribution indeed has its covariance bounded from above by $I$.
Hence, \Cref{alg:r-mean-est-infty} can be used to solve the $N$-coin problem with the same sample complexity (see \Cref{cor:spherical-foam-l-inf-mean}).
% Combining it with \Cref{lemma:l-inf-tester-implies-learner} then gives a replicable algorithm for multihypothesis testing as well. 

Glossing over some detail, we show that one can learn the mean up to $\gamma$ error in $\ell_\infty$ distance if one simply uses (almost) the same algorithm 
from \Cref{thm:tiling-to-replicable} to learn the mean up to $\eps := \tilde \Theta \lp( \sqrt{N} \gamma \rp)$ error in $\ell_2$ distance, and observes that the rounding error will be roughly in a uniform direction.
This gives the following upper bound on replicably learning in $\ell_\infty$ distance.
\begin{theorem}[$\ell_\infty$ Replicable Mean Estimation]
\label{thm:ell-infty-mean}
Under the same setup as \Cref{thm:tiling-to-replicable},
if the objective is to estimate up to $\gamma$ error in $\ell_\infty$ distance for some $\gamma \in (0, 1)$, 
then there exists a $O(\rho)$-replicable mean estimation algorithm (\Cref{alg:r-mean-est-infty}) 
that succeeds with probability at least $1 - \delta$.
Moreover, the algorithm uses $m := \Theta \lp( A^2 N^{-1} \gamma^{-2} \rho^{-2} \log^3(N/\delta) \rp)$ vector samples, uses $1$ deterministic membership query, and runs in time $\poly{N m}$.
\end{theorem}
Similar to \Cref{thm:tiling-to-replicable}, \Cref{thm:ell-infty-mean} combined with an  isoperimetric tiling with optimal surface-area to volume ratio yields a replicable $\ell_\infty$ mean estimation algorithm that has a (nearly) optimal sample complexity of $ \Theta\lp(  N \gamma^{-2}  \rho^{-2} \log^3(N/\delta) \rp)$.

\subsubsection{Rounding Scheme from Isoperimetric Tiling}
The core of our mean estimation algorithms is a method of building a replicable rounding scheme from any isoperimetric approximate tiling, that is a scheme such that run on two nearby inputs with \emph{shared randomness}, the outputs will with high probability 1) be the same, and 2) be close to their original inputs. Such schemes are also sometimes called ``noise resistant'' or ``coordinated discretization schemes''. \cite{kindler2012spherical}.

\maxh{The $\delta$ dependence here is somewhat strange. Is there a reason we don't just always round successfully by returning $u$ if $||\bar{u}-u||>\varepsilon$...?}
\begin{proposition}[Replicable Rounding Scheme]
\label{prop:replicable-rounding}
Let $\rho \in (0, 1)$ and $A >0$.
Let $\mathcal V$ be a $(\rho,A)$-isoperimetric approximate tiling of $\R^N$, and $\mathcal R: \R^N \mapsto \R^N$ its membership oracle.
% Let $u^{(1)}, u^{(2)} \in  [-N, N]^N$ such that $\snorm{2}{ u^{(1)} - u^{(2)} } \leq c \frac{ \sqrt{N} \eps \rho }{A}$ for some sufficiently small constant $c$.
Given access to $\mathcal R$, there exists an algorithm 
\alg{rPartialTilingRounding} that takes input 
$u \in [-N, N]^N$,
$\eps \in (0, \sqrt{N})$, $\delta < \rho \in (0, 1)$, and outputs a rounded vector $\bar u \in \R^N$
such that the following hold:
\begin{itemize}
\item \textbf{Bounded Rounding Error:} We have that $\snorm{2}{ \bar u - u } \leq \epsilon $ with probability at least $1 - \delta$.
\item \textbf{Replicability:}
% \footnote{
% When discussing the randomized rounding scheme, 
% we abuse the terminology replicability here slightly, and use it to refer to the property that the algorithm gives the same output with high probability for inputs with sufficiently small distance.}
Let $\bar u^{(i)} = \alg{rPartialTilingRounding}( u^{(i)}, \eps, \delta, \rho )$ for $i \in \{1, 2\}$ with shared internal randomness.
Assume that $\snorm{2}{ u^{(1)} - u^{(2)} } \leq c \frac{\sqrt{N} \eps \rho}{A}$ for some sufficiently small constant $c$.  Then it holds
$ \bar u^{(1)} = \bar u^{(2)} $ with probability at least $1 - \rho$.
\end{itemize}
\end{proposition}
It is not hard to imagine \Cref{thm:tiling-to-replicable} and \Cref{thm:ell-infty-mean} follow from combining such a scheme with a non-replicable estimator, since rounding the output of the latter over two independent samples (with shared randomness) then results in the same solution with high probability. Of course some further detail is required, which we defer to the following subsections.


% Our overall approach is to round a non-replicable mean estimator according to a tiling $\mathcal V$ with optimal surface-to-volume ratio (see \Cref{def:approximate-tiling}).
% As pointed out in \cite{impagliazzo2022reproducibility}, no deterministic algorithm is adversarially replicable, and hence we should not expect \emph{any deterministic rounding procedure to work}.
% Our main technical contribution in this subsection is a randomized rounding scheme based on an isoperimetric tiling that can could render any mean estimator that has good $\ell_2$ accuracy into a replicable one.
% In particular, if one runs the randomized routine twice on two inputs that are close to each other in $\ell_2$ distance with \emph{shared randomness}, the outputs will be the same, and also close to their inputs in $\ell_2$ distance with high probability. 

We first overview the steps of our rounding scheme. Naively, one might hope to simply round using the membership oracle of $\mathcal{V}$ itself, but as was observed by \cite{impagliazzo2022reproducibility} in the 1-D case, deterministic procedures of this sort always fail replicability in the worst-case. Namely no matter how close two inputs might be, if they cross the boundary of the partition, they will round to different outputs.
To avoid such worst case scenarios, we will apply a random shift $b \sim \Uni([-\BX, \BX]^N)$ to $u$ before we apply the rounding procedure for some $Q$ that is sufficiently large in $N, \epsilon, \delta^{-1}$.
For technical reasons, the proceeding analysis will be easier if the post-shift point has a uniformly random distribution over a fixed cube $\Uni([-\BX, \BX]^N)$ for any input $u \in [-N, N]$. 
Thus, we will also apply a ``wrap around'' after shifting:
\begin{align}
\label{eq:wrap-def}
    \text{Wrap}(x)_i =  \lp( (x_i + \BX)  \mod 2\BX \rp) - \BX. 
\end{align}
% \chris{parentheses around the mod?}。
This ensures that the distribution over the post-shifted point will be uniform over the cube. As a result, no matter where the original input vector lies, after translating and wrapping the probability the point lies near the boundary of our tiling is proportional to the boundary's surface area.

% the post-shift point will be close to the boundary of the tiling with probability proportional to the boundary surface area, helping us avoid the worst case locations of $u^{(1)}$ and $u^{(2)}$.

Given only the above strategy, if two input vectors $u^{(1)}, u^{(2)}$ are $\eta$-close, to ensure replicability we need our wrapped translation procedure to send $u^{(1)}$ $\eta$-far away from the boundary since $u^{(2)}-u^{(1)}$ might point directly towards the boundary and cross otherwise. This turns out to be too expensive, and can be avoided by first \textit{rotating} the vectors, ensuring this difference lies in a random instead of worst-case direction.

% Naively, if we have that the input vectors $u^{(1)}, u^{(2)}$ are $\eta$-close to the boundary with probability $\rho$, one will think that we would need $\snorm{2}{ u^{(1)} - u^{(2)} } \leq \eta$ to guarantee that their rounding results are the same.
% However, we note that this will be the case only if the difference vector $u^{(2)} - u^{(1)}$ happens to be pointing towards the closest boundary point from $u^{(1)}$, which is the \emph{the worst direction}.
% Though the random shift successfully helps us avoid the worst-case scenario, it will not directly give us the optimal sample complexity.
% To see this, we note that with probability about $\rho$, the distribution mean after the random shift can still be $\rho / A$ close to the boundary. In the worst case, the error vector between the estimator and the distribution mean may be pointing right towards the closest point (from the distribution mean) on the boundary. 
% If that happens, we will need to take $N A^2 / \rho^2$ many samples to ensure that the error vector is small enough such that it will not cross the tiling boundary.
% \chris{maybe explain where the extra $N$ comes from? I assume this is the $d$ from CFB19 but might be nice to state explicitly since from median-of-means it would just be $\frac{A^2}{\rho^2}$ and Theorem 5.3 seems to only have constant $\rho, \delta$ right now.}
% This makes us still a factor of $N$ from the sample complexity bound in \Cref{thm:tiling-to-replicable}.
% Hence, further improvements can be made if we can make the difference vector point towards a \emph{uniformly random direction}.
% % This is easy if we use sample mean as our estimator and the target distribution is centrally symmetric, but not so obvious when we use the more involved estimator from \Cref{thm:sub-gaussian-mean} on distribution with merely bounded covariance. 
% Fortunately, applying a random rotation on the input does the job.
% However, we note that the random direction property can be easily ensured if we also apply a random rotation on the estimator.

Altogether, this leads to the following random transformation on the estimator $u$ before applying the membership query.
\begin{align*}
   v := \text{Wrap} \lp(  R u + b \rp) \, ,
\end{align*}
where $R \sim \Uni( \SO(N) )$, 
% \chris{remember to define this in prelims}
and $b \sim \Uni( [-\BX, \BX]^N )$.
% We note that the transformation is invertible.
% Thus, after the rounding query, we can simply apply the inverse transformation to obtain our final output.


% Specifically, with our rounding approach, 
% To circumvent the issue, we need to randomize our rounding scheme. 
% We do so by applying a random transformation on the \snew{mean estimator obtained from \Cref{thm:sub-gaussian-mean}.}
% In particular, we will (i) apply a random rotation $R \in \SO(N)$ \maxh{Shouldn't this be $SO(n)$, not $O(n)$?}
% on the sample mean learned, (ii) add a uniform random shift $b \sim \Uni\lp( [-N^2, N^2]^N\rp)$, and then (iii) ``wrap around'' the cube $ [-N^2, N^2]^N$. 
% Specifically, we define the \emph{Wrap} function:
% \begin{align}
% \label{eq:wrap-def}
%     \text{Wrap}(x)_i =  (x_i + N^2)  \mod 2N^2 - N^2.
% \end{align}
% \maxh{This seems a bit strange when we're over $N^2$? Also mod $2N-N$? are there supposed to be parentheses here somewhere?}
The above addresses only replicability of the rounding scheme. Ensuring that we have small rounding error (i.e., the rounding output is close to the input) requires some extra care. First, since we are working with a tiling with constant radius, naively applying the membership oracle leads to constant error. To achieve any error $\varepsilon$, we may simply `scale' the tiling by outputting $\tilde v = \eps \mathcal R(\eps^{-1}v )$ on input $v$ to the membership oracle $\mathcal R$. Finally, to ensure our output is actually near the original point, we need to `invert' our rotation and translation procedure.
% In particular, if we round a point $v$ according to the tiling $\mathcal V$, the resulting point $\tilde v$ may be in the worst case at a distance $\Theta(1)$ from $x$.
% To make sure in the end we have accuracy $\epsilon$, we will round based on a scaled version of the tiling. 
% In particular, 
% Given the rounding query $\mathcal R$ and a point $v$, we round it by computing $\tilde v = \eps \mathcal R(\eps^{-1}v )$.
% % This ensures the rounding error will be properly scaled to $\eps$ as well.
% Lastly, recall that we have applied a random transformation on the input before applying the rounding query. Thus, as our last step, we need to invert the transformation. 
The final output will therefore be given by 
$ \bar u = R^{-1} \text{Wrap}\lp( \tilde v - b\rp) $.
This ensures the output $\bar u$ will be close to the original input $u$ rather than the transformed input $v$. 
% Finally we scale the result of this procedure by $\varepsilon^{-1}$, round the resulting vector to its canonical point in the partition, then reverse the transformation to get the output. The scaling ensures our rounding only incurs $\varepsilon$ error in the resulting mean. 
The pseudocode is given in \Cref{alg:r-mean-est}.

In the remaining of the subsection, we provide the proof of \Cref{prop:replicable-rounding}.
We reiterate the notations that will be used throughout the analysis.
Let $u^{(1)}, u^{(2)}$ be the input vectors given in two different runs of the algorithm, $v^{(1)}, v^{(2)}$ be the randomly transformed points $v^{(i)} = \text{Wrap} \lp( R u^{(i)} + b \rp) $, $\tilde v^{(1)}, \tilde v^{(2)}$ be the rounded points, i.e., $\tilde v^{(i)} = \eps\mathcal R(\eps^{-1}v^{(i)} )$, and $\bar u^{(1)}, \bar u^{(2)}$ be the final outputs, i.e.,
$\bar u^{(i)} = R^{-1}\text{Wrap} \lp( \tilde v^{(i)} - b \rp)$. 

% \maxh{Maybe it makes sense to include $\varepsilon$ as part of the transformation, rather than as part of the rounding?}
% \sihan{I make it part of rounding cuz I want to separate the random part and the deterministic part.}

Since the randomness of $R \in \SO(N)$ and $b\in [-\BX,\BX]^N$ is shared across the two runs of the algorithm, the outcomes are identical as long as $\eps^{-1} v^{(1)}, \eps^{-1} v^{(2)}$ lie in some common set $V \in \mathcal V$ within the tiling (implying that they will be rounded to the same point).
Our main task is to bound this probability by the surface-area parameter $A$ of the tiling.
% Equivalently, replicability is ensured if the segment $\seg\lp( v^{(1)}, v^{(2)}\rp)$ does not intersect with any facet of any Voronoi cell of the lattice.
% Therefore, we proceed to bound from the above the probability that this happens.


\IncMargin{1em}
\begin{algorithm}

\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}\SetKwInOut{Parameters}{Parameters}
\Input{Input vector $u \in [-N, N]^N$, membership oracle $\mathcal R: \R^N \mapsto \R^N$ of a $(\rho,A)$-approximate isoperimetric tiling $\mathcal V$.}
\Parameters{Rounding error parameter $\eps \in (0, \sqrt{N})$, fail probability $\delta \in (0, 1)$, replicability parameter $\rho \in (0, 1)$.}
\Output{
$\bar \mu \in \R^N$.}
\begin{algorithmic}[1]
% \State Set $\BX = C \; \lp( N \eps \delta^{-1} + \sqrt{N} (\BD + \eps) \rp)$, for some sufficiently large constant $C$.
% \State 
% Set $m_1:=C  \log(N/\delta) \rho^{-2}$ and $m_2 := 
% C \; \lp( N + \log(1/\delta) \rp) A^2 N^{-1} \eps^{-2} \rho^{-2}$.
% for some sufficiently large constant $C$.
% \State Use \Cref{lem:warmup-round} to replicably learn $\tilde u$
% with $m_1$ samples such that $\snorm{\infty}{ \tilde u - \Ep[D]} \leq N$ in $\ell_\infty$ distance.\label{line:warmup1}

% % \State Transform the coordinate system by $\tilde \mu$. \label{line:warmup2}
% \State Compute the \snew{estimator $u$ with the algorithm from \Cref{thm:sub-gaussian-mean}} 
% \If{Norm is $\ell_2$}
% with $m_2$ many samples.
% \ElseIf{Norm is $\ell_\infty$}
% \State Compute the \snew{median-of-mean estimator $u$ (\Cref{clm:median-of-mean})} with $m_3$ many samples.
% \EndIf



\State 
\snew{Set $\BX := C\lp( N^{3/2} + 
N \varepsilon \delta^{-1}
\rp)$ for some sufficiently large constant $C$.}

\State Sample $R \sim \Uni( \SO(N) )$, $b \sim\Uni\lp(   [-\BX, \BX]^N \rp)$.

\State Apply the random transformation: $v = \text{Wrap} \lp( R u + b \rp)$.

\State Apply the scaled membership query: $\tilde v = \eps \mathcal R \lp( 
 \eps^{-1} v \rp)$.


\State Invert the transformation: $\bar u = R^{-1} \text{Wrap} \lp( \tilde v - b \rp)$.

\State \Return $\bar u$ if $\snorm{2}{ \tilde v - v } \leq \eps$ 
and $u$ otherwise.


\caption{Replicable Tiling Rounding} 
\label{alg:r-rounding}

\end{algorithmic}
\end{algorithm}
\DecMargin{1em}
\maxh{Why don't we return $u$ if $||\bar{u}-u||_2 \geq \varepsilon$?}
% Let $u^{(1)}, u^{(2)}$ be the sample means estimated in two different runs of the algorithm. 
% We will denote by $q^{(1)}, q^{(2)} \in [-N, N]^N$ the points obtained after step (i) of the random transformation, and $v^{(1)}, v^{(2)} \in [-N, N]^N$ the points after step (ii).
If one think of the segments $\seg\lp( u^{(1)}, u^{(2)} \rp)$ as  a ``needle'',
at a high level, applying the random rotation $R$ ensures that the needle will be pointing towards a random direction, and adding the random offset $b$ ensures that the needle will appear at any place of the cube $ [-\BX, \BX]^N$ uniformly at random.
A caveat is that the needle may cross the boundary of the cube after the random shift, and hence 
be  ``wrapped around'' the cube. 
A convenient way of thinking of the ``wrap around'' effect is to view the process as taking place on the torus $\mathbb T^N := \R^N / \mathbb Z^N$ after scaling and translating the space appropriately. 
% \chris{$N$ not $d$?}. 
This gives the following equivalent stochastic process (up to proper scaling and translation) described via a random Buffon needle in $\mathbb T^d$.
\begin{definition}[Random Buffon Needle in $\mathbb T^N$]
Let $\eps \in [0, 1/3)$.
Let $x$ be a uniformly random point from $\mathbb T^N$,  $u$ a uniformly random unit vector, and $y = x + \eps u   \in \mathbb T^N$.\footnote{We assume by default the addition and multiplication on elements from $\mathbb T^N$ are the ``wrapped around'' operations, i.e., $ a + b = (a+b) \mod 1$ and $a b = (a b) \mod 1$.}
% Return the pair $ 
% \lp( N \lp( 2 x - \mathbf 1\rp),
% N \lp( 2 y - \mathbf 1 \rp) \rp) \subset [-N,N]^N$.
Given $x, y \in \mathbb T^N$, we define the torus segment as
$\ell_{\mathbb T}(x, y):= \{
x + t (y-x)  \in \mathbb T^N, \, \text{ where } 0 \leq t \leq 1
\}$.
We define the $\eps$-Buffon needle distribution to be the distribution over torus segments $\ell_{\mathbb T}(x, y)$.
\end{definition}
% \maxh{$1_N \to \frac{1_N}{2}$ throughout?} 
% \chris{feel like the $N$ is unnecessary and would look better without, but up to you}
% At a high level, step (i) ensures that $q^{(2)} - q^{(1)}$ will
% The key property of the random transformation is that it ensures that the marginal distributions of $v^{(1)}, v^{(2)}$ will be uniform over the cube $[-N, N]^N$, and that the vector $v^{(2)} - v^{(1)}$ will be pointing towards a random direction in most of time.
% We formalize the two properties below.
\begin{lemma}
\label{lem:Buffon-equivalence}
Let $u^{(1)}, u^{(2)} \in [-N, N]^N$,   
$R \sim \Uni(\SO(N))$, $b \in \Uni(  [-\BX, \BX]^N )$ for some $\BX \gg N^{3/2}$,  and $v^{(1)}, v^{(2)}$ be such that
$v^{(i)} = \text{Wrap}\lp( R u^{(i)} + b  \rp)$.
Then the distribution of
$$
\ell_{\mathbb T}\lp( 
\frac{v^{(1)}}{2\BX} + \mathbf 1_N/2
, \frac{v^{(2)}}{2\BX} + \mathbf 1_N/2 \rp)
$$ 
is identical to the $\eps$-Buffon needle distribution, where $\eps:=\snorm{2}{ u^{(2)} - u^{(1)} } / (2N^2)$.
\end{lemma}
\begin{proof}
It suffices to argue that (a) $R (u^{(1)} - u^{(2)})$ points towards a uniformly random direction, and
(b) $v^{(1)}$ is uniform over the cube $[-\BX, \BX]^{2N}$ conditioned on any $R$. \maxh{$2N$? And why is $\varepsilon$ normalized by $2N^2$? Is it not just normalized by $2Q$?}

Since $u^{(i)} \in [-N, N]^N$, it follows that $R u^{(i)} \in [-N^{3/2}, N^{3/2}]^N$.
Claim (b) then follows from the observation that for any interval $[a,b]$ and $y \sim [0,b-a]$ uniformly, if $x \in [a,b]$ is any arbitrary point then $x + y$ wrapped around $[a,b]$ is uniform. Applying this to each coordinate of $v^{(i)}$ then implies the desired uniformity. 
Claim (a) follows from the fact that $R \sim \SO(N)$ uniformly at random.
\end{proof}

With the equivalence of the two stochastic processes in mind, we can bound the probability two close transformed points cross the boundary of our partition (i.e.\ fail replicability) by a classical result in geometry known as Buffon's needle theorem \cite{santalo2004integral}.
% Buffon's needle theorem
% then apply the following classical result in geometry \cite{santalo2004integral} bounding the expected number of intersections of a random needle from $\mathbb T^N$ with any piece-wise smooth surface within it.
\begin{lemma}[Buffon's Needle Theorem (as stated in \cite{kindler2012spherical})]
\label{lem:expected-torus-surface-intersection}
Let $S$ be a piecewise smooth surface in the torus $\mathbb T^N$.
Let $x,y$ be a pair of random points such that 
the torus segment $\ell_{\mathbb T}(x, y)$ follows the $\eps$-Buffon needle distribution. 
Let $\kappa$ denotes the number of times the torus segment $\ell_{\mathbb T}(x, y)$ intersects with the surface $S$.
Then it holds that
$$
\Ep_{ \ell_{\mathbb T}(x, y) }\lp[ \kappa \rp] \leq 
O \lp( \frac{1}{ \sqrt{N} } \rp) \; \eps \; \area(S).
$$
\end{lemma}

% The proof of \Cref{thm:tiling-to-replicable} follows from \Cref{lem:Buffon-equivalence,lem:expected-torus-surface-intersection}.
% \begin{lemma}
% Let $\mathcal F$ be the collection of all facets of the Voronoi cells of the lattice.
% $$
% \Pr\lp[ 
% \seg\lp( v^{(1)}, v^{(2)}\rp) \cap  
% \bigcup_{F \in \mathcal F} F
% \rp] \leq \rho.
% $$
% \end{lemma}
We are now ready to give the formal proof of \Cref{prop:replicable-rounding}.
\begin{proof}[Proof of \Cref{prop:replicable-rounding}]
% We start with a preliminary simplification that allows us to reduce to the case $\eps = 1$.
% Instead of drawing samples from the unknown distribution $D$ directly, we replace each sample with an average sample $\bar x = 
% \eps^{-1}
% \frac{1}{\ell} \sum_{i=1}^{\ell} x^{(i)} $, where $\ell = \ceil{ 10/\eps^2 }$, $x^{(1)}, \cdots x^{(\ell)}$ are \iid samples from $D$.
% Then $\bar x$ can be viewed as an \iid sample from the distribution $D'$ with mean $ 10 \eps^{-1} \E[D] $ and covariance bounded from above by $I$.
% Suppose we have a 
% $0.1$-replicable mean estimation algorithm that estimates the mean of $D'$ up to accuracy $1$ (in $\ell_2$ or $\ell_\infty$ distance). 
% Then we can simply multiply the output by $\eps/10$ to obtain a replicable estimation of $D$ up to accuracy $\eps$ (in $\ell_2$ or $\ell_\infty$ distance).
% Thus, in the rest of the proof, we assume without loss of generality that $\eps = 1$.



% \maxh{What step is this? I thought we used median of means? And don't we use $A^2\eps^{-2}$ samples in this step (even if not needed for the analysis)?}. 
We bound the rounding error and the replicability parameter of the algorithm separately.
\paragraph{Rounding Error}
Recall our algorithm first applies a random transformation on the input and wraps it around the cube $ [-\BX, \BX]^N$, where $\BX := C \lp(  N^{3/2} + N \eps \delta^{-1} \rp)$ for some sufficiently large constant $C$.
In particular, let $v = \text{Wrap}\lp( R u + b \rp)$, where $R \sim \Uni( \SO(N) )$, $b \in \Uni\lp( [-\BX , \BX]^{N} \rp)$, and $\text{Wrap}: \R^N \mapsto  [-\BX, \BX]^N$ is as in \Cref{eq:wrap-def}.
The algorithm then applies the scaled membership oracle, which gives $\tilde v = \eps \mathcal R( \eps^{-1} v)$, where $\mathcal R$ is the rounding query with respect to the tiling $\mathcal V$.
If $\snorm{2}{ v - \tilde v } > \varepsilon$, the algorithm outputs $\bar u = u$ directly, which has rounding error $0$.
Otherwise, 
the final output of the algorithm is $ \bar u = R^{-1} \text{Wrap}\lp(  \tilde v - b \rp) $ if $\snorm{2}{ \tilde v - v } \leq \epsilon$. 
% By the triangle inequality and \Cref{eq:sub-gaussian-mean} it is enough 
% Conditioned on $\snorm{2}{ v - \tilde v } \leq \epsilon$, 
Our goal is to show that
\begin{align}\label{eq:part-to-rep-correct}
|| \bar u - u ||_2 \leq \varepsilon
\end{align}
with probability at least $1 - O(\delta)$.

We will show this in two steps. 
First, we claim that the final transformation 
$f(x) = R^{-1} \text{Wrap}( x - b )$ inverts the random transformation $g(x) = \text{Wrap}(Rx +b)$.
\begin{claim}\label{claim:no-wrapping}
% With probability at least $1 - \delta$ over the choice of $u,v$:
It holds that
$
R^{-1}\text{Wrap}(v-b) = u.
$
\end{claim}
Second, we argue that the (scaled) rounding procedure, that maps $v$ to $\tilde{v}$, introduces at most $\varepsilon$ error even after the inversion.
\begin{claim}\label{claim:rounding-error}
If $\snorm{2}{ v - \tilde v } \leq \epsilon$ and $v$ is $\epsilon$-far from the boundary of the cube $[-\BX, \BX]^N$,
% With probability at least $1 - \delta$ over the choice of $u,v$:
it holds that
\begin{align*}
\snorm{2}{ R^{-1}\text{Wrap}\lp( \tilde v - b \rp) 
-R^{-1}\text{Wrap}\lp( v - b \rp)
}\leq \varepsilon.
\end{align*}
\end{claim}
Consider the events
$\mathcal B: v$ is $\epsilon$-far to the boundary of the cube $[-\BX ,\BX]^N$, and $\mathcal E: \snorm{2}{v - \tilde v} \leq \eps$.
Under $\mathcal B \land \mathcal E$, we can apply \Cref{claim:rounding-error} and \Cref{claim:no-wrapping} to derive \Cref{eq:part-to-rep-correct}. In particular,
\begin{align*}
|| \bar u - u ||_2
&=
\| R^{-1} \text{Wrap}\lp( \tilde v - b \rp) - u \|_2 \\
&=
\| R^{-1} \text{Wrap}\lp( \tilde v - b \rp) -  R^{-1} \text{Wrap}\lp( v - b \rp) \|_2 \\
&\leq \eps,
\end{align*}
where the first equality is true since the algorithm outputs $\bar u = R^{-1} \text{Wrap}\lp( \tilde v - b \rp)$ when $\snorm{2}{v - \tilde v} \leq \eps$, 
the second equality uses \Cref{claim:no-wrapping}, and the last inequality uses \Cref{claim:rounding-error}.
Under the event $\mathcal B \land (\neg \mathcal E)$, \Cref{eq:part-to-rep-correct} is trivially true since we output $\bar u = u$ under $\neg \mathcal E$.
Hence, the only case where \Cref{eq:part-to-rep-correct} does not hold is $\neg \mathcal B$.
Using the fact that $v$ is uniform over $[-\BX, \BX]^N$ (\Cref{lem:Buffon-equivalence}), we have that $\mathcal B$ fails to hold with probability at most $ N \epsilon / Q \ll \delta $ by our choice of $Q$.

It is left to prove the claims. Toward \Cref{claim:no-wrapping}, recall $u \in [-N, N]^N$ by assumption, so $R u \in [-N^{3/2}, N^{3/2}]^N \subset [-\BX, \BX]^N$ and we have
 $$
 \text{Wrap} \lp( \text{Wrap} \lp( Ru + b \rp) - b \rp) = Ru.
 $$
 Combining this with the definition $v =  \text{Wrap}\lp( R u + b\rp)$ implies
\begin{align}
\label{eq:inverse-wrap}
u = R^{-1} \text{Wrap} \lp( \text{Wrap} \lp( Ru + b \rp) - b \rp)
=  R^{-1} \text{Wrap}\lp( v - b \rp).
\end{align}
as desired. Toward \Cref{claim:rounding-error}, 
% observe that since each set $V \in \mathcal V$ has bounded maximum distance by assumption, 
% \snew{since we are in the case that the algorithm outputs $u$ directly}, we should have that
% % $\snorm{2}{ \eps^{-1} \tilde v - \eps^{-1} v } \leq 1$, which in turn implies that
% \begin{align}
% \label{eq:rounding-err}
%     \snorm{2}{\tilde v - v } \leq \eps.
% \end{align}
we claim that  
\begin{align}
\label{eq:wrap-preserve-distance}    
\snorm{2}{ \text{Wrap}\lp( \tilde v - b \rp) 
-\text{Wrap}\lp( v - b \rp)
} = \snorm{2}{ \tilde v - v }
\end{align}
when $v$ is $\eps$-far from the boundary of the cube $[-\BX, \BX]^N$.
Since $R^{-1}$ is a rotation it preserves $\ell_2$-norm, so \Cref{claim:rounding-error} immediately follows from \Cref{eq:wrap-preserve-distance}.

The only obstruction to \Cref{eq:wrap-preserve-distance} is if exactly one of $\tilde v$ and $v$ `wraps' around the cube when shifted by $b$. Note this cannot occur if both $v$ and $\text{Wrap}(v-b)$ are at least $\eps$-far from the boundaries of the cube $ [-\BX, \BX]^N$. In this case the function $f(x) = \text{Wrap}(x - b)$ maps the $\eps$-ball around $v$ to the $\eps$-ball around $\text{Wrap}\lp( v - b \rp)$. 
Since $\tilde{v}$ is promised to lie in the former, $\text{Wrap}\lp( \tilde v - b \rp)$ therefore lies in the latter as desired and in particular has the same $\ell_2$ distance to $\text{Wrap}\lp( v - b \rp)$ as that between $\tilde v$ and $v$.

It remains to show that $\text{Wrap}(v-b)$  and $v$ are both at least $\eps$-far from the boundaries with probability at least $1 - \delta$.
% \chris{always? under assumption of $\varepsilon$-far?}.
The latter is $\eps$-far from the boundaries by the assuption of \Cref{claim:rounding-error}.
By \Cref{claim:no-wrapping}, the former is exactly $R u$, and hence lies in the cube $[-N^{3/2}, N^{3/2}]^N$.
It follows that the former is also $\eps$-far from the boundaries of the cube $[-\BX, \BX]^N$ as $\BX \gg N^{3/2}$ and $\epsilon <\sqrt{N}$.
This completes the proof of \Cref{eq:wrap-preserve-distance} and therefore \Cref{claim:rounding-error} as desired.
% Hence, this completes the upper bound on the rounding error.
% Specifically, note that $R u \in  [-N^2, N^2]^N$ conditioned on \Cref{eq:sub-gaussian-mean} and the success of the warmup rounding procedure. 


% \chris{spell out \Cref{eq:inverse-wrap} a bit more?}
% Combining \Cref{eq:inverse-wrap} and \Cref{eq:u-norm-bound} then gives that
% \[
% \snorm{\infty}{ \text{Wrap}\lp( v - b \rp) }
% = \snorm{\infty}{ R u }
% \leq \sqrt{N} ( N + \eps)
% \]
% so $\text{Wrap}\lp( v - b \rp)$ is indeed at least $\eps$-far from the boundary of the cube $[-\BX, \BX]^{N}$
% as we choose $\BX  \gg  \sqrt{N} (N + \eps)$.


% We now turn our attention to $v$. By \Cref{lem:Buffon-equivalence}, the distribution of $v$ is uniform over the cube $[-\BX, \BX]^{N}$. Hence, it follows that $v$ is $\eps$-close to any of the boundary of the cube with probability at most $  O \lp( N \; \eps / \BX \rp) \ll \delta$ since $\eps = O(\sqrt{N})$ by assumption, and we choose 
% $\BX \gg N \; \eps \delta^{-1}$,
% which completes the proof.



% To conclude the correctness proof, we note that
% \begin{align}
% \label{eq:rounding-error}
% \snorm{2}{ R^{-1} \text{Wrap} \lp(\tilde v - b\rp)  -  u
% }
% =
% \snorm{2}{ R^{-1}\lp(\tilde v - b\rp) 
% -  R^{-1} \text{Wrap} \lp(v - b\rp)
% }
% = \snorm{2}{ \tilde v - v } \leq \eps \, ,
% \end{align}
% where the first equality again follows from \Cref{eq:inverse-wrap}, the second equality uses \Cref{eq:wrap-preserve-distance} and the fact that $R$ preserves $\ell_2$ distance between vectors, and the third inequality uses \Cref{eq:rounding-err}.
% Combining \Cref{eq:rounding-error,eq:sub-gaussian-mean} and the triangle inequality then gives that  
% $$
% \snorm{2}{ R^{-1} \text{Wrap} \lp(\tilde v - b\rp) - \Ep[D] } \leq 2 \eps.
% $$
% This concludes the correctness proof of the algorithm.

\paragraph{Replicability}
Next we argue the replicability.
% Let $u^{(1)}, u^{(2)}$ be the estimtors from \Cref{thm:sub-gaussian-mean} computed from $\Theta \lp(  \lp( N + \log(1/\delta) \rp)
% A^2 N^{-1} \eps^{-2} \rho^{-2} \rp)$ many \iid samples from two runs of the algorithm. 
% \maxh{Is this post coordinate transformation?}
Let $u^{(1)}, u^{(2)}$ be any two inputs satisfying
\begin{align}
\label{eq:median-of-mean-concentration}
\snorm{2}{u^{(1)} - u^{(2)}}
\ll \frac{ \sqrt{N} \eps \rho  }{ A }.
\end{align}
Our goal is to show \Cref{alg:r-rounding} maps $u^{(1)}$ and $u^{(2)}$ to the same point with high probability:
\[
\Pr[\bar{u}^{(1)} = \bar{u}^{(2)}] \geq 1-O(\rho)
\]
where the probability is over the (shared) internal randomness of the procedure.

With this in mind, let $R \sim \Uni( \SO(N) )$, $b \in \Uni\lp( [-\BX,\BX]^N \rp)$, $v^{(i)} = \text{Wrap}\lp( R u^{(i)} + b\rp)$, and  $\tilde v^{(i)} = \eps \mathcal R\lp( \eps^{-1} v^{(i)} \rp)$.
% $v^{(1)}, v^{(2)}$ be the points obtained after the random transformation, i.e., 
% $v^{(i)} = \text{Wrap}\lp( R u^{(i)} + b\rp)$, 
% and $\tilde v^{(1)}, \tilde v^{(2)}$ be the points after applying the rounding queries, i.e., $\tilde v^{(i)} = \eps \mathcal R\lp( \eps^{-1} v^{(i)} \rp)$.
% It is not hard to see that
% the algorithm is always replicable 
Conditioned on the events
$L_1: \tilde v^{(1)} = \tilde v^{(2)}$ and $L_2:\snorm{2}{ \tilde v^{(i)} - v^{(i)} } \leq \epsilon$ for $i \in \{1, 2\}$, 
the algorithm in both runs outputs 
$\bar{u}^{(1)}=R^{-1} \text{Wrap}( \tilde v^{(1)} - b  ) = R^{-1} \text{Wrap}( \tilde v^{(2)} - b  )=\bar{u}^{(2)}$, so it suffices to show
\begin{align}
\label{eq:bad-rep-event}
\Pr(\neg L_1 \lor \neg  L_2) \leq O(\rho). 
\end{align}
Since we only have good control of the membership query when the input point lies in some $V \in \mathcal V$ within the approximate tiling, we will perform a case analysis depending on the ancillary event 
$J: \eps^{-1} v^{(1)}, \eps^{-1} v^{(2)} \in \bigcup_{V \in \mathcal V} V$. 
Note that
\begin{align}
\label{eq:marginalize-J}
\Pr(  \neg L_1 \lor \neg  L_2  )
&= 
\Pr(  \lp( \neg L_1 \lor \neg  L_2 \rp) \land J )
+ \Pr(  \lp( \neg L_1 \lor \neg  L_2 \rp) \land \neg J )
\nonumber \\
&\leq 
\Pr(  \lp( \neg L_1 \lor \neg  L_2 \rp) \land J )
+ 
\Pr(\neg J) \nonumber \\
&\leq
\Pr(  \neg L_1 \land J )
+ 
\Pr( \neg L_2 \land J )
+ 
\Pr(\neg J) \, ,
\end{align}
where in the second inequality we apply the union bound.

We will tackle the three terms separately.
By definition, $\bigcup_{V \in \mathcal V} V$ covers all but a $\rho$-fraction of points within every integer cube.
By \Cref{lem:Buffon-equivalence}, the distribution of $v^{(i)}$ is uniform over the cube $[-Q, Q]^N$. 
Without loss of generality, we assume that $Q$ and $\eps^{-1}$ are both integers. \maxh{Why? The below seems true for non-integer values? If this is just because you want to be careful with mod calculations, shouldn't we say $Q$ is integer earlier? And does it matter still that $\varepsilon^{-1}Q$ be integer?}
Then $\eps^{-1} v^{(i)}$ will be uniformly random over the cube $[-\eps^{-1} Q, \eps^{-1} Q]^N$, implying
\begin{align}
\label{eq:J-bound}
    \Pr(\neg J)
    \leq 2 \; \Pr_{ v \sim \Uni\lp( [-\eps^{-1} Q, \eps^{-1} Q]^N \rp) }( v^{(1)} \not \in \bigcup_{V \in \mathcal V} V \lor v^{(2)} \not \in \bigcup_{V \in \mathcal V} V )
    \leq 2 \rho.
\end{align}
% We first bound from above $\Pr \lp[ \snorm{2}{ \tilde v^{(i)} - v^{(i)} } > \epsilon \rp]$. 
By the definition of an approximate isoperimetric tiling (\Cref{def:approximate-tiling}), each set $V \in \mathcal V$ has diameter $0.1$. 
% \chris{radius 0.1}
Thus, whenever $\eps^{-1} v^{(i)} \in V$ for some $V \in \mathcal V$, 
we will have that
$\snorm{2}{ \eps^{-1} \tilde v^{(i)} - \eps^{-1} v^{(i)} } \leq 1$, which implies that 
$\snorm{2}{  \tilde v^{(i)} -  v^{(i)} } \leq \eps$.
In other words, $J$ implies $L_2$, showing that
\begin{align}
\label{eq:J-imply-L2}
    \Pr(\neg L_2 \land J) = 0.
\end{align}
% By definition, $\bigcup_{V \in \mathcal V} V$ covers all but $\rho$-fraction of points within every integer cube.
% By \Cref{lem:Buffon-equivalence}, the distribution of $v^{(i)}$ is uniform over the cube $[-Q, Q]^N$. 
% It then follows that
% $\Pr \lp[ \snorm{2}{ \tilde v^{(i)} - v^{(i)} } > \epsilon \rp] \leq \rho$.



It remains to bound from above $\Pr(\neg L_1 \land J)$ over the randomness of $v^{(1)}, v^{(2)}$.
Toward this end, we need the following definitions regarding the boundary of our tiling $\mathcal{V}$:
\begin{itemize}
    \item Let $F$ be the union of all boundaries of $\mathcal V$, i.e., 
    $F = \bigcup_{V \in \mathcal V} \partial V$.
    \item Denote by $F_{\mathbb T}$ the torus restriction of $F$ after proper translation and scaling. Specifically, define $F_{\mathbb T}
= 
\lp( F \cap [- \eps^{-1} \BX,  \eps^{-1} \BX]^N \rp)
\; \frac{ \eps }{ 2 \BX } + \mathbf 1_N/2 \subset [0, 1]^N \cong \mathbb T^N$.
\end{itemize}
We note that $\neg L_1 \land J$ happens only if 
$\eps^{-1} v^{(1)}, \eps^{-1} v^{(2)}$ lie in different sets within $\mathcal V$, or equivalently, when the segment $\lp( \eps^{-1} v^{(1)}, \eps^{-1} v^{(2)}\rp)$ intersects with the union of the boundaries $F$.
% We note that the event happens only if $\eps^{-1} v^{(1)}, \eps^{-1} v^{(2)}$ lie in 
% different sets $\mathcal V$.

To bound from above the probability this occurs, we view the segment as a random Buffon needle in $\mathbb T^N$ after proper translation and scaling.
In particular, we consider the torus segment  
$$
\ell_{\mathbb T}\lp( 
\frac{v^{(1)}}{2\BX} + \mathbf 1_N/2
, \frac{v^{(2)}}{2\BX} + \mathbf 1_N/2 \rp).
$$ 
One can verify that this is a well-defined segment in the torus $\mathbb T^N$, indeed $\frac{v^{(i)}}{2\BX} + \mathbf 1_N/2$ lies in $[0, 1]^N$ since $v^{(i)} \in  [-\BX, \BX]^N$.
% Define the event 
% $G: \ell_{\mathbb T}\lp( 
% \frac{v^{(1)}}{2\BX} + \mathbf 1_N/2
% , \frac{v^{(2)}}{2\BX} + \mathbf 1_N/2 \rp) \cap F_{\mathbb T} \neq \emptyset$.
There are only two cases when the segment $ \lp( \eps^{-1} v^{(1)}, \eps^{-1} v^{(2)} \rp)$ intersects with $F$: 
either the above torus segment intersects with $F_{\mathbb T}$   
or  $v^{(1)} + R ( u^{(2)} - u^{(1)} ) \not \in  [-\BX, \BX]^N$ 
% \chris{maybe say this is $v^{(2)}$ without wrapping?} 
(when the torus segment is wrapped around the torus). In other words, we have that 
% \chris{make probabilities consistent}
\begin{align}
&\Pr(\neg L_1 \land J)  \nonumber \\
&\leq \Pr\lp( v^{(1)} + R ( u^{(2)} - u^{(1)} ) \not \in  [-\BX, \BX]^N \rp) + \Pr\lp(  
\ell_{\mathbb T}\lp( 
\frac{v^{(1)}}{2\BX} + \mathbf 1_N/2
, \frac{v^{(2)}}{2\BX} + \mathbf 1_N/2 \rp) \cap F_{\mathbb T} 
\neq \emptyset
\rp).
\label{eq:wrap-around-marginalize}
\end{align}

% We will thus perform another case analysis depending on the ancillary event $E$ : $ v^{(1)} + R ( u^{(2)} - u^{(1)} ) \in  [-\BX, \BX]^N$.
% Intuitively, $E$ tells whether the Buffon needle will be wrapped around the torus in the corresponding Buffon needle process.
% If $E$ happens, then $\neg L_1 \land J$
% Let $E$ be the event that $v^{(1)} + R ( u^{(2)} - u^{(1)} ) \in [-N, N]^N$, and
% $D$ be the event that 
% Note that
% $$
% \Pr[ \neg L_1 \land J ] \leq \Pr[ \neg L_1 \land J \land E] + \Pr[\neg E]    
% $$
It is not hard to see that $ v^{(1)} + R ( u^{(2)} - u^{(1)} ) \not \in  [-\BX, \BX]^N $ only if $v^{(1)}$ is at least $\snorm{2}{ u^{(2)} - u^{(1)} }$-close to some boundary of the cube $ [-\BX, \BX]^N$. Since $v^{(1)}$ is uniform over the cube, we can bound this probability from above as
\begin{align}
\label{eq:close-to-boundary}
\Pr( v^{(1)} + R ( u^{(2)} - u^{(1)} ) \not \in  [-\BX, \BX]^N ) 
\leq 2 N \; \frac{ \snorm{2}{u^{(2)} - u^{(1)}} }{\BX} \ll 
\delta \leq \rho     \, ,
\end{align}
since $\snorm{2}{u^{(2)} - u^{(1)}} \ll \eps$ and 
$\BX \gg N \varepsilon \delta^{-1}$.

It remains to bound the probability that the torus segment $\ell_{\mathbb T}\lp( 
\frac{v^{(1)}}{2\BX} + \mathbf 1_N/2
, \frac{v^{(2)}}{2\BX} + \mathbf 1_N/2 \rp)$ intersects with 
$F_{\mathbb T}$.
To bound the probability of this event,
we consider the expected number of intersections between the torus segment and $F_{\mathbb T}$:
$$
\kappa := \Ep\lp[ 
\abs{
\ell_{\mathbb T}\lp( 
\frac{v^{(1)}}{2\BX} + \mathbf 1_N/2
, \frac{v^{(2)}}{2\BX} + \mathbf 1_N/2 \rp) \cap F_{\mathbb T} }
\rp].
$$
We claim that
\begin{align}
\label{eq:exp-intersection-bound}    
\kappa \leq \rho.
\end{align}
Given \Cref{eq:exp-intersection-bound}, we can apply Markov's inequality to derive that
\begin{align}
% \Pr[  E \text{ and } D ] 
&\Pr\lp(  
\ell_{\mathbb T}\lp( 
\frac{v^{(1)}}{2\BX} + \mathbf 1_N/2
, \frac{v^{(2)}}{2\BX} + \mathbf 1_N/2 \rp) \cap F_{\mathbb T} 
\neq \emptyset
\rp) \nonumber \\
&= \Pr\lp(
\lp|
\ell_{\mathbb T}\lp( 
\frac{v^{(1)}}{2\BX} + \mathbf 1_N/2
, \frac{v^{(2)}}{2\BX} + \mathbf 1_N/2 \rp) \cap F_{\mathbb T} 
\rp|
\geq 1
\rp) \nonumber \\
&\leq \Pr\lp( 
\lp|
\ell_{\mathbb T}\lp( 
\frac{v^{(1)}}{2\BX} + \mathbf 1_N/2
, \frac{v^{(2)}}{2\BX} + \mathbf 1_N/2 \rp) \cap F_{\mathbb T} 
\rp|
\geq \rho^{-1} \kappa
\rp)  \leq \rho \, ,
\label{eq:prob-to-surface}
\end{align}
Combining \Cref{eq:prob-to-surface,eq:wrap-around-marginalize,eq:close-to-boundary} then shows that
\begin{align}
\label{eq:neg-L1-J-bound}
\Pr( \neg L_1 \land J )
\leq O(\rho).
\end{align}
Substituting \Cref{eq:J-bound,eq:J-imply-L2,eq:neg-L1-J-bound} into \Cref{eq:marginalize-J} then shows \Cref{eq:bad-rep-event},
implying that the algorithm is $O(\rho)$-replicable.

% where in the second line we use 
% the fact that $\Ep\lp[ 
% \abs{
% \ell_{\mathbb T}\lp( 
% \frac{v^{(1)}}{2N^2} + \mathbf 1_N/2
% , \frac{v^{(2)}}{2N^2} + \mathbf 1_N/2 \rp) \cap F_{\mathbb T} }
% \rp] \ll 1$ and Markov's inequality \maxh{How? It seems like the first line is $\Pr[|size| > 0]$, so Markov should not imply anything since $|size|$ isn't bounded away from 0?}, and in the third line we apply \Cref{lem:expected-torus-surface-intersection} and \Cref{lem:Buffon-equivalence}.


It remains to show \Cref{eq:exp-intersection-bound}.
Note that the distance between the two points
$ v^{(i)} / (2\BX) + \mathbf 1_{N} / 2 $ within the torus $\mathbb T^N$ is exactly $\snorm{2}{ u^{(1)} - u^{(2)} } / (2\BX)$
\footnote{We define the distance between two points within the torus to be the length of the shortest torus segment connecting the two points. Under such a notion, the torus distance between the two points $ v^{(i)} / (2\BX) + \mathbf 1_{N} / 2 $ is exactly $\snorm{2}{ u^{(1)} - u^{(2)} } / (2\BX)$ in all cases. }.
% . \chris{conditioned on no wrapping?}
By \Cref{lem:Buffon-equivalence} and \Cref{lem:expected-torus-surface-intersection}, it holds
\begin{align*}
\kappa \leq O( N^{-1/2} )
\frac{\snorm{2}{ u^{(1)} - u^{(2)}  }}{2\BX}
\area( F_{\mathbb T} ).
\end{align*}
% where the equality follows from our conditioning of $E$, which implies that there is no wrap around effect when applying the operation
% $v^{(i)} = \text{Wrap} \lp( R u^{(i)} + b \rp)$.
By our assumption \Cref{eq:median-of-mean-concentration}, we further have that
\begin{equation}
\label{eq:kappa-to-area}
\kappa \ll  \frac{ \eps \rho }{2 \; A \; Q} \; \area( F_{\mathbb T} ).    
\end{equation}

We then proceed to bound from above 
$\area( F_{\mathbb T}  )$.
Note that 
\begin{equation}
\label{eq:surface-scale-equality}
    \area( F_{\mathbb T}  ) = 
    \frac{ \area\lp( F \cap [-\eps^{-1} \BX , \eps^{-1} \BX ]^N \rp)  }{ (2 \BX \eps^{-1})^{N-1} }
\end{equation}
by definition.
% Let $\mathcal {\tilde V}$ be the collection of sets within the tiling $\mathcal V$ that have non-trivial intersection with the cube $[-\eps^{-1}N^2, \eps^{-1}N^2]^N$. 
\snew{
Without loss of generality, we assume that $Q \eps^{-1}$ are integers. 
Then the cube $[- \eps^{-1} \BX, \eps^{-1} \BX]^N$ can be partitioned into $ \lp( 2 \eps^{-1} \BX \rp)^N $ many integer unit cubes.
}
Thus, by the property that an \iat{} has small normalized surface area (Property~\ref{item:approximate-tiling:surface-area} in \Cref{def:approximate-cube-isoperimetry}), 
we have that
\begin{equation}
\label{eq:extend-voronoi-boundary-surface}
\area\lp( F \cap [-\eps^{-1}\BX, \eps^{-1}\BX]^N \rp)
\leq 
A  \vol \lp( \bigcup_{V \in \mathcal V }
V \cap [-\eps^{-1}\BX, \eps^{-1}\BX]^N \rp)
\leq A \lp(2\BX \eps^{-1}\rp)^N.
\end{equation}
\begin{remark}
\label{rmk:huge-cube-relax}
We note that this is the only place where we invoke the normalized surface area of an \iat~in the argument. 
Since $\eps^{-1} \BX \gg N$, 
one can see that the argument still holds if we relax the definition to be that the surface area of the tiling within 
any cube of side length $C N$ is at most $O(A) \; (C N)^N$ for some appropriate constant $C$.
This will be important to the proof of \Cref{thm:rep-pre} in \Cref{sec:cvpp}, where we instantiate the tiling to be the Voronoi cells of lattices that don't necessarily give rise to partitions of integer cubes.
\end{remark}
% \maxh{This follows from stacking the side-length 10 cubes I guess? I suppose also requires $N^2/\eps \geq 20$?}
% Since each $V$ has packing radius $1$, 
% applying \Cref{lem:convex-surface-to-volume} gives that
% \begin{align}
% \label{eq:area-to-vol}    
% \sum_{V \in \mathcal {\tilde V}} 
% \area( \delta V )
% \leq N \; \sum_{V \in \mathcal {\tilde V}}
% \vol( V ).
% \end{align}
% Since no two $V, V' \in \mathcal V$ have non-trivial overlap, 
% we have that 
% $ \sum_{V \in \mathcal {\tilde V}}
% \vol( V ) = \vol\lp( \bigcup_{V \in \mathcal {\tilde V}}  V\rp)$.
% Since each $V$ has covering radius $1$, 
% we have $\bigcup_{V \in \mathcal {\tilde V}}
% \subseteq [  -N^2\eps^{-1}-1, N^2 \eps^{-1}+1 ]^N
% $ by the definition of $\tilde V$.
% It then follows that
% \begin{align}
% \label{eq:intersect-vol-bound}
% \sum_{V \in \mathcal {\tilde V}}
% \vol( V )
% \leq (2N^2 \eps^{-1} + 2)^N.    
% \end{align}

Combining 
\Cref{eq:surface-scale-equality,eq:extend-voronoi-boundary-surface,}
then gives
\begin{align*}
\area( F_{\mathbb T}  )
\leq
2 A Q \eps^{-1}
\end{align*}
Substituting the above into \Cref{eq:kappa-to-area} then gives that
\begin{align*}
\kappa 
\ll \frac{\eps \rho}{A Q} \;  A Q  \; \eps^{-1}
\leq \rho \, ,
\end{align*}
which shows \Cref{eq:exp-intersection-bound},
% where in the last inequality we use \Cref{eq:median-of-mean-concentration}.
and hence concludes the proof of \Cref{prop:replicable-rounding}.
\end{proof}

\subsubsection{Reduction to Bounded Domain}
\maxh{Do we really need it to be bounded? Why don't we make the box-size depend on the target norm in a replicable way? I.e. define some giant enough box, where the side length is random depending on the norm of the input vector in such a way that for two nearby points, the box size is the same except with probability $\rho$.}

A slight caveat of our rounding scheme (\Cref{prop:replicable-rounding}) is that it requires the input to be within a bounded cube $[-N, N]^N$. 
We show that this is a mild assumption when we want to apply the routine to replicable mean estimation: there is an easy replicable reduction to the case where the mean of the unknown distribution lies in a bounded domain.
% The first step of our algorithm is to reduce to the simpler setting where the population mean lies in a bounded domain $[-\BD,\BD]^N$.
This is done via a replicable procedure that coarsely learns the mean up to error $\BD$ in $\ell_\infty$ distance. Translating our coordinate system by the learned vector then places the true mean within a $\BD$-length cube with high probability.
\maxh{Probably we need to assume $K<N$ here right?}
\begin{lemma}
\label{lem:warmup-round}
Let $\delta < \rho \in (0, 1)$, and $\distribution$ be a distribution on $\R^N$ with covariance at most $I$. 
Then there exists a $\rho$-replicable algorithm \rCoordinateRound{} that 
draws $\Theta\lp(  
( K \rho / N )^{-2}
\log(N/\delta) \rp) $ many \iid 
vector samples, and efficiently estimates the mean of $\distribution$ up to $K$-accuracy in $\ell_\infty$-distance with probability at least $1 - \delta$.
\end{lemma}
% We start with a simple coordinate-wise rounding scheme that consumes $O(N)$ samples, and allows us to (replicably) reduce to the case where the population mean lies in a box with side length $\tilde O\lp( \sqrt{N}\rp)$.
% To achieve this, we essentially need to estimate the mean up to $\tilde O\lp( \sqrt{N}\rp)$ error in $\ell_\infty$ distance.

\rCoordinateRound{} is based on the classical ``median-of-mean'' estimator. 
% whose concentration properties follow from Chebyshev's inequality and the union bound.
\begin{claim}[Median of Means]
\label{clm:median-of-mean}
Let $\delta \in (0, 1)$, and $\distribution$ be an $N$-dimensional distribution with 
mean $\mu$ and covariance at most $I$. 
Given $m$ \iid samples, there exists a \algname{Median-of-Mean} estimator 
$\bar \mu$ such that
\begin{align*}
\snorm{\infty}{ \bar \mu  - \mu}
\leq O \lp( \sqrt{\log (N/\delta) / m} \rp)
% \snorm{2}{ \bar \mu  - \mu}
% \leq O \lp( \sqrt{ N \log (N/\delta) / m} \rp) \, ,
\end{align*}
with probability at least $1 - \delta$.
\end{claim}
\begin{proof}
After taking $m /  \log(N/\delta) $ many samples, 
the algorithm computes the empirical mean $\hat \mu$.
Let $\mu$ be the true mean of $\distribution$.
Fix some coordinate $i$.
By Chebyshev's inequality, we have that $\abs{\hat \mu_i - \mu_i} \leq O \lp( \sqrt{ \log (N/\delta) / m } \rp)$ with probability at least $2/3$.
If we repeat this process $T:=\log(N/\delta)$ many times, we obtain a set of empirical means $\hat \mu^{(1)}, \cdots, \hat \mu^{(T)}$.
Let $\bar \mu$ be the coordinate-wise median of these empirical means.
Fix some coordinate $i$.
Then, by the Chernoff Bound, it holds that
$\abs{\bar \mu_i - \mu_i} \leq O \lp( \sqrt{ \log (N/\delta) / m } \rp)$ with probability at least $1 - \delta / N$.
Finally union bounding over $N$ coordinates gives that
$$
\snorm{\infty}{ \bar \mu - \mu  } \leq O \lp( \sqrt{ \log (N/\delta) / m } \rp)
$$
with probability at least $1 - \delta$.
% Then $\ell_2$ bound follows from the fact that $\snorm{2}{u} \leq \sqrt{N} \snorm{\infty}{u}$ for any $u \in \R^N$.
\end{proof}
We obtain the desired coarse replicable estimator simply by rounding each coordinate of Median-of-Means to the nearest integer multiple of $N$.
% , we obtain a replicable mean estimation algorithm.
% The algorithm does not have optimal sample efficiency. 
% Nonetheless, if we translate the coordinate system by the sample mean learned, 
% we can replicably reduce to the case where the population mean lies in a bounded domain.
\begin{proof}[Proof of {\Cref{lem:warmup-round}}]
Let $\bar \mu$ be the \textit{Median-of-Mean} estimator from \Cref{clm:median-of-mean} computed from $m \geq C \; ( K \rho / N )^{-2}
\log(N/\delta)$ many samples for some sufficiently large constant $C$.
Then by \Cref{clm:median-of-mean}
\begin{align}
\label{eq:median-of-mean-err}
\snorm{\infty}{\bar \mu - \mu} \leq  K \rho  / N
\end{align}
with probability at least $1 - \delta$.
Consider the process in which we round each coordinate of $\bar \mu$ to the nearest integer multiples of $ K $ based on some random threshold chosen uniformly at random. 
Specifically, if $\bar \mu_i \in [a K, (a+1) K]$ for some integer $a$, we choose $\alpha_i \sim \Uni( [aK, (a+1)K] )$, and round $\bar \mu_i$ to $aK$ if $\bar \mu_i < \alpha_i$ (and to $(a+1) K$) otherwise.
Fix some coordinate $i$.
% If we choose the rounding threshold 
% for the $i$-th coordinate uniformly at random \maxh{Maybe specify you pick threshold $\alpha \in [0,N\log N]$ u.a.r and round based on comparison to alpha mod $N\log N$.},
It holds that $\mu_i$ is $K \rho / N$ close to a rounding threshold with probability at most $O(\rho / N)$. 
% Denote the rounding result as $\tilde \mu$
By the union bound, the rounding threshold $\alpha_i$ is at least $K \rho / N$-far from the true mean $\mu_i$ for every coordinate $i$ with probability at least $1 - O(\rho)$.  
It then follows that the algorithm's output is replicable with probability at least $1 - O(\rho)$.
Finally, the resulting error of the rounded estimator follows from \Cref{eq:median-of-mean-err} and the fact that the rounding shifts each coordinate by at most $K$.
\end{proof}



\subsubsection{A Replicable \texorpdfstring{$\ell_2$}{2 norm} Estimator}
To prove \Cref{thm:tiling-to-replicable}, we combine \Cref{prop:replicable-rounding} with an $\ell_2$ estimator for bounded covariance distributions.
% Though it is tempting to use just the empirical means, 
% we note that the epi mean fails to achieve the optimal sub-Gaussian convergence rate for distributions with only bounded covariance. 
Since we care about the sample complexity of the problem in the high success probability regime, we will be using the estimator from \cite{cherapanamjeri2019fast}.
Importantly, the estimator achieves the optimal sub-gaussian convergence rate, and is efficiently computable.
\begin{theorem}[Sub-Gaussian mean estimator from \cite{cherapanamjeri2019fast}]
\label{thm:sub-gaussian-mean}
Let $\distribution$ be a distribution 
on $\R^N$
with covariance bounded from above by $I$, and $\snorm{2}{ \Ep[\distribution] } \leq \poly{N}$.
Given $m$ \iid samples from $\distribution$,
there exists an efficient algorithm that computes an estimate $\hat \mu$ such that 
\begin{align*}
\snorm{2}{\Ep[\distribution]  - \hat \mu}
\leq O\lp( 
\sqrt{ d / m }
+ \sqrt{ \log(1/\delta) / m }
\rp).
\end{align*}
\end{theorem}
\IncMargin{1em}
\begin{algorithm}

\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}\SetKwInOut{Parameters}{Parameters}
\Input{Sample access to distribution $\distribution$ on $\R^N$ and rounding query $\mathcal R: \R^N \mapsto \R^N$.}
\Parameters{$\eps$ accuracy}
\Output{
$\bar \mu$: an estimate of $\Ep[\distribution]$ up to $\eps$-accuracy
in $\ell_2$ distance.}
\begin{algorithmic}[1]
% \State Set $\BX = C \; \lp( N \eps \delta^{-1} + \sqrt{N} (\BD + \eps) \rp)$, for some sufficiently large constant $C$.
\State 
Set $m_1:=C  \log(N/\delta) \rho^{-2}$ and $m_2 := 
C \; \lp( N + \log(1/\delta) \rp) A^2 N^{-1} \eps^{-2} \rho^{-2}$
for some sufficiently large constant $C$.
\State Use \Cref{lem:warmup-round} to replicably learn $\tilde u$
with $m_1$ samples such that $\snorm{\infty}{ \tilde u - \Ep[\distribution]} \leq N$ in $\ell_\infty$ distance.\label{line:warmup1}

\State Transform the coordinate system by $\tilde \mu$. \label{line:warmup2}
\State Compute the \snew{estimator $u$ with the algorithm from \Cref{thm:sub-gaussian-mean}} with $m_2$ many samples.
% \If{Norm is $\ell_2$}
% with $m_2$ many samples.
% \ElseIf{Norm is $\ell_\infty$}
% \State Compute the \snew{median-of-mean estimator $u$ (\Cref{clm:median-of-mean})} with $m_3$ many samples.
% \EndIf



\State Round $u$ into $\bar u$ with the randomized rounding scheme \Cref{alg:r-rounding} with accuracy $\epsilon$, failure probability $\delta$, and replicability parameter $\rho$.

\State Output $\bar u$.


\caption{Replicable $\ell_2$ mean estimator} 
\label{alg:r-mean-est}

\end{algorithmic}
\end{algorithm}
\DecMargin{1em}
We are now ready to conclude the proof of \Cref{thm:tiling-to-replicable}.
\begin{proof}[Proof of \Cref{thm:tiling-to-replicable}]
By \Cref{lem:warmup-round}, the warmup rounding process (Lines~\ref{line:warmup1} and~\ref{line:warmup2} from \Cref{alg:r-mean-est}) succeeds with probability at least $1 - \delta$, and is $\rho$-replicable.
Conditioned on that, we reduce to the case where the distribution mean $\Ep[\distribution]$ lies in the domain $[-N/2 , N/2]^{N}$.

% \paragraph{Correctness}
% We first argue the correctness of the algorithm.
Let $u$ be the estimator from \Cref{thm:sub-gaussian-mean} computed from $\Theta \lp(  \lp( N + \log(1/\delta) \rp)
A^2 N^{-1} \eps^{-2} \rho^{-2} \rp) \gg (N + \log(1/\delta)) \eps^{-2}$ \iid samples (Recall that we know the surface-to-volume ratio $A$ of any tiling is at least $N$ by the isoperimetric inequality).
By \Cref{thm:sub-gaussian-mean}, we have that
% Note that $u - \Ep[D]$ is a random vector with $0$ mean and covariance at most $\frac{1}{m}I$, its expected squared $\ell_2$ norm is at most $N/m$ and by Markov's inequality we have
\begin{align}
\label{eq:sub-gaussian-mean}
\snorm{2}{u - \Ep[\distribution]} \ll  \frac{\sqrt{N} \eps \rho  }{A} \,
% \text{ for } i \in \{1, 2\}
\end{align}
\snew{with probability at least $1 - \delta$.}
Applying \Cref{prop:replicable-rounding} gives that
$\snorm{2}{ \bar u - u } \leq \eps$ with probability at least $1 - \delta$.
Thus, the output is close to $\Ep[\distribution]$ in $\ell_2$ distance with probability at least $1 - 2 \delta$ by the union bound and the triangle inequality. 

Let $u^{(1)}, u^{(2)}$ be the estimator computed in two different runs of the algorithm. Still, by the triangle inequality and the union bound, it holds that
$$
\snorm{2}{ u^{(1)} - u^{(2)} } \ll  \frac{\sqrt{N} \eps \rho  }{A}.
$$
Conditioned on the above, 
applying \Cref{prop:replicable-rounding} gives that the algorithm is replicable with probability at least $1 - \rho$.
This concludes the proof of \Cref{thm:tiling-to-replicable}.
\end{proof}

\subsubsection{A Replicable \texorpdfstring{$\ell_\infty$}{infinity norm} Estimator}
% Finally, we prove \Cref{thm:ell-infty-mean}.

Finally we cover the case of $\ell_\infty$-mean-estimation (\Cref{thm:ell-infty-mean}). The algorithm is identical to \Cref{alg:r-mean-est} except that we replace the non-replicable estimator from \Cref{thm:sub-gaussian-mean}, which is customized for $\ell_2$ estimation, with the Median-of-Means estimator from \Cref{clm:median-of-mean}. Roughly speaking replicability then follows the same argument, while for correctness we take advantage of the fact that
% Replicability of the algorithm largely follows from the fact that we use the same randomized rounding procedure as the $\ell_2$ learning algorithm.
% To argue the correctness of the algorithm, we will take advantage of the fact that 
the rounding error vector $\xi$ points in a uniformly random direction.
% Without the randomized rounding procedure, the error bound follows from concentration properties of the median-of-mean estimator
% (\Cref{clm:median-of-mean}).
% Thus, it remains to argue that the randomized rounding procedure
% introduces small error in $\ell_\infty$ distance. 
% The argument from the proof of \Cref{thm:tiling-to-replicable} give that the rounding error is small in $\ell_2$ distance.
% To turn that into 
% At a high level, the correctness follows from the observation that the error vector
% $\bar u - \Ep[D]$ will be in a uniformly random direction.
This means that with high probability
$$
\snorm{\infty}{\xi} \leq O \lp( \log N \snorm{2}{\xi} / \sqrt{N} \rp),
$$
allowing us to save an extra factor of $\tilde \Theta\lp(N\rp)$ from the overall algorithm's sample complexity.
\IncMargin{1em}
\begin{algorithm}

\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}\SetKwInOut{Parameters}{Parameters}
\Input{Sample access to distribution $\distribution$ on $\R^N$ and rounding query $\mathcal R: \R^N \mapsto \R^N$.}
\Parameters{$\gamma$ accuracy}
\Output{
$\bar \mu$: an estimate of $\Ep[\distribution]$ up to $\gamma$-accuracy
in $\ell_\infty$ distance.}
\begin{algorithmic}[1]
% \State Set $\BX = C \; \lp( N \eps \delta^{-1} + \sqrt{N} (\BD + \eps) \rp)$, for some sufficiently large constant $C$.
\State 
Set $m_1:=C  \log(N/\delta) \rho^{-2}$ and $m_2 := 
C \;    A^2 N^{-1} \; \log^3(N/\delta) \; \gamma^{-2} \rho^{-2}$
for some sufficiently large constant $C$.
\State Use \Cref{lem:warmup-round} to replicably learn $\tilde u$
with $m_1$ samples such that $\snorm{\infty}{ \tilde u - \Ep[\distribution]} \leq N$.

\State Transform the coordinate system by $\tilde \mu$.
\State Compute the median-of-mean estimator $u$ (\Cref{clm:median-of-mean}) with $m_2$ many samples.
% \If{Norm is $\ell_2$}
% with $m_2$ many samples.
% \ElseIf{Norm is $\ell_\infty$}
% \State Compute the \snew{median-of-mean estimator $u$ (\Cref{clm:median-of-mean})} with $m_3$ many samples.
% \EndIf

\State Round $u$ into $\bar u$ with the randomized rounding scheme \Cref{alg:r-rounding} with accuracy $\epsilon:=\sqrt{N} \gamma / \log(N/\delta)$, failure probability $\delta$, and replicability parameter $\rho$.

\State Output $\bar u$.


\caption{Replicable $\ell_{\infty}$ mean estimator} 
\label{alg:r-mean-est-infty}

\end{algorithmic}
\end{algorithm}
\DecMargin{1em}
\begin{proof}[Proof of \Cref{thm:ell-infty-mean}]
% If we want to estimate up to accuracy $\gamma$ in $\ell_\infty$ distance, 
% we will use the $\ell_2$ estimation algorithm
% \Cref{alg:r-mean-est} but set the accuracy parameter as $\eps = \gamma \sqrt{N} / \sqrt{\log N}$.
% Besides, instead of rounding the empirical mean, we now set $u$ to be the median-of-mean estimator (\Cref{clm:median-of-mean}) computed from $m := \Theta \lp( A^2 \log N \eps^{-2}  \rp)$ many samples.
% Replicability of the algorithm follows from the proof of \Cref{thm:tiling-to-replicable}.

% It remains to show correctness of the algorithm.
% We will use the same set of notations as the proof of \Cref{thm:tiling-to-replicable}.
As in the proof of \Cref{thm:tiling-to-replicable}, condition on the success of the warm-up rounding procedure and assume therefore that $\Ep[\distribution] \in [-N/2, N/2]^N$.

Let $u^{(1)}, u^{(2)}$ be the median-of-mean estimators computed 
from $m = C \; A^{2} N^{-1} \log^3(N/\delta) \gamma^{-2} \rho^{-2}$ many samples in two runs.
By \Cref{clm:median-of-mean}, we have that
$$
\snorm{\infty}{ u^{(i)} - \Ep[\distribution] } \ll 
\frac{\sqrt{N} \gamma \rho }{ \log(N/\delta) A} \, ,
$$
which implies that
$$
\snorm{2}{ u^{(i)} - \Ep[\distribution] } \ll 
\frac{N \gamma \rho }{\log(N/\delta) A}
$$
for $ i \in \{1, 2\}$.
% Let $u^{(1)}, u^{(2)}$ be the estimators computed in two different runs of the algorithm.
By the union bound and the triangle inequality,
we have that
$$
\snorm{2}{ u^{(1)} - u^{(2)} } \ll \frac{N \gamma \rho }{\log(N/\delta) A}.
$$
Conditioned on this event, applying \Cref{prop:replicable-rounding} 
with $\eps = \sqrt{N} \gamma / \log(N/\delta)$ gives that the algorithm is replicable
with probability at least $1 - \rho$.

It remains to argue correctness.
Let $u$ be the Median-of-Means estimator computed in a single run of the algorithm, and $\bar u$ be the rounding result. 
% Again by \Cref{prop:replicable-rounding}, we have that
% $$
% \snorm{2}{ u - \bar u } \leq \sqrt{N} \gamma.
% $$
To argue that $u$ and $\bar u$ are close in $\ell_\infty$ norm, we need to take a closer look at the randomized rounding scheme.
In particular, let $v = \text{Wrap}\lp( R u + b \rp)$, where $R \sim \Uni( \SO(N) )$, $b \in \Uni\lp( [-N^2 , N^2]^{N} \rp)$,  and $\tilde v = \eps \mathcal R( \eps^{-1} v)$ where $\mathcal R$ is the rounding query with respect to the tiling $\mathcal V$, and $\eps = \sqrt{N} \gamma / \log (N/\delta)$. 
Then we have $ \bar u = R^{-1} \text{Wrap}\lp(  \tilde v - b \rp) $.
\maxh{Box size here is different than in the rounding scheme. $N^2$ vs $Q$? Also isn't $\bar{u}$ only this under some conditions on $v$ and $\tilde{v}$?}
% By \Cref{clm:median-of-mean}, we have that the median-of-means estimator satisfies
% \[
% ||u-\mathbb{E}[D]||_\infty \ll \gamma
% \]
% with high constant probability, so it is enough to argue that $||u-\bar{u}||_\infty \ll \gamma$.

Toward this end, we will condition on the following events: (i) the warmup rounding procedure succeeds such that we reduce to the case
$\Ep[\distribution] \in [-N/2, N/2]^{N}$, (ii) 
the median of mean estimator $u$ is $\sqrt{N} \gamma / \log(N/\delta)$-close to $\Ep[\distribution]$ in $\ell_2$ distance, and (iii)
$v$ is at least $\sqrt{N} \gamma / \log(N/\delta)$-far from the boundary of the cube $ [-\BX, \BX]^N$.
By \Cref{lem:warmup-round}, (i) succeeds with probability at least $1 - \delta$.
(ii) holds with probability at least $1 - \delta$ as argued in the replicability proof.
Finally from the correctness proof of \Cref{thm:tiling-to-replicable}, we know that (iii) also holds with high probability at least $1 - \delta$.
By the union bound, the above events hold simultanously with probability at least $1 - O(\delta)$.

Under these conditions, recall from \Cref{claim:rounding-error} and \Cref{claim:no-wrapping} we always have
\begin{align}
\label{eq:before-rotation}
\snorm{2}{ 
\text{Wrap}\lp( v - b \rp) - 
\text{Wrap}\lp( \tilde v - b \rp) } \leq \sqrt{N} \gamma / \log(N/\delta).
\end{align}
and
    \begin{align}\label{eq:no-wrapping-2}
R^{-1}\text{Wrap}(v-b) = u
\end{align}
These immediately give us a bound on $\ell_2$ error. 
To get the bound on $\ell_\infty$, we use the random rotation $R$ to argue the coordinates of the error vector are near-uniform. To do this, we need to first observe that $R$ remains uniform over $\SO(N)$ even under the above conditions. Note these conditioning are on the random variables $v, u$ and the success of the warmup rounding procedure. The latter two are clearly independent from the randomness of $R$. Hence, it suffices to show that the distribution of $R$ is still uniform over $\SO(N)$ conditioned on any value of $v$.
It is not hard to see that the distribution of $v$ is uniform conditioned on any $R$. Namely since $v=\text{Wrap}(Ru+b)$, which is uniform no matter the `start point' $Ru$. This implies that $v, R$ are independent, so in particular $R$ is still uniform conditioned on any particular value of $v$.

We now bound the distance from $u$ to the output $\bar u = R^{-1}\text{Wrap}( \tilde v - b )$ in $\ell_\infty$ distance. First, by \Cref{eq:no-wrapping-2}, we have
\[
\snorm{\infty}{ R^{-1} \text{Wrap} \lp(\tilde v - b\rp)  -  u
}
=
\snorm{\infty}{ R^{-1} 
\lp( 
\text{Wrap} \lp(\tilde v - b\rp)  - 
\text{Wrap} \lp(v - b\rp) 
\rp)}.
\]
Fix any $v$ such that \Cref{eq:before-rotation} is satisfied ($\tilde v$ is then also uniquely determined).
Consider the $i$-th coordinate of the vector $R^{-1} \lp( 
\text{Wrap} \lp(\tilde v - b\rp)  - 
\text{Wrap} \lp(v - b\rp) 
\rp)$. We thus have
\begin{align*}
&\Ep_{ R \sim \Uni( \SO(N) )  }
\lp[ 
\lp( R^{-1} 
\lp( 
\text{Wrap} \lp(\tilde v - b\rp)  - 
\text{Wrap} \lp(v - b\rp) 
\rp) \rp)_i
\rp] \\
 &\leq O\lp( N^{-1/2} \rp)  \snorm{2}{\lp( 
\text{Wrap} \lp(\tilde v - b\rp)  - 
\text{Wrap} \lp(v - b\rp) 
\rp)}\\
 &\leq O( \gamma / {\log (N/\delta)} ) \, ,
\end{align*}
where in the last inequality we use \Cref{eq:before-rotation}.
By the concentration of inner product of random unit vectors (see e.g.\ \cite[Theorem A.10]{diakonikolas2023algorithmic}), we have that
$$
\Pr \lp(
 \lp| \lp( R^{-1} 
\lp( 
\text{Wrap} \lp(\tilde v - b\rp)  - 
\text{Wrap} \lp(v - b\rp) 
\rp) \rp)_i \rp|
 \geq  C' \gamma 
\rp)
\leq \delta / N \, ,
$$
where $C'$ is a sufficiently large constant.
\maxh{Clarify application of Theorem A.10 is to basis vector $e_i$, maybe footnote that statement is for two random unit vectors but applies to $1$ fixed by randomly rotating.}

By the union bound, it follows that 
$$
\snorm{\infty}{ 
R^{-1}  \text{Wrap} \lp(\tilde v - b\rp)  - 
u} =
\snorm{\infty}{ R^{-1} 
\lp( 
\text{Wrap} \lp(\tilde v - b\rp)  - 
\text{Wrap} \lp(v - b\rp) 
\rp)} \leq O(\gamma)
$$
with probability at least $1 - O(\delta)$, completing the proof.
% Lastly, from standard concentration arguments, we have that
% $ \snorm{\infty}{u - \Ep[D]} \leq \gamma$ with high constant probability. Hence, by the union bound and the triangle inequality, we have that 
% $$
% \snorm{\infty}{ R^{-1}  \text{Wrap} \lp(\tilde v - b\rp) - \Ep[D] } 
% \leq O\lp( \gamma\rp)
% $$
% with high constant probability. 
% This concludes the proof of \Cref{thm:ell-infty-mean}.
\end{proof}



==> inputs/statistical_queries.tex <==
\subsection{Multiple Statistical Queries}
\label{sec:n-coin:n-stat-q}

A natural application of our multiple hypothesis testing framework is the problem of replicably answering many statistical queries at once.
Our adaptive single statistical query algorithm above gives a simple computationally efficient algorithm for replicably answering $N$ statistical queries using only $N^2$ samples.

\iffalse 

Next, we define both the non-adaptive and adaptive $N$ query statistical query oracle for multiple queries.
In the adaptive statistical query oracle setting, we answer queries sequentially.
In particular, the query $\phi_i$ is allowed to depend on the outputs of the statistical query oracle on previous queries.
In the non-adaptive setting, we can assume that all queries $\phi_i$ are given simultaneously.

\begin{definition}[Non-Adaptive Statistical Query Algorithm]
Let $\distribution$ be a distribution over domain $\domain$.
Let $\tau, \delta \in [0, 1]$ and $\phi_i: \domain \mapsto [0, 1]$ be queries.
Let $\mu_i = \E{\phi_i(x)}$ where $x$ is drawn from $\distribution$.
Then, a $N$-query non-adaptive statistical query oracle algorithm outputs $v$ such that $|v_i - \mu_i| \leq \tau$ for all $i$ with probability at least $1 - \delta$.
\end{definition}

\fi

\begin{definition}[Adaptive Statistical Query Algorithm]
Let $\distribution$ be a distribution over domain $\domain$.
Let $\tau, \delta \in [0, 1]$ and $\phi_i: \domain \mapsto [0, 1]$ be queries.
Let $\mu_i = \E{\phi_i(x)}$ where $x$ is drawn from $\distribution$.
Then, a $N$-query adaptive statistical query oracle algorithm outputs $v$ such that $|v_i - \mu_i| \leq \tau$ for all $i$ with probability at least $1 - \delta$.
In the adaptive setting, the query function $\phi_i$ is allowed to depend on 
the results of the previous statistical query oracles, i.e., $\{ v_j \}_{j=1}^i$.
\end{definition}

% In this section, we give matching upper and lower bounds for non-adaptive and adaptive statistical query oracles.
% Since the sample complexities are identical up to polylogarithmic factors, we show an upper bound for the adaptive setting and a lower bound for the non-adaptive setting.

We give the algorithm below.

\begin{restatable}{theorem}{rnstatqoracle}
    \label{thm:r-n-stat-q-adaptive}
    Let $\frac{1}{2} \geq \rho > \delta > 0$.
    Algorithm \ref{alg:r-n-stat-q} is a $\rho$-replicable $N$-query adaptive statistical query oracle algorithm with expected sample complexity $\bigtO{\frac{N^2}{\tau^2 \rho}}$ and worst case sample complexity $\bigtO{\frac{N^2}{\tau^2 \rho^2}}$.
\end{restatable}

\IncMargin{1em}
\begin{algorithm}

\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}\SetKwInOut{Parameters}{Parameters}
\Input{Sample access to distribution $\distribution$ over $\domain$. 
Statistical queries $\set{\phi_{i}}_{i = 1}^{N}$ with $\phi_i: \domain \mapsto [0, 1]$}
\Parameters{$\rho$ replicability, $\tau$ tolerance, and $\delta$ accuracy}
\Output{$\hat{v} \in [0, 1]^{N}$}

$\mathrm{SampleLimit} \gets C \frac{N^2}{\tau^2 \rho^2} \log \frac{N}{\delta}$

\If{Total number of samples collected exceeds $\mathrm{SampleLimit}$}{
    \Return $\multiStatQ \left(\distribution, \set{\phi_{i}}_{i = 1}^{N}, \tau, \delta / 2 \right)$
}

\For{$i \in [N]$}{
    $v_i \gets \rAdaptiveStatQ\left( \domain, \phi_i, \frac{\rho}{2N}, \tau, \frac{\delta}{2N} \right)$
}

\Return $v$

\caption{$\rMultiStatQ \left(\distribution, \set{\phi_{i}}_{i = 1}^{N}, \rho, \tau, \delta \right)$} 
\label{alg:r-n-stat-q}

\end{algorithm}
\DecMargin{1em}

The proof of Theorem \ref{thm:r-n-stat-q-adaptive} closely follows that of Theorem \ref{thm:r-n-coin-problem}.
In particular, we simply apply $\rAdaptiveStatQ$ to each query, drawing fresh samples from distribution $\distribution$ for each query.

\begin{proof}[Proof of Correctness of \Cref{alg:r-n-stat-q}]
    Correctness follows immediately from the correctness of the algorithms $\multiStatQ$ and $\rAdaptiveStatQ$ and the union bound.
\end{proof}

\begin{proof}[Proof of Replicability of \Cref{alg:r-n-stat-q}]
    If the sample limit is not reached, then replicability follows from the replicability of the algorithm $\rAdaptiveStatQ$ and the union bound.
    It therefore suffices to bound the probability that we reach the sample limit.
    In order to apply the union bound, we draw fresh samples from $\distribution_i$ to answer each statistical query. 
    For each $i$, let $M_i$ denote the number of samples required to answer the $i$-th query $\phi_i$.
    From Theorem \ref{thm:r-adaptive-stat-q}, we have that,
    \begin{align*}
        M_i &= \bigO{\frac{N^2}{\tau^2 \rho^2} \log \frac{N}{\delta}} \\
        \E{M_i} &= \bigO{\frac{N}{\tau^2 \rho} \log \frac{N}{\delta}}
    \end{align*}
    where we require each distinguisher to be $\frac{\delta}{2N}$-accurate and $\frac{\rho}{2N}$-replicable.

    Then, if we let $M = \sum M_i$ denote the total sample complexity,
    \begin{equation*}
        \E{M} = \sum_{i = 1}^{N} \E{M_i} = \bigO{\frac{N^2}{\tau^2 \rho} \log \frac{N}{\delta}} \leq C \frac{N^2}{\tau^2 \rho} \log \frac{N}{\delta}
    \end{equation*}
    where $C$ is some large enough constant.

    Since $M$ is a non-negative random variable, we apply Markov's inequality,
    \begin{equation*}
        \Pr\left(M > C \frac{N^2}{\tau^2 \rho^2} \log \frac{N}{\delta} \right) < \rho
    \end{equation*}
    and therefore upper bound the probability that we exceed the total sample limit.
\end{proof}

\begin{proof}[Proof of Sample Complexity of \Cref{alg:r-n-stat-q}]
    The total number of samples taken is at most the sum of $\mathrm{SampleLimit}$ and the sample complexity of $\multiCoinTester$.
    From Lemma \ref{lemma:n-stat-q}, this is at most $O(\mathrm{SampleLimit})$.

    The expected sample complexity is exactly that of $N$ copies of $\rAdaptiveCoinTester$ since the probability of hitting $\mathrm{SampleLimit}$ is at most $\rho$.
\end{proof}

The following lemma gives a statistical query oracle with no replicability guarantee.

\begin{lemma}
    \label{lemma:n-stat-q}
    There is a $N$-statistical query oracle with total sample complexity
    \begin{equation*}
        m = \bigO{\frac{N}{\tau^2} \log \frac{N}{\delta}} = \bigtO{\frac{N}{\tau^2}}
    \end{equation*}

    Denote this algorithm $\multiStatQ$.
\end{lemma}

\begin{proof}[Proof of Lemma \ref{lemma:n-stat-q}]
    If we ignore replicability, there is a simple statistical query oracle with sample complexity $\bigO{\frac{1}{\tau^2} \log \frac{1}{\delta}}$.
    In particular, we can simply run Algorithm \ref{alg:r-adapt-stat-q} with only the first iteration $t = 1$ and output $v_i$ as the empirical mean of $\phi_i(x)$ for $x$ sampled from distribution $\distribution$.
    By Lemma \ref{lemma:sample-error-bound}, we have $|v_i - \mu_i| \geq \tau_t = \tau_1 = \frac{\tau}{8}$ with probability at most $\frac{\delta}{2}$.

    Now we would like to simultaneously 
    To do so, it suffices to amplify the accuracy parameter to $\frac{\delta}{N}$, so that each coin has sample complexity $\bigO{\frac{q_0}{(q_0 - p_0)^2} \log \frac{N}{\delta}}$.
    Performing this amplified test over $N$ coins completes the lemma.
\end{proof}

\iffalse

\subsection{Lower Bounds for Multiple Statistical Query Oracles}

The multiple statistical query problem is qualitatively different from the multiple coin problem.
Specifically, the samples from the distribution $\distribution$ could be shared between various statistical queries, whereas samples from different coins are drawn from completely independent distributions. 
At least intuitively, it is feasible that the $N$ statistical queries can share samples from the distribution $\distribution$, therefore reducing overall sample complexity.
In this section, we show that this is in fact not possible, even for non-adaptive $N$-query statistical query oracles when the $N$ statistical queries are all given in advance.
Specifically, we show that even for the $N$ coin problem, a replicable algorithm requires for at least one coin, a number of samples matching the overall sample complexity.
Our results show that under the constraint of replicability, non-adaptive and adaptive statistical query oracles have the same sample complexity, up to polylogarithmic factors.
The lower bound follows a reduction similar to Theorem \ref{thm:n-coin-lower-adaptive}.

\begin{theorem}
    \label{thm:n-coin-one-coin-sample-lower}
    Let $\tau < \frac{1}{4}$.
    Let $\rho, \delta < \frac{1}{16}$.
    Any $\rho$-replicable non-adaptive $N$-query statistical query oracle $\innerAlg$ requires expected sample complexity at least,
    \begin{equation*}
        \bigOm{\frac{N^2}{\rho \tau^2}}
    \end{equation*}
\end{theorem}

\begin{proof}
    A $\tau$-tolerant $\rho$-replicable statistical query algorithm naturally induces a $\rho$-replicable algorithm for the $N$ coin problem with $p_0 = \frac{1}{2} - \tau$ and $q_0 = \frac{1}{2} + \tau$, where the results of the coin flips are $\phi_i(x)$.
    Specifically, we can imagine $\domain$ to be the set of all (infinite) length binary strings and $\phi_i(x)$ to be the $i$-th bit of some string $x$.
    The distribution $\distribution$ can then be fixed so that the marginal distributions of $\phi_i(x)$ are bernoulli random variables with bias $p_i$ for all $i$.
    Furthermore, note that in the $N$ coin problem, all queries $\phi_i$ are given in advance, so that a non-adaptive $N$-query statistical query oracle can successfully determine the bias of all $N$ coins.
    Therefore, to obtain a lower bound against non-adaptive $N$-query statistical query oracles, it suffices to obtain a sample complexity lower bound against replicable algorithms for the $N$ coin problem.

    \proofparagraph{Lower Bound on $N$ Coin Problem: Maximum Sample Complexity of Single Coin}

    Let $\innerAlg$ be a $\rho$-replicable algorithm for the $N$ coin problem.
    Let $M_i$ be a random variable denoting the number of samples drawn from the $i$-th coin.
    Let $M = \sum M_i$ and $M_{\max} = \max M_i$.
    Observe that $M \leq N M_{\max}$.
    Suppose for contradiction that $\E{M_{\max}} = \littleO{\frac{N^2}{\rho \tau^2}}$.

    We then construct a non-adaptive algorithm for the $N$ coin problem as in Algorithm \ref{alg:r-n-coin-tester-lb}, setting $m = \ceil{\frac{4 \E{M}}{\rho}}$ to be the sample limit for all coins.
    Then, following Markov's inequality no coin is sampled more than $m$ times except with probability $\frac{\rho}{4}$.
    In this case, Algorithm \ref{alg:r-n-coin-tester-lb} returns the result from $\innerAlg$ so that $\outerAlg$ is replicable by the union bound.
    Observe that correctness follows from the union bound and the correctness of $\multiCoinTester$ and $\innerAlg$.
    Finally, we bound the sample complexity,
    \begin{equation*}
        \sum m_i = \bigO{\frac{N}{\rho} \E{M}} = \littleO{\frac{N^3}{\rho^2 \tau^2}}
    \end{equation*}
    violating Theorem \ref{thm:n-coin-lower-const-prob}.

    \proofparagraph{Lower Bound for $N$-Query Statistical Oracle}

    Following the earlier discussion, this implies our sample complexity lower bound for non-adaptive statistical query oracles.
    In particular, any non-adaptive statistical query oracle also solves the $N$ coin problem.
    Since we require $\frac{N^2}{\rho \tau^2}$ samples from a single coin to solve the $N$ coin problem, even with reusing samples between different queries, the statistical query oracle is still subject to this lower bound as the corresponding statistical query oracle requires $\frac{N^2}{\rho \tau^2}$ samples from the input distribution $\distribution$.
\end{proof}

\fi

==> inputs/uniformity_testing.tex <==
\section{Replicable Uniformity Testing}
\label{sec:uniformity-testing}

In this section, we give an algorithm with almost optimal sample complexity for the uniformity testing problem, and a matching lower bound up to polylogarithmic factors.
In the uniformity testing problem, we are given an unknown distribution on a finite domain $[n]$, and we are asked to determine whether the unknown distribution is uniform or $\varepsilon$-far from uniform.

\begin{definition}[Uniformity Testing Problem]
    Let $\varepsilon, \delta > 0$.
    Let $U_{n}$ denote the uniform distribution on $[n]$.
    Given samples to an unknown distribution $\distribution$ on $[n]$, a uniformity testing algorithm satisfies the following with probability at least $1 - \delta$:
    \begin{enumerate}
        \item (Completeness) If $\distribution \sim U_{n}$ is the uniform distribution, output $\accept$.
        \item (Soundness) If $\tvd{\distribution, U_n} \geq \varepsilon$ is $\varepsilon$-far from uniform, output $\reject$.
    \end{enumerate}
\end{definition}

\input{inputs/uniformity_testing_algorithm}

\input{inputs/uniformity_testing_lower_bound}


==> inputs/uniformity_testing_algorithm.tex <==
\subsection{A Replicable Uniformity Testing Algorithm}

We present our algorithm for uniformity testing.

\thmruniformitytester

Our algorithm has worst case sample complexity that incurs an additional $\frac{1}{\rho}$ factor on the sample complexity for known non-replicable results for uniformity testing.
To the best of our knowledge, this is the first replicable algorithm for distribution testing that has linear dependence on the replicability parameter in the worst case.

\paragraph{Algorithm Overview}
Our algorithm follows the uniformity tester of \cite{DBLP:conf/icalp/DiakonikolasGPP18}.
At a high level, the algorithm computes a test statistic: the total variation distance between the empirical distribution and the uniform distribution.
While the expectation gap in the test statistic follows from \cite{DBLP:conf/icalp/DiakonikolasGPP18}, we require different analysis in bounding the concentration of the test statistic.
Since a replicable algorithm must consistently handle arbitrary distributions, it is no longer possible to assume a certain structure on the worst-case distribution.
However, we show that when the variation of the test statistic is too large (Case 2.1), even if the input distribution itself is not in the soundness regime, the test statistic is with high probability in the soundness regime, leading the algorithm to replicably reject samples drawn from the input distribution.
This leads to sufficiently strong concentration in the test statistic, so that a randomly chosen threshold does not land between empirical test statistics computed from independent samples.

\IncMargin{1em}
\begin{algorithm}

\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}\SetKwInOut{Parameters}{Parameters}
\Input{Sample access $S$ to distribution $\distribution$ on domain $[n]$}
\Parameters{$\varepsilon$ tolerance, $\rho$ replicability, and $\delta$ accuracy}
\Output{$\accept$ if $\distribution \sim U_{n}$ is uniform, $\reject$ if $\tvd{\distribution, U_{n}} \geq \varepsilon$}

$m \gets \bigTh{\frac{\sqrt{n}}{\rho \varepsilon^2} \sqrt{\log \frac{n}{\delta}} + \frac{1}{\rho^2 \varepsilon^2}}$

\For{$1 \leq i \leq m' \gets \bigTh{\log 1/\delta}$}{
    $D_i$ gets $m$ samples from $\distribution$
    
    $S_i \gets \frac{1}{2} \sum_{i = 1}^{n} \left| \frac{X_i}{m} - \frac{1}{n} \right|$ where $X_i$ is the frequency of $i \in [n]$ in $D$
}

$S_{median} \gets $ median of $\set{S_i}$

$\mu(U_n)$ is expectation of $\frac{1}{2} \sum_{i = 1}^{n} \left| \frac{X_i}{m} - \frac{1}{n} \right|$ under uniform distribution

$r_0 \gets \UnifD{\frac{1}{4}, \frac{3}{4}}$

Set threshold $r \gets \mu(U_n) +  r_0 \cdot C \cdot \begin{cases}
    \varepsilon^2 \frac{m^2}{n^2} & m \leq n \\
    \varepsilon^2 \sqrt{\frac{m}{n}} & n < m \leq \frac{n}{\varepsilon^2} \\
    \varepsilon & \frac{n}{\varepsilon^2} < m
\end{cases}$ ($C$ given by Lemma \ref{lemma:uniformity-expectation-gap})

\If{$S_{median} < r$}{
    \Return $\accept$
}\Else{
    \Return $\reject$
}

\caption{$\rUniformityTester(\distribution, \varepsilon, \rho, \delta)$} 
\label{alg:r-uniformity-tester}

\end{algorithm}
\DecMargin{1em}

Note that $\mu(U_n)$ can be computed efficiently as shown in \cite{DBLP:conf/icalp/DiakonikolasGPP18}, so that the given algorithm is computationally efficient.
We begin with a few useful lemmas.
First, we use an expectation gap in the test statistic to ensure that the algorithm outputs $\reject$ in the soundness case.

\begin{lemma}[Lemma 4 of \cite{DBLP:conf/icalp/DiakonikolasGPP18}]
    \label{lemma:uniformity-expectation-gap}
    Let $\distribution$ be a distribution on $[n]$ such that $\varepsilon = \tvd{\distribution, U_{n}}$.
    For any distribution $\distribution$, let $\mu(\distribution) = \Ep_{\distribution^{m}}[S]$ denote the expectation of the test statistic $S = \frac{1}{2} \sum_{i = 1}^{n} \left| \frac{X_i}{m} - \frac{1}{n} \right|$ given $m$ samples drawn from $\distribution$.
    For all $m \geq 6, n \geq 2$, there is a constant $C$ such that,
    \begin{equation*}
        \mu(\distribution) - \mu(U_n) \geq C \cdot \begin{cases}
            \varepsilon^2 \frac{m^2}{n^2} & m \leq n \\
            \varepsilon^2 \sqrt{\frac{m}{n}} & n < m \leq \frac{n}{\varepsilon^2} \\
            \varepsilon & \frac{n}{\varepsilon^2} \leq m
        \end{cases}
    \end{equation*}
\end{lemma}

\subsubsection*{Concentration of the Test Statistic}

Next, we show that after taking $m$ samples for sufficiently large $m$, the test statistic is concentrated around its expectation $\mu(\distribution) = \Ep_{\distribution}[S]$.
Suppose we take $m$ i.i.d. samples from $\distribution$.
Let $T_{1}, \dotsc, T_{m}$ be random variables representing each sample.
Denote $X = \set{X_1, \cdots X_n}$ to be the histogram of samples where $X_i$ denotes the empirical frequency of $i$.
We proceed by case analysis.

\subsubsection*{Case 1: $m \geq n$}

We bound the concentration of $S$ when $m \geq n$ with McDiarmid's Inequality.

\begin{theorem}[McDiarmid's Inequality]
    \label{thm:mcdiarmid}
    Let $X_1, \dotsc, X_n$ be independent random variables taking values in $\domain$.
    Let $f: \domain^{n} \mapsto \R$ be a function such that for all pairs of tuples $(x_1, \dotsc, x_n), (x_1', \dotsc x_n') \in \domain^{n}$ such that $x_i = x_i'$ for all but one $j \in [n]$, 
    \begin{equation*}
        \left|f(x_1, \dotsc, x_n) - f(x_1', \dotsc, x_n')\right| \leq B
    \end{equation*}
    Then, 
    \begin{equation*}
        \Pr \left( \left|f(X_1, \dotsc, X_n) - \E{f(X_1, \dotsc, N_n)}\right| \geq t \right) < 2 \exp \left( - \frac{2 t^2}{n B^2} \right)
    \end{equation*}
\end{theorem}

Observe that the samples $T_j$ are independent and a change in $T_j$ changes $S$ by at most $\frac{1}{m}$, since at most two values $X_i$ change by at most $\frac{1}{2m}$ each.
Then, Theorem \ref{thm:mcdiarmid} implies that,
\begin{equation*}
    \Pr\left( |S - \E{S}| \geq t \right) < 2 \exp \left( - \frac{2 m^2 t^2}{n} \right) < 2 \exp \left( - 2 m t^2 \right)
\end{equation*}

When $n \leq m \leq \frac{n}{\varepsilon^2}$, we can conclude,
\begin{equation*}
    \Pr\left( |S - \E{S}| \geq \rho \cdot \frac{C}{16} \cdot \varepsilon^2 \sqrt{\frac{m}{n}} \right) < 2 \exp \left( - 2 m t^2 \right) < \frac{1}{10}
\end{equation*}
whenever $m \geq \bigTh{\frac{\sqrt{n}}{\rho \varepsilon^2}}$.

Otherwise, $n \geq \frac{n}{\varepsilon^2}$ and,
\begin{equation*}
    \Pr\left( |Z - \E{Z}| \geq \rho \cdot \frac{C}{16} \cdot \varepsilon \right) < 2 \exp \left( - 2 m t^2 \right) < \frac{1}{10}
\end{equation*}
whenever $m \geq \bigTh{\frac{1}{\rho^2 \varepsilon^2}}$.

We now claim that $S_{median}$ is within $\frac{C}{16} \varepsilon^2 \frac{m^2}{n^2}$ of $\mu(\distribution) = \E{Z}$.
Note that the median does not satisfy the condition only if at least half of the intermediate statistics $Z$ do not satisfy the condition.
By a Chernoff bound, this occurs with probability at most $\delta$ if $m' \geq \bigTh{\log \frac{1}{\delta}}$.

\subsubsection*{Case 2: $m \leq n$}

We now consider the sublinear case.
Following an observation by \cite{DBLP:conf/icalp/DiakonikolasGPP18}, we rewrite the test statistic,
\begin{equation*}
    S = \frac{1}{2} \sum_{i = 1} \left| \frac{X_i}{m} - \frac{1}{n} \right| = \frac{1}{2} \sum_{i = 1} \frac{X_i}{m} - \frac{1}{n} + \frac{2}{n} \cdot \ind{X_i = 0} = \frac{1}{n} \abs{\set{i \given X_i = 0}}
\end{equation*}
where we define the random variable $Z = \abs{\set{i \given X_i = 0}}$.

Our goal now is to bound the variance of $Z$.
For each $k \in [n]$, let $b_k = \ind{\distribution(k) \geq \unifheavythreshold}$ indicate whether $k$ is a ``heavy" or ``light" element in the distribution $\distribution$.
We define the random variables $Y_1, \dotsc, Y_m$ to indicate where the $i$-th sample collides with any samples $j$ before it, i.e. $j < 1$.
Furthermore, we define $\tilde{Y}_1, \dotsc, \tilde{Y}_m$ to indicate $Y_i = 1$ and $Y_i = k$ for some $k \in [n]$ such that $b_k = 0$.
Observe that $\Pr(\tilde{Y}_i = 1) \leq \Pr(Y_i = 1)$.
Finally, let $H$ denote the number of samples falling into a bucket where $b_k = 1$.
Then, we obtain the identities,
\begin{align*}
    Z &= n - m + \sum_{i = 1}^{Y_i} = Z_H + Z_L \\
    Z_H &= \abs{\set{i \text{ such that } X_i = 0 \andT b_i = 1 }}\\
    Z_L &= \abs{\set{i \text{ such that } X_i = 0 \andT b_i = 0 }} = n - m + H + \sum_{i = 1}^{m} \tilde{Y}_{i}
\end{align*}

where we define $Z_H, Z_L$ to be the parts of $Z$ of heavy and light elements respectively.
We will bound the variance of $Z_H, Z_L$ separately.
First, we note that $Z_H = 0$ with high probability.
In particular, the probability that an element with $b_k = 1$ does not occur in $m$ samples is at most $(1 - \distribution(x))^{m} < \left(\frac{\delta}{10n}\right)^2$, so that the probability that some heavy element does not occur is at most $\frac{\delta^2}{100 n}$.
We therefore condition on $Z_H = 0$, so that $\Var(Z_H) = 0$.

To bound the concentration of $Z_L$, we separately bound the variance of $H$ and $\sum_{i = 1}^{m} \tilde{Y}_{i}$.
We begin with the first term, beginning with an upper bound on the expectation of $H$.
We show the expected number of ``heavy" elements is at most a constant multiple of the expected number of collisions.

\begin{lemma}
    \label{lemma:heavy-distribution-ub}
    Let $H$ denote the number of samples falling into a bucket where $b_k = 1$.
    \begin{equation*}
        4 \sum_{i = 1}^{m} \E{Y_i} \geq m \sum_{b_k = 1} \distribution(k) = \E{H} \geq \Var(H)
    \end{equation*}
\end{lemma}

\begin{proof}[Proof of Lemma \ref{lemma:heavy-distribution-ub}]
    Note that $H$ is a binomial random variable so that its expectation is an upper bound on its variance.
    Since the $Y_i$ are non-negative random variables and $\E{Y_i}$ is an increasing sequence, it suffices to show the following lower bound.
    \begin{equation*}
         4 \sum_{i = 1}^{m} \E{Y_i} \geq 4 \sum_{i = m/2}^{m} \E{Y_i} \geq 2 m \E{Y_{m/2}} \geq m \sum_{b_k = 1} \distribution(k)
    \end{equation*}
    or equivalently,
    \begin{equation*}
        \E{Y_{m/2}} = \Pr(Y_{m/2} = 1) \geq \frac{1}{2} \sum_{b_k = 1} \distribution(k)
    \end{equation*}
    Consider an element $k$ such that $b_k = 1$ or equivalently $\distribution(k) \geq \unifheavythreshold$.
    Then, the probability that $k$ does not occur in the first $m/2$ samples is at most $\frac{\delta}{10 n}$.
    Union bounding over at most $n$ elements, each element with $b_k = 1$ occurs in the first $\frac{m}{2}$ samples with probability at least $1 - \frac{\delta}{10} \geq \frac{9}{10}$.
    Conditioned on this, $\Pr(Y_{m/2} = 1) \geq \sum_{b_k = 1} \distribution(k)$ so that we conclude,
    \begin{equation*}
        \Pr(Y_{m/2} = 1) \geq \frac{1}{2} \sum_{b_k = 1} \distribution(k)
    \end{equation*}
\end{proof}

Now, we move on to the term $\sum_{i = 1}^{m} \tilde{Y}_i$.
Using linearity of expectation, we have

\begin{align*} 
\E{ \left( \sum_{i=1}^m \tilde{Y}_i \right)^2 } = \sum_{i=1}^m \E{ \tilde{Y}_i^2 } + \sum_{i \neq j} \E{ \tilde{Y}_i \tilde{Y}_j }
\end{align*}

For the first term, $\E{\tilde{Y}_i^2} = \E{\tilde{Y}_i}$ since $\tilde{Y}_i$ is an indicator variable. 
Considering the second term, we introduce the variables $Z_{i,j}$ denoting whether the $i$-th and $j$-th samples collide, i.e. $Z_{i, j} = \ind{T_i = T_j}$.
We can write
\begin{align*}
\Pr( \tilde{Y}_i \tilde{Y}_j = 1 ) = \Pr( \tilde{Y}_i \tilde{Y}_j = 1 , Z_{i,j} = 1) + \Pr( \tilde{Y}_i \tilde{Y}_j = 1 , Z_{i,j} = 0)
\end{align*}

We now bound the first term.

\begin{lemma}
    \label{lemma:i-j-same-collision-ub}
    Let $Y_i$ denote the event that the $i$-th sample collides with a previous sample.
    Let $\tilde{Y}_i$ denote the event $Y_i = 1$ and the $i$-th sample falls in a bucket with $b_k = 0$.
    Let $Z_{i, j}$ denote the event the $i$-th and $j$-th sample fall in the same bucket.
    Then,
    \begin{equation*}
        \sum_{i \neq j} \Pr(\tilde{Y}_i \tilde{Y}_j Z_{i, j} = 1) \leq 2 \log \frac{10 n}{\delta} \sum_{i = 1}^{m} \E{\tilde{Y}_i} \leq 2 \log \frac{10 n}{\delta} \sum_{i = 1}^{m} \E{Y_i}
    \end{equation*}
\end{lemma}

\begin{proof}[Proof of Lemma \ref{lemma:i-j-same-collision-ub}]
    The event $\tilde{Y}_i, \tilde{Y}_j = 1, Z_{i,j} = 0$ happens when there is some element $k \in [n]$ such that,
    \begin{enumerate}
        \item $b_k = 0$
        \item both samples $S_i = S_j = k$
        \item some samples from $S_{< i}$ fall in $k$. We denote this event as $E_{i,k}$.
    \end{enumerate}
    We compute as follows,
    \begin{align*}
        \Pr(\tilde{Y}_i \tilde{Y}_j Z_{i, j} = 1) &= \sum_{b_k = 0} \Pr(E_{i, k}) \Pr(S_i = k) \Pr(S_j = k) \\
        &= \sum_{b_k = 0} \Pr(E_{i, k} = 1) \distribution(k)^2 \\
        &\leq \unifheavythreshold \sum_{b_k = 0} \distribution(k) \Pr(E_{i, k} = 1) \\
        &= \unifheavythreshold \E{\tilde{Y}_i}
    \end{align*}
    where in the inequality we have used $b_k = 0$ gives an upper bound on $\distribution(k)$.
    Then, for each $i$ we sum over $m - 1 \leq m$ indices $j \neq i$ to conclude the proof.
\end{proof}

For the second term, we argue it can be upper bounded by $\Pr(\tilde{Y}_i = 1) \Pr(\tilde{Y}_j = 1)$ with Kleitman’s Lemma.

\begin{lemma}[Kleitman's Lemma~\cite{alon2016probabilistic}]
\label{lemma:kleitman}
Let $Q$ be a product distribution over random bit strings $\{0, 1, 2\}^n$.
Let $\mathcal A, \mathcal B$ be two indicator functions of events about $Q$ such that $\mathcal A$ is non-decreasing in each coordinate and $\mathcal B$ is non-increasing in each coordinate. Then, it holds

\begin{equation*}
    \Pr \left( \mathcal A(Q) \mathcal B(Q) \right) \leq \Pr \left( \mathcal A(Q) \right) \Pr \left( \mathcal B(Q) \right)
\end{equation*}

\end{lemma}

\begin{lemma}
\label{lemma:collision-correlation-inequality}
For $i \neq j$, we have $\Pr( \tilde{Y}_i \; \tilde{Y}_j = 1 , Z_{i,j} = 0) \leq \Pr(\tilde{Y}_i = 1) \Pr(\tilde{Y}_j = 1)$
\end{lemma}

\begin{proof}[Proof of Lemma \ref{lemma:collision-correlation-inequality}]
Without loss of generality, we assume $i < j$.
We will use $S_{< x} = (S_1, \dotsc, S_{x - 1})$ to denote the set of samples ranging from $1$ to $x-1$.

The event $\tilde{Y}_i \; \tilde{Y}_j = 1 , Z_{i,j} = 0$ happens when there exists two distinct elements $k \neq  \ell \in [n]$ such that 

\begin{enumerate}
    \item the $i$-th sample is $S_i = k$, the $j$-th sample is $S_j = \ell$ 
    \item some samples from $S_{< i}$ fall in $k$, some samples from $S_{< j}$ fall in $\ell$. We denote the two events as $E_{i,k}$ and $E_{j, \ell}$ respectively.
\end{enumerate}

Hence, we can write

\begin{align} 
\label{eq:prob-decomposition}
\Pr[ \tilde{Y}_i \; \tilde{Y}_j = 1 , Z_{i,j} = 0 ]    
= \sum_{k \neq \ell, b_k = b_{\ell} = 0} \Pr[  E_{i,k}, E_{j, \ell}   ] \; p_k \; p_{\ell}
\end{align}

Fix a pair of $k  < \ell$.
Consider the string $\beta^{(k, \ell)}$ such that $\beta^{(k, \ell)}_i = 1$ if the $i$-th sample falls in the $k$-th bucket, $\beta^{(k, \ell)}_i = 2$ if the $i$-th sample fall in neither $k$-th nor $\ell$-th bucket, 
$\beta^{(k, \ell)}_i = 3$ if the $i$-th sample falls in the $\ell$-th bucket.
Then, both $E_{i, k}, E_{j, \ell}$ are completely determined by the string $\beta^{(k, \ell)}$.
Moreover, $E_{i, k}$ is monotonically decreasing in each coordinate and $E_{j, \ell}$ is monotonically increasing in each coordinate.
As a result, we have

\begin{equation*}
    \Pr(E_{i, k} E_{j, \ell}) \leq \Pr(E_{i, k}) \Pr(E_{j, \ell})
\end{equation*}

Substituting this into Equation~\eqref{eq:prob-decomposition} then gives us
\begin{align*}
    \Pr(\tilde{Y}_i \tilde{Y}_j = 1, Z_{i,j = 0})
    &\leq \sum_{k \neq \ell} \Pr(E_{j,\ell}) \Pr(E_{i,k}) p_{k} \; p_{\ell} \\
    &\leq \left(  \sum_{k} \Pr(E_{i,k}) p_{k} \right) \; \left(  \sum_{\ell} \Pr(E_{j,\ell}) p_{\ell} \right) \\
    &\leq \Pr(\tilde{Y}_i = 1) \Pr(\tilde{Y}_j = 1)
\end{align*}
\end{proof}

To bound the total contribution to the variance of the second term, we sum and obtain,
\begin{equation*}
    \sum_{i \neq j} \Pr(\tilde{Y}_i \tilde{Y}_j = 1, Z_{i,j = 0}) \leq \sum_{i \neq j} \E{\tilde{Y}_i} \E{\tilde{Y}_j}  
\end{equation*}

Note that the contribution $\sum_{i \neq j} \E{\tilde{Y}_i}\E{\tilde{Y}_j}$ is at most $\E{\sum \tilde{Y}_i}^2$, so that it does not factor into the variance of $\sum \tilde{Y}_i$.
In particular,
\begin{equation*}
    \Var \left( \sum \tilde{Y}_i \right) \leq 2 \log \frac{10n}{\delta} \sum \E{Y_i}
\end{equation*}

We thus obtain the following bound on the variance of $Z$.

\begin{lemma}
    \label{lemma:z-variance-bound}
    Recall $Z = \abs{\set{i \given X_i = 0}}$ where $X_i$ is the frequency of $i$ in a sample of size $m$.
    Let $Z_H$ (resp. $Z_L$) be $\abs{\set{i \given X_i = 0, b_i = 1}}$ (resp. $\abs{\set{i \given X_i = 0, b_i = 0}}$) where $b_i$ indicates $\distribution(i) \geq \unifheavythreshold$.
    Conditioned on $Z_H = 0$, we have,
    \begin{equation*}
        \Var(Z) \leq 24 \log \frac{10n}{\delta} \sum_{i = 1}^{m} \E{Y_i}
    \end{equation*}
\end{lemma}

\begin{proof}[Proof of Lemma \ref{lemma:z-variance-bound}]
    Since $Z_H = 0$, we have,
    \begin{align*}
        \Var(Z) &= \Var(Z_L) \\
        &\leq 4 \left(\Var(H) + \Var\left(\sum_{i = 1}^{m} \tilde{Y}_i\right)\right) \\
        &\leq 16 \sum_{i = 1}^{m} \E{Y_i} + 8 \log \frac{10n}{\delta} \sum_{i = 1}^{m} \E{Y_i} \\
        &\leq 24 \log \frac{10n}{\delta} \sum_{i = 1}^{m} \E{Y_i}
    \end{align*}
\end{proof}

We now consider two sub-cases.

\subsubsection*{Case 2.1: Many Collisions --- \texorpdfstring{$\sum_{i = 1}^{m} \E{Y_i} \geq \collisionexpectationthreshold$}{}}

We argue that when there are many collisions, the algorithm replicably outputs $\reject$.
First, let us consider the expectation of the test statistic if the input distribution is uniform.

\begin{lemma}
    \label{lemma:uniform-test-statistic-exp}
    Let $\mu(U_n)$ be the expectation of $S$ given a sample from $U_n$.
    \begin{equation*}
        n \cdot \mu(U_n) \leq n - m + \frac{m^2}{n}
    \end{equation*}
\end{lemma}

\begin{proof}[Proof of Lemma \ref{lemma:uniform-test-statistic-exp}]
    For each $i$, note that there are at most $m$ distinct elements sampled before the $i$-th sample.
    In particular, $\E{Y_i} \leq \frac{m}{n}$.
    We conclude with the identity $\E{Z} = n - m + \sum_{i = 1}^{m} \E{Y_i}$.
\end{proof}

Now, we show that with probability at least $\frac{9}{10}$, $S \geq \mu(U_n) + C \cdot \varepsilon^2 \frac{m^2}{n^2}$.
The expectation of $Z$ is,
\begin{equation*}
    \E{Z} = n - m + \sum_{i = 1}^{m} \E{Y_i}
\end{equation*}

From Lemma \ref{lemma:z-variance-bound}, we have $\Var(Z) = \bigtO{\sum_{i = 1}^{m} \E{Y_i}}$.
By Chebyshev's inequality, we have that,
\begin{equation*}
    \Pr\left(Z < \E{Z} - \sqrt{10 \Var(Z)}\right) < \frac{1}{10}
\end{equation*}

Therefore, it suffices to show $\E{Z} - \sqrt{10 \Var(Z)} \geq n \cdot \mu(U_n) + C \frac{m^2}{n}$ where the constant $C$ is given by Lemma \ref{lemma:uniformity-expectation-gap}.
If this holds, then with probability at least $\frac{9}{10}$, $S$ is beyond the random threshold.
From Lemma \ref{lemma:z-variance-bound}, we have,
\begin{align*}
    \sqrt{\Var(Z)} &\leq \sqrt{24 \log \frac{10n}{\delta} \sum_{i = 1}^{m} \E{Y_i}}
\end{align*}
Then, to ensure $\E{Z} - \sqrt{10 \Var(Z)} \geq n \cdot \mu(U_n) + C \frac{m^2}{n}$,
\begin{align*}
    \sum_{i = 1}^{m} \E{Y_i} &\geq C \cdot \frac{m^2}{n} + \sqrt{240 \log \frac{10n}{\delta} \sum_{i = 1}^{m} \E{Y_i}} \\
    \sum_{i = 1}^{m} \E{Y_i} &\geq \max \left( 2 C \frac{m^2}{n}, 2 \sqrt{240 \log \frac{10n}{\delta} \sum_{i = 1}^{m} \E{Y_i}} \right) \\
    &= 2 C \frac{m^2}{n}
\end{align*}
for $m = \bigTh{\frac{\sqrt{n}}{\rho \varepsilon^2} \sqrt{\log \frac{n}{\delta}}}$.
Note that our choice of $\collisionexpectationthreshold$ is large enough.

\subsubsection*{Case 2.2: Few Collisions --- \texorpdfstring{$\sum_{i = 1}^{m} \E{Y_i} \leq \collisionexpectationthreshold$}{}}

Following Lemma \ref{lemma:z-variance-bound}, we obtain an upper bound on the variance of $S = \frac{Z}{n}$,
\begin{align*}
    \Var(Z) &\leq 24 \log \frac{10n}{\delta} \sum_{i = 1}^{m} \E{Y_i} \\
    &= \bigO{\frac{m^2}{n} \log \frac{n}{\delta} } \\
    \Var(S) &= \bigO{\frac{m^2}{n^3} \log \frac{n}{\delta}}
\end{align*}

By Chebyshev's inequality,
\begin{equation*}
    \Pr \left( |S - \mu(\distribution)| > C' \frac{m}{n^{3/2}} \right) < \frac{1}{10}
\end{equation*}
for some appropriately large constant $C'$.
In order to obtain the desired concentration, we require,
\begin{equation*}
    C' \frac{m}{n^{3/2}} \leq \rho \cdot \frac{C}{16} \cdot \varepsilon^2 \frac{m^2}{n^2}
\end{equation*}
which is satisfied by our choice of $m$,
\begin{equation*}
    m \geq \bigTh{\frac{\sqrt{n}}{\rho \varepsilon^2} \sqrt{\log \frac{n}{\delta}}}
\end{equation*}

Our above discussions yield the following structural lemma on the concentration of $S$.

\begin{lemma}
    \label{lemma:uniformity-test-statistic-concentration}
    Let $\distribution$ be a distribution over $[n]$ and $S_{median}$ the statistic obtained in Algorithm \ref{alg:r-uniformity-tester}.
    Then,
    \begin{enumerate}
        \item {\bf Sublinear Case: $m \leq n$}
        
        If $\sum_{i} \E{Y_i} \geq \collisionexpectationthreshold$, then $S_{median} < \mu(U_n) + C \frac{m^2}{n^2}$ with probability at most $\frac{\delta}{2}$.
        
        Otherwise, $|S_{median} - \mu(\distribution)| > \rho \cdot \frac{C}{16} \cdot \varepsilon^2 \frac{m^2}{n^2}$ with probability at most $\frac{\delta}{2}$.
        
        \item {\bf Superlinear Case: $n < m$}

        If $m < \frac{n}{\varepsilon^2}$, then $|S_{median} - \mu(\distribution)| > \rho \cdot \frac{C}{16} \cdot \varepsilon^2 \sqrt{\frac{m}{n}}$ with probability at most $\frac{\delta}{2}$.

        Otherwise, $m \geq \frac{n}{\varepsilon^2}$ and $|S_{median} - \mu(\distribution)| > \rho \cdot \frac{C}{16} \cdot \varepsilon$ with probability at most $\frac{\delta}{2}$.
    \end{enumerate}
\end{lemma}

\begin{proof}
    We begin with the sublinear case $m \leq n$.
    First, suppose $\sum_{i} \E{Y_i} \geq \collisionexpectationthreshold$.
    Then, $S_{median} < \mu(U_n) + C \frac{m^2}{n^2}$ with probability at most $\frac{\delta}{2}$ only if $S_i < \mu(U_n) + C \frac{m^2}{n^2}$ for more than half of $i \leq m'$.
    This occurs with probability at most $\frac{\delta}{2}$ by our choice of $m'$.

    For the remaining cases, observe that we have shown $S \in (\mu(\distribution) - \tau, \mu(\distribution) + \tau)$ with probability at least $\frac{9}{10}$.
    $S_{median} \not\in (\mu(\distribution) - \tau, \mu(\distribution) + \tau)$ implies that half of the $S_i$ do not fall within this interval.
    This occurs with probability at most $\frac{\delta}{2}$ by our choice of $m'$ and a Chernoff bound.
\end{proof}

\begin{proof}[Proof of Correctness of Algorithm \ref{alg:r-uniformity-tester}]
    Recall that we condition on $Z_H = 0$, with occurs with $1 - \frac{\delta}{2}$ probability.
    
    We begin with the uniform distribution.
    Note that $\E{Y_i} \leq \frac{m}{n}$ so that by Lemma \ref{lemma:uniformity-test-statistic-concentration}, $S_{median} \leq \mu(U_n) + \frac{C}{16} \varepsilon^2 \frac{m^2}{n^2}$ with probability at least $1 - \frac{\delta}{2}$.
    In particular, since the random threshold $r > \mu(U_n) + \frac{C}{4} \varepsilon^2 \frac{m^2}{n^2}$, the algorithm outputs $\accept$.
    
    Now, suppose $\tvd{\distribution, U_n} \geq \varepsilon$.
    If $m \leq n$ and $\sum_{i} \E{Y_i} \geq \collisionexpectationthreshold$ then $S_{median} \geq \mu(U_n) + C \varepsilon^2 \frac{m^2}{n^2}$ with probability at least $1 - \frac{\delta}{2}$.
    Since the random threshold $r < \mu(U_n) + \frac{3 C}{4} \varepsilon^2 \frac{m^2}{n^2}$, the algorithm outputs $\reject$.
    Otherwise, by Lemma \ref{lemma:uniformity-test-statistic-concentration}, $S_{median} \geq \mu(U_n) + \frac{15C}{16} \varepsilon^2 \frac{m^2}{n^2}$ with probability at least $1 - \frac{\delta}{2}$.
    In particular, since the random threshold $r < \mu(U_n) + \frac{3 C}{4} \varepsilon^2 \frac{m^2}{n^2}$, the algorithm outputs $\reject$.
\end{proof}

\begin{proof}[Proof of Replicability of Algorithm \ref{alg:r-uniformity-tester}]
    Consider two executions of the algorithm.
    If $\mu(\distribution)$ is uniform or $\tvd{\distribution, U_{n}} \geq \varepsilon$, then following a union bound two executions of the algorithm output different values with probability at most $2 \delta$.
    
    Then, suppose $m \leq n$ and $\sum_{i} \E{Y_i} \geq \collisionexpectationthreshold$.
    By our above arguments, both samples lead the algorithm to output $\reject$ with probability at least $1 - 2 \delta$ so that the algorithm is $\rho$-replicable.

    Otherwise, let $R$ denote the expectation gap given by Lemma \ref{lemma:uniformity-expectation-gap}.
    Our concentration bounds show that with probability at most $2 \delta < \frac{\rho}{2}$, we have $|S_{median} - \mu(\distribution)| \leq \rho \frac{R}{16}$ over both samples.
    In particular, whenever the random threshold $r$ does not fall in the interval $(\mu(\distribution) - \frac{\rho R}{16}, \mu(\distribution) + \frac{\rho R}{16})$, both executions output the same result.
    Since $r$ is chosen uniformly at random, this occurs with probability at most $\frac{\rho}{2}$.
    By a union bound, we observe that Algorithm \ref{alg:r-uniformity-tester} is $\rho$-replicable.
\end{proof}

\begin{proof}[Proof of Sample Complexity of Algorithm \ref{alg:r-uniformity-tester}]
    The sample complexity is immediately obtained by our values of $m \cdot m'$.
\end{proof}

==> inputs/uniformity_testing_lower_bound.tex <==
\subsection{Lower Bound for Uniformity Testing}

We now give a matching lower bound (up to polylogarithmic factors) for a $\rho$-replicable uniformity tester.

\newcommand{\epsa}{\varepsilon_0}
\newcommand{\epsb}{\varepsilon_1}

\runiformitytesterlb

\paragraph{Proof Overview}

\chris{Sihan?}

\begin{proof}
    Let $\domain$ be a finite domain of $n$ elements and $\distribution$ a distribution on $\domain$.
    For a given $\eps > 0$, consider the following family of measures $T_{\eps}$ on $\domain$.
    Every $x \in \domain$ is given measure $\frac{1 + \eps}{n}$ and $\frac{1 - \eps}{n}$ with equal probability.
    Note that with high probability, the total measure of a distribution chosen from $T_{\eps}$ is close to 1.
    
    Let $\innerAlg$ be an algorithm requiring $m$ samples. 
    Let $S_{\eps}$ denote $m$ samples drawn independently from a distribution chosen from $T_{\eps}$.
    Then, by Markov's inequality, with probability at least $\frac{1}{4}$ a random string $r$ satisfies:
    \begin{enumerate}
        \item $\Pr(\innerAlg(S_{0}; r) = 1) < \delta$ so that $\Pr_r(\Pr_{S_{0}}(\innerAlg(S_{0}; r) = 1) > 4 \delta) < \frac{1}{4}$.
        \item $\Pr(\innerAlg(S_{\eps}; r) = 1) < \delta$ so that $\Pr_r(\Pr_{S_{\eps}}(\innerAlg(S_{\eps}; r) = 1) > 4 \delta) < \frac{1}{4}$.
        \item Let $x \in (0, \eps)$ and $S_{x}, S'_{x}$ be two independent samples drawn from a distribution chosen from $T_x$. 
        Then, $\Pr_{r}(\Pr_{S_{x}, S'_{x}}(\innerAlg(S_{x}; r) \neq \innerAlg(S'_{x}; r)) > 4 \rho) < \frac{1}{4}$.
    \end{enumerate}
    
    By the union bound, at least $\frac{1}{4}$ of random strings satisfy the above conditions.
    We call such random strings {\bf good}.
    Fix some {\bf good} random string $r$ on which $\innerAlg$ is correct and $\rho$-replicable.
    In the following, assume we execute $\innerAlg$ with a fixed random string $r$.

    Then, fix arbitrary $0 \leq \epsa \leq \epsb \leq \eps$ and $\delta = \epsb - \epsa$.
    The sample distribution on $\domain$ is determined first by drawing $X \sim \set{0, 1}$ uniformly, and then defining a distribution on $\domain$ by choosing one from $T_{\eps_{X}}$.

    We claim that for small enough $\delta$, it is difficult to identify $X$ when given samples from such a distribution.
    Consider the following reduction that converts a uniformity tester $\innerAlg$ into an algorithm $\outerAlg$ that correctly guesses $X$ with probability at least 51\%.
    Let $A_{b}$ denote the probability that $\innerAlg$ outputs 1 when given a sample drawn from the distribution where $X = b$.
    In particular, by running $\innerAlg$ on $\bigO{\frac{1}{|A_0 - A_1|^2}}$ independent samples we have an algorithm $\outerAlg$ with sample complexity $\bigO{\frac{k}{|A_0 - A_1|^2}}$ that can guess $X$ with probability at least 51\%.
    
    We may now turn our attention towards lower bounding the sample complexity of such an algorithm. 
    Let $M_x$ denote the random variable representing the number of occurrences of $x \in \domain$ in a sample $S$ drawn from this distribution, and $M = (M_x)_{x \in \domain}$.
    Since conditioned on $X$, $M_x$ are mutually independent, we can upper bound,
    \begin{equation*}
        I(X:M) \leq \sum_{x \in \domain} I(X: M_x) = \bigO{\eps^2 \delta^2 \frac{k^2}{n}}
    \end{equation*}

    In particular, for any constant $c_0$ and $\delta \leq \frac{c_0 \sqrt{n}}{k \eps}$, we have $I(X:M) = O(1)$.
    Notice for small enough choice of $c_0$, $I(X:A) < 2 \cdot 10^{-4}$ so that $f$ fails to guess $X$ with probability at least 51\% by Lemma \ref{lemma:alg-mutual-info-lower-bound}.
    Therefore, for such small $\delta$ we may upper bound $|f_0 - f_1| = O(1)$.

    Above we have established that up to some threshold of $\delta$, the acceptance probability of our algorithm cannot change significantly. 
    We will now use this to lower bound the sample complexity of a replicable algorithm.
    For any $x \in [0, \eps]$, let $f_x$ denote the probability that $\innerAlg$ accepts when given a sample drawn from a distribution chosen from $T_{x}$. 
    Then, by the correctness of $\innerAlg$, $f_0 < \frac{1}{4}$ and $f_{\eps} > \frac{3}{4}$.
    Furthermore, I claim that $f_x$ is a continuous function with respect to $x$.
    In particular, we may write the acceptance probability as,
    \begin{equation*}
        f_x = \sum_{s} \Pr(S = s) \innerAlg(s; r) = \frac{1}{\sum_{s} \prod_{i = 1}^{k} \left( \frac{1 \pm x}{n} \right)} \sum_{s} \innerAlg(s; r) \prod_{i = 1}^{k} \left( \frac{1 \pm x}{n} \right) 
    \end{equation*}
    which is continuous with respect to $x$.
    Thus, there is some $x^*$ for which $f_{x^*} = \frac{1}{2}$.
    Then, by our above arguments, for all $y \in [x - \delta, x + \delta]$, we have that $f_y \in \left( \frac{1}{3}, \frac{2}{3} \right)$.
    In particular, by choosing $y$ randomly from $[0, \eps]$, replicability implies that,
    \begin{align*}
        \frac{c_0 \sqrt{n}}{k \eps} \frac{1}{\eps} \leq \rho
    \end{align*}
    so that,
    \begin{equation*}
        k = \bigOm{\frac{\sqrt{n}}{\rho \eps^2}}
    \end{equation*}
    proving the desired lower bound.
\end{proof}

\begin{lemma}
    \label{lemma:cdvv-distinguishability}
    (Proposition 11 of \cite{CDVV14closeness})
    For any $b \in [0, 1]$ and $\eps < \sqrt{b}$, there exists a distribution $p_b$ and a family of distributions $T_{p, \eps}$ such that for a $q$ drawn from $T_{p, \eps}$ uniformly at random, the following hold:
    \begin{enumerate}
        \item $\norm{p}{2}^2 \in \left[\frac{b}{2}, b\right]$ and $\max_i p_i \in \left[\frac{b}{2}, b\right]$ and with probability at least $1 - o(1)$, $\norm{q}{2}^2 \in \left[\frac{b}{2}, b\right]$ and $\max_i q_i \in \left[\frac{b}{2}, b\right]$ 

        \item With probability at least $1 - o(1)$, $\norm{p - q}{2} \geq \frac{\eps}{2}$

        \item No algorithm can distinguish a set of $k = c \frac{\sqrt{b}}{\eps^2}$ samples from $q$ from a set drawn from $p$ with probability of success greater than $\frac{3}{4}$, hence no algorithm can distinguish sets of $k$ samples drawn from the pair $(p, p)$ versus drawn from $(p, q)$ with this probability.
    \end{enumerate}
\end{lemma}

In order to obtain our lower bounds, we show that for an algorithm taking few samples, the mutual information between the observed sample and the input distribution is small, so that no algorithm can successfully distinguish two input distributions.
We will use the following upper bound on mutual information.

\begin{lemma}
    \label{lemma:one-elem-info-bound}
    For all $x \in \domain$, let $a_{x}$ be a random variable denoting the empirical frequency of $x$.
    Then, for all $x_i, x_{i + 1} \in \domain$ where $i = 1 \mod 2$,
    \begin{equation*}
        I(X: a_{x_i} a_{x_{i + 1}}) = O \left( \eps^2 \delta^2 \frac{k^2}{n^2} \; \log^4(n) \right)
    \end{equation*}
\end{lemma}

\begin{proof}
    The proof follows as a consequence of Lemmas \ref{lemma:break-mutual-info-bound}, \ref{lemma:sublin-info-bound}, \ref{lemma:superlin-info-bound}, and~\ref{lemma:superlearn-info-bound}.
\end{proof}

We begin by bounding the mutual information of the sub-linear regime.

\begin{lemma}
    \label{lemma:sublin-info-bound}
    Let $\frac{k}{n} \leq 1$.
    Let $\delta = |\epsa - \epsb|$ and $\eps = \max(\epsa, \epsb)$.
    Then,
    \begin{equation}
        \label{eq:sublin-info-bound}
        \sum_{a, b \in \N}
        \frac{(\Pr(M_1 = a, M_2 = b\mid X = 0) - \Pr(M_1 = a, M_2 = b \mid X = 1))^2}{\Pr(M_1 = a, M_2 = b)} \leq O \left( \frac{\eps^2 \delta^2 k^2}{n^2} \right).
    \end{equation}
\end{lemma}
\begin{proof}
    First, let us expand the conditional probabilities for a fixed $a,b$. 
    Expanding the definition of the random variables $M_1, M_2, X$ and applying the probability mass function of Poisson distributions, we arrive at the expression 
    % noting that if $a$ is a Poisson random variable with parameter either $\frac{k(1 \pm \epsa)}{n}$ or $\frac{k(1 \pm \epsb)}{n}$ depending on $X = 0, 1$.
    \begin{align*}
        &\Pr(M_1=a,M_2=b \mid X = 0) = \frac{1}{2 a!b!} \;
        \exp\left(-\frac{2k}{n}\right) \;
        \lp( \frac{k}{n} \rp)^{a+b}
        \lp( 
        \left(1 + \epsa \right)^a
        \left(1 - \epsa \right)^b
        +
        \left(1 - \epsa \right)^a
        \left(1 + \epsa \right)^b
        \rp) \, ,\\
        &\Pr(M_1=a,M_2=b \mid X = 0) = \frac{1}{2 a!b!} \;
        \exp\left(-\frac{2k}{n}\right) \;
        \lp( \frac{k}{n} \rp)^{a+b}
        \lp( 
        \left(1 + \epsb \right)^a
        \left(1 - \epsb \right)^b
        +
        \left(1 - \epsb \right)^a
        \left(1 + \epsb \right)^b
        \rp) \\
    \end{align*}
Define the function
$$
f_{a,b}( x )
:= (1 + x)^a(1-x)^b + (1-x)^a(1+x)^b. 
$$
Then we have
\begin{align}
&\sum_{ a,b \in \N }
\frac{(\Pr(M_1 = a, M_2 = b\mid X = 0) - \Pr(M_1 = a, M_2 = b \mid X = 1))^2}{\Pr(M_1 = a, M_2 = b)} \nonumber \\
&= 
O(1) \; 
\sum_{ a,b \in \N }
\frac{1}{a! b!} \exp\lp( - \frac{2k}{n} \rp) \lp(\frac{k}{n}\rp)^{a+b}
\frac{\lp( f_{a,b}(\epsb) - f_{a,b}(\epsa) \rp)^2}
{ f_{a,b}(\epsb) + f_{a,b}(\epsa) } \nonumber \\
&\leq
O(1) \; 
\sum_{ a,b \in \N }
\frac{1}{a! b!} \exp\lp( - \frac{2k}{n} \rp) \lp(\frac{k}{n}\rp)^{a+b}
\frac{\max_{ \epsa \leq x \leq \epsb }
\lp( \frac{\partial}{\partial x} f_{a,b}(x) \rp)^2}
{ f_{a,b}(\epsa) + f_{a,b}(\epsb) }
\lp( \epsb - \epsa \rp)^2 \, ,
\label{eq:mean-value}
\end{align}
where in the last line we use the mean value theorem.
The main technical step will be to bound from above the quantity
$\frac{\max_{ \epsa \leq x \leq \epsb }
\lp( \frac{\partial}{\partial x} f_{a,b}(x) \rp)^2}
{ f_{a,b}(\epsa) + f_{a,b}(\epsb) }$.
Specifically, we show the following technical claim.
\begin{claim}
\label{clm:poly-derivative}
There exists an absolute constant $C$ such that
\begin{equation}
\max_{\epsa < x < \epsb} \frac{\lp(\frac{\partial}{ \partial x} f_{a,b}(x)\rp)^2}{\lp( f_{a,b}(\epsa) + f_{a,b}(\epsb) \rp)}
= C \;
\begin{cases}
 &0 \,\text{ if } a+b \leq 1\\
 &(a^4+b^4) \eps^2 \,\text{ if } 1 < a+b \leq \eps^{-1} / 2 \\
 &(a+b)^2 \lp( \frac{1 + \eps}{ 1 - \eps} \rp)^{a+b} \,\text{ if } a+b > \eps^{-1}/2.
\end{cases}
\end{equation}    
\end{claim}
\begin{proof}
If $a+b \leq 1$, $f_{a,b}(x) = 2$. Thus, $\frac{d}{dx} f_{a,b}(x) = 0$, which gives the first case.

We next analyze the case $2 \leq a+b \leq \eps^{-1}$.
Note that $f_{a,b}(x)$ is an odd function with respect to $x$, i.e., $f_{a,b}(x) = f_{a,b}(-x)$.
This allows us to write $f_{a,b}(x) = \frac{1}{2} f_{a,b}(x) + f_{a,b}(-x)$. As a result, we can conclude that $f_{a,b}(x)$ does not contain any monomial of $x$ with odd degree.
Thus, we can write
\begin{align}
f_{a,b}(x) = c_{a,b}^{(0)} + \sum_{ d \in [a+b] \text{ is odd} } c_{a,b}^{(d)} x^d
\end{align}
for some coefficients $c_{a,b}^{(d)}$ that depend on $a,b$ only.
This implies that
\begin{align}
\frac{\partial}{\partial x} f_{a,b}(x) =  \sum_{ d \in [a+b] \text{ is odd} } d c_{a,b}^{(d)} x^{d-1}
\end{align}
When $2 \leq a+b \leq \eps^{-1}$, the coefficients $c_{a,b}^{(d)}$ is of order ${(a+b) \choose d}$.
Since $x < \eps / 2$, we must have that $|d c_{a,b}^{(d)} x^{d-1}|$ decreases exponentially fast in $d$.
This shows that $|\frac{\partial}{\partial x} f_{a,b}(x)|$ is dominated by the contribution from the monomial $|c_{a,b}^{(2)} x^1|$, which implies that
\begin{align}
\label{eq:caseII-derivative}
\max_{\epsa < x < \epsb} |\frac{\partial}{\partial x} f_{a,b}(x)|
\leq O(1) \; (a+b)^2 \eps.
\end{align}
To finish the analysis for this case, it then suffices to bound from below $f_{a,b}(\epsa) + f_{a,b}(\epsb)$.
Without loss of generality, assume that $a \leq b$. Then we have
\begin{align}
\label{eq:caseII-denominator}
f_{a,b}(\epsb) \geq (1-\epsb^2)^a \geq \Omega( 1 - a \epsb^2 ) \geq \Omega(1)  \, ,
\end{align}
where the last inequality follows from $a \leq a+b < \eps^{-1}$ and $\epsb < \eps$.
Combining \Cref{eq:caseII-derivative} and \Cref{eq:caseII-denominator} then concludes the proof of the second case.

Lastly, we analyze the case $(a+b) > \eps^{-1}/2$.
In this case, for $\eps_0 \leq x \leq \eps_1$,
we note that
\begin{align*}
\frac{\partial}{\partial x} f_{a,b}(x)
&= (1+x)^a(1-x)^b \lp( 
\frac{a}{1+x} - \frac{b}{1-x} \rp) 
+ (1-x)^a(1+x)^b
\lp( 
\frac{b}{1+x} - \frac{a}{1-x} \rp).
\end{align*}
It then follows that
\begin{align}
\label{eq:caseIII-derivative}
\lp| \frac{\partial}{\partial x} f_{a,b}(x) \rp|
&\leq
O(a+b) \; \lp(  (1+x)^a(1-x)^b + (1-x)^a(1+x)^b \rp) \nonumber\\
&\leq
O(a+b) \; \lp(  (1+x)^a + (1+x)^b \rp) \, ,
\end{align}
where in the first inequality we use that $ \abs{u - v} \leq u+v $ for any $u, v > 0$, and the second inequality simply follows from $1- x < 1$.
We can therefore conclude that
\begin{align*}
\max_{ \epsa \leq x \leq \epsb }
\frac{\lp( \frac{\partial}{\partial x} f_{a,b}(x) \rp)^2}{ f_{a,b}(\epsa)^2 + f_{a,b}(\epsb)^2 }
&\leq 
O(1) (a+b)^2 \; 
\frac{  \lp( (1+ \epsb )^{a} +  (1+\epsb)^{b} \rp)^2 }{ (1+\epsb)^a(1-\epsb)^b 
+ (1+\epsb)^b(1-x)^b
}  \\
&\leq 
O(1) (a+b)^2 \; 
\lp( \frac{  (1+ \epsb )^{a} }{ (1-\epsb)^b
} 
+ \frac{   (1+ \epsb )^{b} }{ (1-\epsb)^a
}  \rp) \\
&\leq 
O(1) (a+b)^2 \; 
\lp( \frac{  1+ \epsb  }{ 1-\epsb
} \rp)^{a+b} \, ,
\end{align*}
where in the first inequality we bound from above the numerator with the square of the right hand side of \Cref{eq:caseIII-derivative} substituted with $x = \epsb$, 
and bound from below the denominator by $f_{a,b}(\epsb)$, in the second inequality we use the fact that $(u+v)^2 \leq 2 u^2 + 2 v^2$, 
and in the last inequality we use that $(1+ \epsb )^{a}$, $(1-\epsb)^{-a}$ are increasing in $a$ and
$(1+ \epsb )^{b}$, $(1-\epsb)^{-b}$ are increasing in $b$.
This concludes the proof of the third case and also \Cref{clm:poly-derivative}.
\end{proof}
It immediately follows from the claim that 
\begin{align}
\label{eq:case-I-informtation-bound}
&\sum_{ a,b: a +b < 2}
\frac{(\Pr(M_1 = a, M_2 = b\mid X = 0) - \Pr(M_1 = a, M_2 = b \mid X = 1))^2}{\Pr(M_1 = a, M_2 = b)}   = 0.  
\end{align}


Consider the terms with $2 \leq a+b \leq \eps^{-1}/2$.
From \Cref{eq:mean-value} and \Cref{clm:poly-derivative}, 
we have that
\begin{align}
&\sum_{ a,b: 2 \leq a+b \leq \eps^{-1}/2}
\frac{(\Pr(M_1 = a, M_2 = b\mid X = 0) - \Pr(M_1 = a, M_2 = b \mid X = 1))^2}{\Pr(M_1 = a, M_2 = b)} 
\nonumber \\
&\leq 
O(1) \; 
\sum_{ a,b: 2 \leq a+b \leq \eps^{-1}/2}
\frac{1}{a! b!} \exp\lp( - \frac{2k}{n} \rp) \lp(\frac{k}{n}\rp)^{a+b}
(a^4+b^4) \delta^2 \eps^2
\nonumber \\
&= 
O(\delta^2 \eps^2)  \;
\lp( 
\sum_{ a \in N } 
\sum_{ b :  b: 2 \leq a+b \leq \eps^{-1}/2}
\frac{a^4}{a! b!}  \lp(\frac{k}{n}\rp)^{a+b}
+ 
\sum_{ b \in N } 
\sum_{ a : 2 \leq a+b \leq \eps^{-1}/2}
\frac{b^4}{a! b!}  \lp(\frac{k}{n}\rp)^{a+b} 
\rp).
% \sum_{ a,b: 2 \leq a+b \leq \eps^{-1}/2}
% \frac{1}{a! b!} \exp\lp( - \frac{2k}{n} \rp) \lp(\frac{k}{n}\rp)^{a+b}
% (a^2+b^2) \delta^2
\label{eq:A-B-split}
\end{align}
Define 
$A:= \sum_{ a \in N } 
\sum_{ b :  b: 2 \leq a+b \leq \eps^{-1}/2}
\frac{a^4}{a! b!}  \lp(\frac{k}{n}\rp)^{a+b}
$ and 
$B:= \sum_{ b \in N } 
\sum_{ a : 2 \leq a+b \leq \eps^{-1}/2}
\frac{b^4}{a! b!}  \lp(\frac{k}{n}\rp)^{a+b} $. One can see the two terms are similar to each other. So we focus on the term $A$.
We have that
\begin{align*}
A &= \sum_{b=1}^{ \eps^{-1}/2-1 }    
\frac{1}{b!} \lp( \frac{k}{n} \rp)^{1+b}
+ 
\sum_{a \geq 2}
\frac{a^4}{a!} \; \lp( \frac{k}{n} \rp)^a
\sum_{ b :  b: 2 \leq a+b \leq \eps^{-1}/2} 
\frac{1}{b!} \; \lp( \frac{k}{n} \rp)^b \\
&\leq 
O(1) \; \lp( \frac{k}{n} \rp)^2
+ 
O(1) \;
\sum_{a \geq 2}
\frac{a^4}{a!} \; \lp( \frac{k}{n} \rp)^a. \\
&\leq O(1) \; \lp( \frac{k}{n} \rp)^2
+ 
O(1) \; 
\exp(k/n) \; 
\sum_{a \geq 2}
\exp(-k/n) \; 
\frac{ a (a-1) + a (a-1)(a-2)(a-3)  }{a!} \; \lp( \frac{k}{n} \rp)^a \\
&\leq
O(1) \; \lp( \frac{k}{n} \rp)^2
+ 
O(1) \; 
\exp(k/n) \; 
\Ep_{ y \sim \PoiD{k/n} }\lp[ y (y-1) + y (y-1)(y-2)(y-3) \rp] \, , \\
&\leq O(1) \; \lp( \frac{k}{n} \rp)^2.
\end{align*}
where in the first inequality we use the assumption $k < n$ to
bound from the above the summation over $b$ by a geometric series with common ratio at most $1/2$, 
in the second inequality we use the fact that $a^4$ is at most  $
10 \;  \lp( a(a-1) + a(a-1)(a-2)(a-3) \rp)$ for all $a \geq 2$, 
in the third inequality we observe that the summation over $a$ can be bounded from above by the moments of some Poisson random variable with mean $k/n$, and in the last inequality we use the fact that $\Ep_{ y \sim \PoiD{\lambda} }[ y(y-1) + y(y-1)(y-2)(y-3) ] = \lambda^2 + \lambda^4$.
One can show the same upper bound for $B$ via an almost identical argument.
Substituting the bounds for $A,B$ into \Cref{eq:A-B-split} then gives that 
\begin{align}
\label{eq:case-II-informtation-bound}
&\sum_{ a,b: 2 \leq a+b \leq \eps^{-1}/2}
\frac{(\Pr(M_1 = a, M_2 = b\mid X = 0) - \Pr(M_1 = a, M_2 = b \mid X = 1))^2}{\Pr(M_1 = a, M_2 = b)}
\leq O( \delta^2 \eps^2 (k/n)^2 ).
\end{align}

It then remains to analyze the terms where $a+b \geq \eps^{-1}/2$.
Again from \Cref{eq:mean-value} and \Cref{clm:poly-derivative}, we have that
\begin{align}
&\sum_{ a,b \in \N }
\frac{(\Pr(M_1 = a, M_2 = b\mid X = 0) - \Pr(M_1 = a, M_2 = b \mid X = 1))^2}{\Pr(M_1 = a, M_2 = b)}
\nonumber \\
&\leq 
O(\delta^2) \; 
\sum_{ a,b: a+b > \eps^{-1}/2}
\frac{1}{a! b!} 
\lp(\frac{k}{n}\rp)^{a+b}
(a+b)^2 \lp(  \frac{1+\eps}{1-\eps} \rp)^{a+b} 
\nonumber \\
&= 
O(\delta^2) \; 
\sum_{ s > \eps^{-1}/2}
\lp(\frac{k}{n} \; \frac{1+\eps}{1-\eps }
\rp)^{s} s^2
\sum_{ a: a+b \leq s }
\frac{ 1  }{a! b!}  \nonumber \\
&\leq
O(\delta^2) \; 
\sum_{ s > \eps^{-1}/2}
\lp(\frac{k}{n} \; \frac{1+\eps}{1-\eps }
\rp)^{s}
\frac{ s^3 }{ \Gamma^2(s/2) } \nonumber \\
&\leq
O(\delta^2) \; 
\lp(\frac{k}{n} \; \frac{1+\eps}{1-\eps }
\rp)^{s}
\frac{ s^3 }{ \Gamma^2(s/2) } \bigg|_{ s = \eps^{-1}/2 } \nonumber \\
&\leq
O(\delta^2) \;
s^3 \; 
\lp( 
\frac{1}{2} \frac{k}{n} \; \frac{1+\eps}{1-\eps } \; 
\rp)^{s}\bigg|_{ s = \eps^{-1}/2 }
\leq O(\delta^2 \eps^2 (k/n)^2). 
\label{eq:case-III-informtation-bound}
\end{align}
where in the second inequality we use the convexity of the gamma function $\Gamma(\cdot)$ to bound each term by 
$(a+b)^2 / (a!b!) \leq \lp( s / \Gamma(s/2) \rp)^2$, 
in the third inequality we note that the summation over $s$ can be bounded from above by a geometric series with common ratio at most $\eps$ when $\eps$ is sufficiently small and $k < n$, in the fourth inequality we bound from below $\Gamma^2(s/2)$ by $2^s$, 
and in the last inequality we use that 
$(k/n)^{ \eps^{-1}/2 } \leq (k/n)^2$,
$ (1 + \eps)(1- \eps) \frac{1}{2} < 0.9 $, and that $0.9^{ \eps^{-1}/2 } \ll \poly{ \eps }$ for sufficiently small $\eps$.

Combining \Cref{eq:case-I-informtation-bound,eq:case-II-informtation-bound,eq:case-III-informtation-bound} then concludes the proof of \Cref{lemma:sublin-info-bound}.
\end{proof}


% \begin{proof}
%     First, let us write the conditional probabilities for general $l$, noting that if $a$ is a Poisson random variable with parameter either $\frac{k(1 \pm \epsa)}{n}$ or $\frac{k(1 \pm \epsb)}{n}$ depending on $X = 0, 1$.
%     \begin{align*}
%         \Pr(a = l \mid X = 0) &= \frac{1}{2} \left( \exp\left(-\frac{k(1+\epsa)}{n}\right) \frac{\left(\frac{k(1+\epsa)}{n}\right)^l}{l!} + \exp\left(-\frac{k(1-\epsa)}{n}\right) \frac{\left(\frac{k(1-\epsa)}{n}\right)^l}{l!} \right) \\ 
%         &= \frac{1}{2} \exp \left( - \frac{k}{n} \right) \frac{\left( \frac{k}{n} \right)^l}{l!} \left( \exp \left( - \frac{k \epsa}{n} \right) (1 + \epsa)^l + \exp \left( \frac{k \epsa}{n} \right) (1 - \epsa)^l \right) \\ 
%         \Pr(a = l \mid X = 1) &= \frac{1}{2} \exp \left( - \frac{k}{n} \right) \frac{\left( \frac{k}{n} \right)^l}{l!} \left( \exp \left( - \frac{k \epsb}{n} \right) (1 + \epsb)^l + \exp \left( \frac{k \epsb}{n} \right) (1 - \epsb)^l \right)
%     \end{align*}

%     In particular, we can express the (square root) of the numerator of \Cref{eq:sublin-info-bound} as,
%     \begin{equation}
%         \label{eq:sublin-prob-diff}
%         \Pr(a = l \mid X = 1) - \Pr(a = l \mid X = 0) = \frac{1}{2} \exp \left( - \frac{k}{n} \right) \frac{\left( \frac{k}{n} \right)^l}{l!} \left( f_{l}(\eps_1) - f_{l}(\eps_0) \right) 
%     \end{equation}
%     where for a fixed $l$, we define the function $f_l$,
%     \begin{equation*}
%         f_l(\eps) := \exp \left( - \frac{k \eps}{n} \right) (1 + \eps)^l + \exp \left( \frac{k \eps}{n} \right) (1 - \eps)^l
%     \end{equation*}

%     We now proceed by case analysis on $l$.
%     Consider the case $2 \leq l \leq \frac{2}{\eps}$. 
%     Using Taylor expansion on $f_l$, we can observe that the odd-degree terms cancel out and instead simplify the function to,
%     \begin{equation*}
%         f_l(\eps) = 2 \left( 1 + \binom{l}{2} \eps^2 - l \eps \frac{k \eps}{n} + \left(\frac{k \eps}{n}\right)^2 + \dotsc \right) = 2 \left( 1 + \left( \binom{l}{2} - \frac{k l}{n} + \frac{k^2}{n^2} \right) \eps^2 +  \dotsc \right)
%     \end{equation*}

%     If we now take the derivative with respect to $\eps$ (using $l \eps \leq 2$ to bound the lower order terms),
%     \begin{equation*}
%         f_l'(\eps) = 2 \left( 2 \left( \binom{l}{2} - \frac{k l}{n} + \frac{k^2}{n^2} \right) \eps + \bigO{\eps^3 l^4} \right) = \bigO{\eps l^2}
%     \end{equation*}
%     where we used $\frac{k}{n} \leq 1$.
%     Then, using a first order Taylor approximation, we can upper bound Equation~\ref{eq:sublin-prob-diff} by
%     \begin{align*}
%         |\Pr(a = l \mid X = 0) - \Pr(a = l \mid X = 1)| &\leq \exp \left( - \frac{k}{n} \right) \frac{\left( \frac{k}{n} \right)^l}{l!} |\epsb - \epsa| \bigO{\eps l^2} \\ 
%         &= \exp \left( - \frac{k}{n} \right) \frac{\left( \frac{k}{n} \right)^l}{l!} \bigO{\delta \eps l^2} \\
%         &= \exp \left( - \frac{k}{n} \right)  \frac{\left( \frac{k}{n} \right)^{l - 2}}{(l - 2)!} \bigO{\frac{k^2}{n^2} \delta \eps}
%     \end{align*}

%     We will separately consider the cases $l = 0, 1$.
%     First, if $l = 0$,
%     \begin{align*}
%         \exp \left( - \frac{k \eps}{n} \right) + \exp \left( \frac{k \eps}{n} \right) &= 2 \left( 1 + \frac{k \eps}{n}^2 + \frac{k \eps}{n}^4 + \dotsc \right)
%     \end{align*}

%     Then, again using the derivative to bound Equation \ref{eq:sublin-prob-diff},
%     \begin{align*}
%         |\Pr(a = 0 \mid X = 0) - \Pr(a = 0 \mid X = 1)| &\leq e^{-\frac{k}{n}} |\epsa - \epsb| \left( \frac{2 k^2}{n^2} \eps + \frac{4 k^3}{n^3} \eps^3 + \dotsc \right) \\ 
%         &=  e^{-\frac{k}{n}} \bigO{\frac{k^2}{n^2} \delta \eps }
%     \end{align*}

%     If $l = 1$,
%     \begin{align*}
%         \exp \left( - \frac{k \eps}{n} \right) (1 + \eps) + \exp \left( \frac{k \eps}{n} \right) (1 - \eps) &= 2 \left( 1 - \eps \frac{k \eps}{n} + \frac{k \eps}{n}^2 - \eps \frac{k \eps}{n}^3 + \frac{k \eps}{n}^4 + \dotsc \right) \\
%         &= 2 \left( 1 + \left( \frac{k^2}{n^2} - \frac{k}{n}\right) \eps^2 + \left( \frac{k^4}{n^4} - \frac{k^3}{n^3} \right) \eps^4 + \dotsc \right)
%     \end{align*}

%     Again, we take the derivative and bound Equation \ref{eq:sublin-prob-diff},

%     \begin{align*}
%         |\Pr(a = 1 \mid X = 0) - \Pr(a = 1 \mid X = 1)| &\leq e^{-\frac{k}{n}} \frac{k}{n} |\epsa - \epsb| \left| 2 \left( \frac{k^2}{n^2} - \frac{k}{n} \right) \eps + 4 \left( \frac{k^4}{n^4} - \frac{k^3}{n^3} \right) \eps^3 + \dotsc \right| \\ 
%         &= e^{-\frac{k}{n}} \bigO{ \frac{k^2}{n^2} \delta \eps}
%     \end{align*}

%     Next, we proceed to estimate the denominator $\Pr(a = l)$ of Equation \ref{eq:sublin-info-bound} for $l \leq \frac{2}{\eps}$.
%     We can assume $\eps < \frac{1}{2}$, so that we can lower bound $f_l(\eps)$,

%     \begin{align*}
%         f_l(\eps) &= \exp \left( - \frac{k \eps}{n} + l \log (1 + \eps) \right) + \exp \left( \frac{k \eps}{n} + l \log (1 - \eps) \right) \\
%         &\geq \exp \left( - \frac{k \eps}{n} + \frac{l \eps}{3} \right) +  \exp \left( \frac{k \eps}{n} - l \eps \right) \\
%         &\geq \exp \left( \eps \left( \frac{l}{3} - \frac{k}{n} \right) \right) \\
%         &\geq e^{- \eps} = \Omega(1)
%     \end{align*}
%     where in the first equality we use $\log (1 + x) \geq \frac{x}{3}$ and $\log (1 - x) \geq - x$ for $x < \frac{1}{2}$, that exponents are non-negative in the second inequality, $l \geq 0$ and $\frac{k}{n} \leq 1$ in the third inequality, and again $\eps < \frac{1}{2}$ in the final equality.

%     Then, we can lower bound $\Pr(a = l)$,
%     \begin{align*}
%         \Pr(a = l) &= \frac{1}{2} \left(\Pr(a = l \mid X = 0) + \Pr(a = l \mid X = 1)\right) \\
%         &= \frac{1}{2} \exp \left( - \frac{k}{n} \right) \frac{\left( \frac{k}{n} \right)^l}{l!} (f_l(\eps_0) + f_l(\eps_1)) \\
%         &= \bigOm{\exp \left( - \frac{k}{n} \right) \frac{\left( \frac{k}{n} \right)^l}{l!}}
%     \end{align*}
%     Since $\frac{k}{n} \leq 1$, the lower bound decreases as $l$ increases.

%     Finally, we can bound the sum of all terms for $l \leq \frac{2}{\eps}$,
%     \begin{align*}
%         \sum_{l = 0}^{1} \frac{(\Pr(a = l \mid X = 0) - \Pr(a = l \mid X = 1))^2}{\Pr(a = l)} &= \bigO{\sum_{l = 0}^{1} \frac{e^{-\frac{2k}{n}} \frac{k^4}{n^4} \delta^2 \eps^2}{e^{-\frac{k}{n}} \frac{k}{n}}} = \bigO{\frac{k^3}{n^3} \delta^2 \eps^2}
%     \end{align*}
%     and,
%     \begin{align*}
%         \sum_{l = 2}^{2/\eps} \frac{(\Pr(a = l \mid X = 0) - \Pr(a = l \mid X = 1))^2}{\Pr(a = l)} &= \bigO{\sum_{l = 2}^{2 / \eps} \frac{e^{-\frac{2 k}{n}} \frac{\left( \frac{k}{n} \right)^{2l - 4}}{(l - 2)!^2} \frac{k^4}{n^4} \delta^2 \eps^2}{e^{-\frac{k}{n}} \frac{\left( \frac{k}{n} \right)^{l}}{l!}}} \\
%         &= \frac{k^2}{n^2} \delta^2 \eps^2 \bigO{\sum_{l = 2}^{2 / \eps} \frac{e^{-\frac{k}{n}} \left( \frac{k}{n} \right)^{l - 2} l (l - 1)}{(l - 2)!}} \\
%         &= \bigO{\frac{k^2}{n^2} \delta^2 \eps^2}
%     \end{align*}

%     where in the last equality, we used that the sum is at most the expectation of $X^2$ where $X$ is a Poisson random variable with parameter $\frac{k}{n} \leq 1$.

%     It remains to analyze $l > \frac{2}{\eps}$.
%     Recall the function $f_l(\eps)$.
%     Previously for small $l$ we were able to use a Taylor approximation to bound the derivative.
%     For large $l$, we bound the derivative directly.

%     \begin{align*}
%         f_l'(\eps) &= \frac{k}{n} e^{\frac{k \eps}{n}} (1 - \eps)^l - l e^{\frac{k \eps}{n}} (1 - \eps)^{l - 1} - \frac{k}{n} e^{-\frac{k \eps}{n}} (1 + \eps)^l + l e^{- \frac{k \eps}{n}} (1 + \eps)^{l - 1} \\
%         &= e^{\frac{k \eps}{n}} (1 - \eps)^{l - 1} \left( \frac{k}{n} (1 - \eps) - l \right) + e^{- \frac{k \eps}{n}} (1 + \eps)^{l - 1} \left( l + \frac{k}{n} (1 + \eps) \right) \\
%         |f_l'(\eps)| &= \bigO{l(1 + \eps)^{l - 1}}
%     \end{align*}

%     Then,
%     \begin{align*}
%         \left|\Pr(a = l \mid X = 0) - \Pr(a = l \mid X = 1)\right|&= \bigO{\exp\left( -\frac{k}{n} \right) \frac{\left( \frac{k}{n} \right)^l}{l!} \delta l (1 + \eps)^{l - 1}}
%     \end{align*}

%     Then, summing over all $l \geq \frac{2}{\eps}$,
%     \begin{align*}
%         \sum_{l = 2/\eps}^{\infty} \frac{(\Pr(a = l \mid X = 0) - \Pr(a = l \mid X = 1))^2}{\Pr(a = l)} &= \delta^2 \bigO{\sum_{l = 2/\eps}^{\infty} e^{-\frac{k}{n}} \frac{\left( \frac{k}{n} \right)^l}{l!} l^2 (1 + \eps)^{2l - 2}} \\
%         &= \frac{k^2}{n^2} \delta^2 \bigO{\sum_{l = 2/\eps}^{\infty} e^{-\frac{k}{n}} \frac{\left( \frac{k}{n} \right)^{l - 2}}{(l - 2)!} (1 + \eps)^{2l - 2}} \\
%         &= \frac{k^2}{n^2} \delta^2 \bigO{e^{-\frac{k}{n}} \sum_{l = 2/\eps}^{\infty} \frac{\left( \frac{k}{n} \right)^{l - 2}}{(l - 2)!} e^{\eps (l - 2)}} \\
%         &= \frac{k^2}{n^2} \delta^2 \bigO{e^{-\frac{k}{n}} \sum_{l = 2/\eps}^{\infty} \frac{\left( \frac{k}{n} e^{\eps} \right)^{l - 2}}{(l - 2)!}} \\
%         &= \bigO{\frac{k^2}{n^2} \delta^2 \eps^2}
%     \end{align*}

%     where in the last step we observe that the sum is simply the error of a Taylor series approximation, thus completing the proof.
% \end{proof}

We now bound the mutual information for the super-linear regime.

\begin{lemma}
    \label{lemma:superlin-info-bound}
    Let $\delta = |\epsa - \epsb|$ and $\eps = \max(\epsa, \epsb)$.
    Let $n < k < \frac{n}{ 2 \; \log^2 n \; \eps^2}$.
    Then,
    \begin{equation*}
        \sum_{l = 0}^{\infty} \frac{(\Pr(a = l \mid X = 0) - \Pr(a = l \mid X = 1))^2}{\Pr(a = l)} \leq O \left( \frac{\eps^2 \delta^2 k^2 \; \log^4 n }{n^2} \right).
    \end{equation*}
\end{lemma}

\begin{proof}
We note that for a Poisson random variable $y$ with mean $\lambda \geq 1$, we have $|y - \lambda| > \sqrt{\lambda} \log n$ with probability at most $o(1/n)$.
we can focus on the terms where $ a $
$l \in [\lambda - \sqrt{\lambda} \log n, \lambda + \sqrt{\lambda} \log n]$.
For reasons that will become clear soon, we will assume that $a,b$ both lie in this range.

As in the sub-linear case,  we define the function
$$
f_{a,b}( x )
:= (1 + x)^a(1-x)^b + (1-x)^a(1+x)^b. 
$$
Instead of computing the derivative of $f_{a,b}$ directly, we will first rewrite it slightly.
\begin{align}
f_{a,b}( x ) 
&=
\exp \lp( a \ln(1+x) + b \ln(1-x)  \rp)
+ 
\exp \lp( a \ln(1-x) + b \ln(1+x)  \rp) \\
&= 
2 + 
a \ln(1-x^2) + b \ln(1-x^2) \\
&+ \sum_{i=2}^{\infty}
\frac{ \lp( a \ln(1+x) + b \ln(1-x) \rp)^i
+ \lp( a \ln(1-x) + b \ln(1+x) \rp)^i
}{i!} \, ,
\end{align}
where in the second equality we apply the Taylor approximation of the exponential function. 
We will analyze the expression terms by terms. 
In particular, define
\begin{align*}
g_{y}(x) =  y \; \ln(1-x^2) \, ,
h_{a,b}(x)  = \sum_{i=2}^{\infty} \frac{ \lp( a \ln(1+x) + b \ln(1-x) \rp)^i
}{i!}.
\end{align*}
Then we have
\begin{align}
\label{eq:f-decompose}
f_{a,b}(x) = 2 + g_{a}(x) + g_b(x) + h_{a,b}(x) + h_{a,b}(-x).
\end{align}
We first analyze $g_{a}(x)$.
When $a \in [ \lambda - \sqrt{\lambda} \log n, \lambda + \sqrt{\lambda} \log n ]$, we have that
\begin{align}
\lp| g_a( \epsb ) - g_a(\epsa) \rp|
&= 
    \abs{ a \log \lp( \frac{1 - \eps_0^2}{1 - \eps_1^2} \rp) }
    \leq a \; \abs{ 1 - \frac{1 - \eps_0^2}{1 - \eps_1^2} } \nonumber \\
&= \frac{a}{ 1-  \eps_1^2 } \lp( \eps_0 + \eps_1 \rp) \abs{\eps_0 - \eps_1}
    \leq O \lp(  \frac{k}{n} \; \log n \; \eps \; \delta \rp) \, ,
\label{eq:g-bound}
\end{align}
where in the first inequality we use the fact $\abs{\log(x)} \leq \abs{1 - x}$ for $x \geq 1$, in the second inequality we use our assumption that
$\max(\eps_0, \eps_1) \leq \eps$ and $\abs{\eps_0 - \eps_1} \leq \delta$, and our assumption that $\abs{ a - k/n } < \log n \sqrt{k/n}$.
Using a similar argument, one can also derive that
\begin{align}
\label{eq:g-bound-2}
|g_b(\eps_1) - g_b(\eps_0)|
\leq O \lp(  \frac{k}{n} \; \log n \; \eps \; \delta \rp).
\end{align}

We then turn to the term $h_{a,b}(x)$.
The derivative with respect to $x$ is given by
\begin{align*}
\frac{\partial}{\partial x}h_{a,b}(x)
&= 
\lp( \frac{a}{ 1+x } - \frac{b}{1-x} \rp)
\sum_{i=2}^{\infty} 
\frac{ \lp( a \ln(1+x) + b \ln(1-x) \rp)^{i-1}
}{ (i-1)! } \\
&= 
\lp( \frac{a}{ 1+x } - \frac{b}{1-x} \rp)
\lp( (1+x)^a(1-x)^b -1 \rp)
\end{align*}
where the second equality follows from the observation that the summation is exactly the Taylor approximation of $\exp  \lp( a \ln(1+x) + b \ln(1-x) \rp)$ without the constant term.
We next proceed to bound from above $\lp| \frac{\partial}{\partial x}h_{a,b}(x) \rp|$
First, when $x$ is sufficiently small and $a,b$ lie in the range $\frac{k}{n} \pm \sqrt{ \frac{k}{n} } \log n$, 
note that
\begin{align}
\lp| 
\frac{a}{1+x} - \frac{b}{1-x}
\rp|
&= 
\lp| 
a-b - O(x) (a+b)
\rp| \nonumber \\
&\leq \abs{a-b} + (a+b) O(x) \nonumber \\
&\leq \sqrt{ \frac{k}{n} } \log n + 2 \frac{k}{n} x
+ 2 \sqrt{  \frac{k}{n}  } \log (n) x \nonumber \\
&\leq O \lp( \sqrt{ \frac{k}{n} } \log n \rp) \, ,
\label{eq:h-derivative-1st}
\end{align}
where in the first line we approximate $\frac{1}{1+x}$ and $\frac{1}{1-x}$ with $1 - O(x)$ and $1 + O(x)$ respectively for sufficiently small $x$, 
the second line follows from the triangle inequality, in the third line we use the assumption on the ranges of $a,b$, 
in the last line we note that $\sqrt{\frac{k}{n}} \log n$ is the dominating term when $x < \eps$
and $k < n / \eps^{2}$.
Next, under the same set of assumptions, we have that
\begin{align}
\lp( (1+x)^a(1-x)^b -1 \rp)    
&\leq
\lp( (1-x^2)^b (1+x)^{|a-b|}   -1 \rp) \nonumber \\
&\leq 
\lp( (1- O(b x^2)  ) (1+ O(|a-b|) x)   -1 \rp)  \nonumber \\
&\leq 
O \lp( \eps \; \sqrt{\frac{k}{n}} \log n \rp) \, ,
\label{eq:h-derivative-2nd}
\end{align}
where in the second inequality we note that 
since $b x^2  = O\lp( 
\frac{k}{n} \eps^2
\rp) = o(1)$ and $ |a-b| x = O\lp( 
\sqrt{\frac{k}{n}} \eps
\rp)  = o(1)$ we can approximate $(1-x^2)^b$ and 
$(1+x)^{|a-b|}$ by $(1- O(b x^2)  ) $ and $(1+ O(|a-b|) x)$ respectively, 
and in the last inequality we use the assumption on the range of $a,b$ and $x < \eps$.
Thus, combining \Cref{eq:h-derivative-1st,eq:h-derivative-2nd}, we arrive at the upper bound
\begin{align*}
\max_{ x \in [\epsa, \epsb] } \frac{\partial}{\partial x}h_{a,b}(x)    
\leq O\lp( \eps \frac{k}{n} \log^2 n  \rp) \, ,
\end{align*}
when $ \frac{k}{n} - \sqrt{k/n} \log n \leq  a, b 
\leq \frac{k}{n} + \sqrt{k/n} \log n
$.
Therefore, by the mean value theorem, we have that
\begin{align}
\label{eq:h-bound}
\abs{ h_{a,b}(\epsb) - h_{a,b}(\epsa) }    
\leq O\lp( \eps \delta \frac{k}{n} \log^2 n  \rp).
\end{align}
Following a similar argument, one can also derive the upper bound
\begin{align}
\label{eq:h-bound-2}
\abs{ h_{a,b}(-\epsb) - h_{a,b}(-\epsa) }    
\leq O\lp( \eps \delta \frac{k}{n} \log^2 n  \rp).
\end{align}
Combining \Cref{eq:f-decompose,eq:g-bound,eq:g-bound-2,eq:h-bound,eq:h-bound-2} then gives that
\begin{align}
\label{eq:f-diff-bound}
\lp| f_{a,b}(\epsb) - f_{a,b}(\epsa) \rp|
\leq O\lp( \eps \delta \frac{k}{n} \log^2 n  \rp).
\end{align}


Recall that in the proof of \Cref{lemma:sublin-info-bound}, we have that
\begin{align}
\label{eq:info-identity-simplify}
&\sum_{ a,b \in \N }
\frac{(\Pr(M_1 = a, M_2 = b\mid X = 0) - \Pr(M_1 = a, M_2 = b \mid X = 1))^2}{\Pr(M_1 = a, M_2 = b)}  \nonumber \\
&= 
O(1) \; 
\sum_{ a,b \in \N }
\frac{1}{a! b!} \exp\lp( - \frac{2k}{n} \rp) \lp(\frac{k}{n}\rp)^{a+b}
\frac{\lp( f_{a,b}(\epsb) - f_{a,b}(\epsa) \rp)^2}
{ f_{a,b}(\epsb) + f_{a,b}(\epsa) }.
\end{align}
Hence, we proceed to bound from below $f_{a,b}( \epsa ) + f_{a,b}( \epsb )$.
Note that we have
\begin{align}
\label{eq:f-lower-bound}
f_{a,b}( \epsa ) + f_{a,b}( \epsb )
\geq (1-x^2)^{ \min(a,b) } (1+x)^{ |a-b| }
\geq 1 - O( \min(a,b) x^2 ) \geq \Omega(1) \, ,
\end{align}
where the first inequality follows from a case analysis on whether $a>b$, in the second inequality we approximate $(1-x^2)^{ \min(a,b) }$ by 
$1 - O( \min(a,b) x^2 )$ since $\min(a,b) x^2 = o(1)$ for $a,b$ in the assumed range and $x < \eps$.
Combining \Cref{eq:info-identity-simplify,eq:f-lower-bound,eq:f-diff-bound} then gives that
\begin{align*}
&\sum_{ a,b \in \N }
\frac{(\Pr(M_1 = a, M_2 = b\mid X = 0) - \Pr(M_1 = a, M_2 = b \mid X = 1))^2}{\Pr(M_1 = a, M_2 = b)}  \\
&\leq
O(1) \; 
\sum_{ a,b \in \N }
\mathbbm 1 \{ k/n - \sqrt{k/n} \log n \leq a,b \leq  k/n + \sqrt{k/n} \log n  \}
\frac{1}{a! b!} \exp\lp( - \frac{2k}{n} \rp) \lp(\frac{k}{n}\rp)^{a+b}
  \eps^2 \delta^2 ((k/n)^2 \log^4 n\\
  &+ 
  O(1) \; 
  \lp( 1 - \Pr_{ a, b \sim \PoiD{ k/n } } \lp[  
  k/n - \sqrt{k/n} \log n \leq a,b \leq  k/n + \sqrt{k/n} \log n
  \rp] \rp) \\
&\leq 
\eps^2 \delta^2 ((k/n)^2 \log^4 n + O(1/n).
\end{align*}





    % Suppose $(b - 1) \sqrt{k/n} \leq \left| l - k/n \right| \leq b \sqrt{k/n}$.
    Recall from the previous section that we had
    \begin{equation*}
        % \label{eq:sublin-prob-diff}
        \Pr(a = l \mid X = 1) - \Pr(a = l \mid X = 0) = \frac{1}{2} \exp \left( - \frac{k}{n} \right) \frac{\left( \frac{k}{n} \right)^l}{l!} \left( f_{l}(\eps_1) - f_{l}(\eps_0) \right) 
    \end{equation*}
    where for a fixed $l$, we define the function $f_l$,
    \begin{equation*}
        f_l(\eps) := \exp \left( - \frac{k \eps}{n} \right) (1 + \eps)^l + \exp \left( \frac{k \eps}{n} \right) (1 - \eps)^l
    \end{equation*}    
    We will first replace the exponential function in $f_{\ell}(\eps)$ with its Taylor expansion. We then have
    \begin{align} \label{eq:exp-expansion}
    f_{\ell}(\eps) 
    = 2 + \ell \log(1 - \eps^2)
    + \sum_{i=2}^{\infty} \frac{ \lp( \frac{ k}{ n} \; \eps + \ell \; \log(1 - \eps) \rp)^i }{i!}       
    + \sum_{i=2}^{\infty} \frac{ \lp( \frac{- k}{ n} \; \eps + \ell \; \log(1 + \eps) \rp)^i }{i!}.
    \end{align}
    Our goal is to upper bound $\abs{ f_{\ell}(\eps_0) - f_{\ell}(\eps_1) }$.
    It is easy to see that the constant term $2$ will be cancelled when computing the difference. Hence, it remains to analyze the three remaining terms.
    For the term $\ell \log(1 - \eps^2)$, we have
    \begin{align*}
    \abs{\ell \log(1-\eps_0^2)        
    - \ell \log(1 - \eps_1^2)}
    &= 
    \abs{ \ell \log \lp( \frac{1 - \eps_0^2}{1 - \eps_1^2} \rp) }
    \leq \ell \; \abs{ 1 - \frac{1 - \eps_0^2}{1 - \eps_1^2} } \\
    &= \frac{\ell}{ 1-  \eps_1^2 } \lp( \eps_0 + \eps_1 \rp) \abs{\eps_0 - \eps_1}
    \leq O( \ell \eps \delta )
    \leq O \lp(  \frac{k}{n} \; \log n \; \eps \; \delta \rp) \, ,
    \end{align*}
    where in the first inequality we use the fact $\abs{\log(x)} \leq \abs{1 - x}$ for $x \geq 1$, in the second inequality we use our assumption that
    $\max(\eps_0, \eps_1) \leq \eps$ and $\abs{\eps_0 - \eps_1} \leq \delta$, and in the last inequality we use our assumption that $\abs{ \ell - k/n } < \log n \sqrt{k/n}$ and  $k < n / ( \log^2 n \; \eps )$.
    % $$
    % \abs{\ell \log(1 - \eps^2)}
    % \leq O( \ell \eps^2 )
    % \leq O \lp( \frac{k}{n} \eps^2 + \sqrt{ \frac{k}{n} } \log n \; \eps^2 \rp)
    % = O \lp(  \frac{k}{n} \; \log n \; \eps \rp) \, ,
    % $$
    % where 
    % in the first inequality we use the Taylor Expansion of $\log(1-\eps)$,
    % in the second inequality we use our assumption that $\abs{ \ell - k/n } < \log n \sqrt{k/n}$,
    % and in the third inequality we use $k < n / ( \log^2 n \; \eps )$.

    To analyze the second term in \Cref{eq:exp-expansion}, we define the function
    $$
    g_{\ell}(\eps) := \sum_{i=2}^{\infty} \frac{ \lp( \frac{ k}{ n} \; \eps + \ell \; \log(1 - \eps) \rp)^i }{i!}.
    $$
    Then we compute its derivative with respect to $\eps$. In particular, we have
    \begin{align}
    \label{eq:g-derivative}
    g_{\ell}'(\eps) 
    = \sum_{i=2}^{\infty} \frac{ 
    \lp( \frac{k}{n} - \frac{\ell}{1 - \eps} \rp) \; 
    \lp( \frac{ k}{ n} \; \eps + \ell \; \log(1 - \eps) \rp)^{i-1} }{(i-1)!}.
    \end{align}
    The absolute value of the first factor in the denominator can be upper bounded by
    $$
    \abs{ \frac{k}{n} - \frac{\ell}{1 - \eps} }
    \leq
    \abs{ \frac{k}{n} - \ell + O( \eps \ell ) }
    \leq 
    O \lp( \sqrt{ \frac{k}{n} } \log n\rp) \, ,
    $$
    where 
    in the first inequality we approximate $\frac{1}{1 - \eps}$ by $(1 + O(\eps))$ when $\eps$ is sufficiently small,
    in the second inequality we use our assumption that $\ell = \frac{k}{n} \pm O( \sqrt{k/n} \; \log n )$ and that $k < n / (\log^2 n \; \eps )$.
    We then analyze the absolute value of term in the denominator that is raised to its $(i-1)$-th power. We can upper bound it by
    \begin{align*}
    \abs{ \frac{k \eps}{n} + \ell \; \log(1 - \eps) }
    &\leq \abs{ \frac{k \eps}{n} - \ell \eps  } + O( \ell \eps^2 )
    \leq O \lp(  \sqrt{ \frac{k}{n} } \; \log n \; \eps \rp) + O( \frac{k}{n} \eps^2  +  \sqrt{\frac{k}{n}} \; \log n \; \eps^2 )         \\
    &\leq O\lp( \sqrt{ \frac{k}{n} } \; \log n \; \eps \rp) \, ,
    \end{align*}
    where in the first inequality we use the Taylor approximation of $\log(1 - \eps) = - \eps + O(\eps^2)$, in the second inequality we use our assumption that $\abs{ \ell - k/n } < \log n \sqrt{k/n}$, and in the last inequality we use $k < n/( \log^2 n \; \eps )$.
    Notice that $\sqrt{k/n} \; \log n \; \eps < 1/2$ by our assumption $k < n/( \log^2 n \; \eps )$.
    Hence, we conclude that the dominating term in the summation in \Cref{eq:g-derivative} is the one with $i = 2$.
    Therefore, we can upper bound $\abs{g_{\ell}'(\eps)}$ by
    $$
    \abs{g_{\ell}'(\eps)}
    \leq O(1) \; \sqrt{ \frac{k}{n} } \log n \; \sqrt{ \frac{k}{n} } \; \log n \; \eps
    = O\lp(  \; \frac{k}{n} \; \log^2 n \; \eps \rp).
    $$
    It then follows that
    $$
    \abs{ g_{\ell}(\eps_0) - g_{\ell}(\eps_1) }
    \leq O\lp(  \; \frac{k}{n} \; \log^2 n \; \eps \; \delta \rp) \, ,
    $$
    since $\max(\eps_0, \eps_1) < \eps$ and $\abs{\eps_0 - \eps_1} < \delta$.
    Now, for the last term in \Cref{eq:exp-expansion}, we can similarly define
$$
    g^{-}_{\ell}(\eps) := \sum_{i=2}^{\infty} \frac{ \lp( \frac{ k}{ n} \; \eps + \ell \; \log(1 - \eps) \rp)^i }{i!}.
$$
Using an argument almost identical to that of $g_{\ell}(\eps)$, we can similarly show
$$
    \abs{ g_{\ell}^{-}(\eps_0) - g_{\ell}^{-}(\eps_1) }
    \leq O\lp(  \; \frac{k}{n} \; \log^2 n \; \eps \; \delta \rp).
$$
Combining our analysis for the four terms in \Cref{eq:exp-expansion}, we therefore conclude
$$
\abs{f_{ \ell }( \eps_0 ) - f_{\ell}(  \eps_1 )}
\leq O\lp(  \; \frac{k}{n} \; \log^2 n \; \eps \; \delta \rp)
$$
for all $\ell > 0$ such that $\abs{ \ell - k/n } \leq \sqrt{k/n \; \log n \; \eps}$.
    Combining this with \Cref{eq:sublin-prob-diff} we obtain,
    \begin{align*}
        \abs{\Pr(a = l \mid X = 1) - \Pr(a = l \mid X = 0)} &= \frac{1}{2} \exp \left( - \frac{k}{n} \right) \frac{\left( \frac{k}{n} \right)^l}{l!} \abs{f_{l}(\eps_1) - f_{l}(\eps_0)} \\
        &\leq 
        O(1) \; 
        \exp\left(- \frac{k}{n}\right) \frac{(k/n)^{l}}{l!} \; 
        \frac{k}{n} \; \log^2 n \; \eps \; \delta.
    \end{align*}
    We now proceed to lower bound the denominator $\Pr(a = l)$. 
    As in \Cref{lemma:sublin-info-bound}, we begin by lower bounding $f_l(\eps)$.
    \begin{align*}
        f_l(\eps) &= \exp \left( - \frac{k \eps}{n} + l \log (1 + \eps) \right) + \exp \left( \frac{k \eps}{n} + l \log (1 - \eps) \right) \\
        &\geq \exp \left( - \eps + \frac{l \eps}{3} \right) +  \exp \left( \frac{k \eps}{n} - l \eps \right) \\
        &\geq \exp \left( \eps \left( \frac{l}{3} - 1 \right) \right) \\
        &\geq e^{- \eps}  \, ,
    \end{align*}
    where in the first inequality we use $\frac{k}{n} \geq 1$ $\log(1 + x) \geq \frac{x}{3}$ and $\log(1 - x) \geq - x$ for $x \in [0, 1/2]$.
    Recall the identity
    $$
        \Pr(a = l)
        = \frac{1}{2} \exp \left( - \frac{k}{n} \right) \frac{\left( \frac{k}{n} \right)^l}{l!} (f_l(\eps_0) + f_l(\eps_1)).
    $$
    Hence, it follows that
    $$
    \Pr(a = l) 
    \geq 
    \exp(-\eps) \; 
    \exp \left( - \frac{k}{n} \right) \frac{\left( \frac{k}{n} \right)^l}{l!}.
    $$
    Therefore, we can upper bound the summand for $\ell \geq 0$ satisfying
    $\abs{ \ell - k/n } \leq \sqrt{k/n \; \log n \; \eps}$ by
    \begin{align*}
    \frac{ \lp(\Pr(a = \ell \mid X = 1) - \Pr(a = \ell \mid X = 0) \rp)^2}{ \Pr(a = \ell) }        
    &\leq O(1) \; \exp\lp( - \frac{k}{n} \rp) \; \frac{ (k/n)^{\ell} }{ \ell! } \; 
    \frac{k^2}{n^2} \; \log^4 n \; \eps^2 \; \delta^2.
    \end{align*}
    Now, we sum over all $\ell \geq 0$. This gives us
    \begin{align*}
        &\sum_{l = 0}^{\infty} \frac{(\Pr(a = l \mid X = 0) - \Pr(a = l \mid X = 1))^2}{\Pr(a = l)}  \\
        &\leq 
        o(1/n)
        + 
        O(1) \; 
        \sum_{l = \max\lp(0, \frac{k}{n} - \sqrt{k}{n} \; \log n\rp)}^{ \frac{k}{n} + \sqrt{k}{n} \; \log n }
        \exp\lp( - \frac{k}{n} \rp) \; \frac{ (k/n)^{\ell} }{ \ell! } \; 
        \frac{k^2}{n^2} \; \log^4 n \; \eps^2 \; \delta^2 \\
        &\leq o(1/ n) + O \lp(  \frac{k^2}{n^2} \; \log^4 n \; \eps^2 \; \delta^2 \rp) \, ,        
    \end{align*}
where in the first inequality we use the fact that $|a - \lambda| > \sqrt{\lambda} \log n$ with probability at most $o(1/n)$ for $a \sim \PoiD{k/n}$,
and in the  last inequality we use the fact that $ \sum_{\ell} \exp\lp( - \frac{k}{n} \rp) \; \frac{ (k/n)^{\ell} }{ \ell! }$ must be less than one since its summand is exactly the probability mass function of Poisson distribution with mean $k/n$ evaluated at the point $\ell$.    
    % Taking the derivative with respect to $\eps$ gives
    % \begin{align*}
    %     f_l'(\eps) &= \left( \frac{l}{1 + \eps} - \frac{k}{n} \right) \exp \left( - \frac{k \eps}{n} + l \log (1 + \eps) \right) + \left( \frac{k}{n} - \frac{l}{1 - \eps} \right) \exp \left( \frac{k \eps}{n} + l \log (1 - \eps) \right).
    % \end{align*}
    % To present our bound cleanly, we define the quantity 
    % $$
    % b_{\ell} := \abs{\ell - \frac{k}{n}} / \lp( \eps \sqrt{k/n} \rp).
    % $$
    % Using the inequality $\log(x) \leq x - 1$
    % and the bound on $\ell$, we can upper bound the first exponential term by
    % \begin{align*}
    %     \exp \left( - \frac{k \eps}{n} + l \log (1 + \eps) \right) 
    %     \leq \exp \left( - \frac{k \eps}{n} + \left( \frac{k}{n} + b_{\ell} \eps \; \sqrt{\frac{k}{n}} \right) \; \eps  \right)
    %     \leq \exp\left(b_{\ell} \eps \right)
    % \end{align*}  
    % where we use $k \leq \frac{n}{\eps^2}$ in the second inequality. 
    % Similarly, we can upper bound the second exponential term by
    % \begin{align*}
    %     \exp \left(  \frac{k \eps}{n} + l \log (1 - \eps) \right) 
    %     \leq \exp \left(  \frac{k \eps}{n} - \left( \frac{k}{n} + b_{\ell} \; \eps \; \sqrt{\frac{k}{n}} \right) \; \eps  \right)
    %     = \exp \lp( - b_{\ell} \; \sqrt{\frac{k}{n}}\; \eps^2  \rp)  < 1.
    % \end{align*}
    % Besides, the absolute values of the linear terms can be upper bounded by
    % \begin{align*}
    % \abs{\frac{\ell}{1 \pm \eps} - \frac{k}{n}}
    % = \abs{ \ell ( 1 \pm O(\eps) ) - \frac{k}{n} }
    % \leq \lp(1 + O(\eps)\rp) \; b_{\ell} \; \eps \; \sqrt{ \frac{k}{n} }.
    % \end{align*}
    % Overall, we can then upper bound the derivative by,
    % \begin{equation*}
    %     |f_l'(\eps)| \leq \exp( b_{\ell} ) \; \lp(1 + O(\eps)\rp) \; b_{\ell} \; \eps \; \sqrt{ \frac{k}{n} }.
    % \end{equation*}
    % Combining this with \Cref{eq:sublin-prob-diff} we obtain,
    % \begin{align*}
    %     |\Pr(a = l \mid X = 1) - \Pr(a = l \mid X = 0)| &= \frac{1}{2} \exp \left( - \frac{k}{n} \right) \frac{\left( \frac{k}{n} \right)^l}{l!} \left( f_{l}(\eps_1) - f_{l}(\eps_0) \right) \\
    %     &\leq 
    %     \frac{1}{2} \;
    %     \exp\left(- \frac{k}{n}\right) \frac{(k/n)^{l}}{l!} \exp( b_{\ell} ) \; \lp(1 + O(\eps)\rp) \; b_{\ell} \;\sqrt{ \frac{k}{n} } \;  \delta.
    % \end{align*}
    % We now proceed to lower bound the denominator $\Pr(a = l)$. 
    % As in \Cref{lemma:sublin-info-bound}, we begin by lower bounding $f_l(\eps)$.
    % \begin{align*}
    %     f_l(\eps) &= \exp \left( - \frac{k \eps}{n} + l \log (1 + \eps) \right) + \exp \left( \frac{k \eps}{n} + l \log (1 - \eps) \right) \\
    %     &\geq \exp \left( - \eps + \frac{l \eps}{3} \right) +  \exp \left( \frac{k \eps}{n} - l \eps \right) \\
    %     &\geq \exp \left( \eps \left( \frac{l}{3} - 1 \right) \right) \\
    %     &\geq e^{- \eps}  \, ,
    % \end{align*}
    % where in the first inequality we use $\frac{k}{n} \geq 1$ $\log(1 + x) \geq \frac{x}{3}$ and $\log(1 - x) \geq - x$ for $x \in [0, 1/2]$.
    % Recall the identity
    % $$
    %     \Pr(a = l)
    %     = \frac{1}{2} \exp \left( - \frac{k}{n} \right) \frac{\left( \frac{k}{n} \right)^l}{l!} (f_l(\eps_0) + f_l(\eps_1)).
    % $$
    % Hence, it follows that
    % $$
    % \Pr(a = l) 
    % \geq 
    % \exp(-\eps) \; 
    % \exp \left( - \frac{k}{n} \right) \frac{\left( \frac{k}{n} \right)^l}{l!}.
    % $$
    % Therefore, we can upper bound the summand for $\ell \in R_{b}$ by
    % \begin{align*}
    % \frac{ \lp(\Pr(a = \ell \mid X = 1) - \Pr(a = \ell \mid X = 0) \rp)^2}{ \Pr(a = \ell) }        
    % &\leq \exp\lp( - \frac{k}{n} \rp) \; \frac{ (k/n)^{\ell} }{ \ell! } \; \exp(2b_{\ell}) \; b_{\ell} \; \sqrt{ \frac{k}{n} } \; \delta \\
    % &= \exp \lp( 
    % - \frac{k}{n} + \ell \; \log( k/n ) + 2 b_{\ell}
    % + \log(b_{\ell})
    % \rp) \; \frac{1}{ \ell ! }
    % \; \sqrt{ \frac{k}/n } \; \delta.
    % \end{align*}
\end{proof}

\begin{proof}
    We note that for a Poisson random variable $a$ with mean $\lambda \geq 1$, we have $|a - \lambda| > \sqrt{\lambda} \log n$ with probability at most $o(1/n)$.
    
    In the following assume, $l \in [\lambda - \sqrt{\lambda} \log n, \lambda + \sqrt{\lambda} \log n]$.

    Fix some $\ell$ in this range.
    % Suppose $(b - 1) \sqrt{k/n} \leq \left| l - k/n \right| \leq b \sqrt{k/n}$.
    Recall from the previous section that we had
    \begin{equation*}
        % \label{eq:sublin-prob-diff}
        \Pr(a = l \mid X = 1) - \Pr(a = l \mid X = 0) = \frac{1}{2} \exp \left( - \frac{k}{n} \right) \frac{\left( \frac{k}{n} \right)^l}{l!} \left( f_{l}(\eps_1) - f_{l}(\eps_0) \right) 
    \end{equation*}
    where for a fixed $l$, we define the function $f_l$,
    \begin{equation*}
        f_l(\eps) := \exp \left( - \frac{k \eps}{n} \right) (1 + \eps)^l + \exp \left( \frac{k \eps}{n} \right) (1 - \eps)^l
    \end{equation*}    
    We will first replace the exponential function in $f_{\ell}(\eps)$ with its Taylor expansion. We then have
    \begin{align} \label{eq:exp-expansion}
    f_{\ell}(\eps) 
    = 2 + \ell \log(1 - \eps^2)
    + \sum_{i=2}^{\infty} \frac{ \lp( \frac{ k}{ n} \; \eps + \ell \; \log(1 - \eps) \rp)^i }{i!}       
    + \sum_{i=2}^{\infty} \frac{ \lp( \frac{- k}{ n} \; \eps + \ell \; \log(1 + \eps) \rp)^i }{i!}.
    \end{align}
    Our goal is to upper bound $\abs{ f_{\ell}(\eps_0) - f_{\ell}(\eps_1) }$.
    It is easy to see that the constant term $2$ will be cancelled when computing the difference. Hence, it remains to analyze the three remaining terms.
    For the term $\ell \log(1 - \eps^2)$, we have
    \begin{align*}
    \abs{\ell \log(1-\eps_0^2)        
    - \ell \log(1 - \eps_1^2)}
    &= 
    \abs{ \ell \log \lp( \frac{1 - \eps_0^2}{1 - \eps_1^2} \rp) }
    \leq \ell \; \abs{ 1 - \frac{1 - \eps_0^2}{1 - \eps_1^2} } \\
    &= \frac{\ell}{ 1-  \eps_1^2 } \lp( \eps_0 + \eps_1 \rp) \abs{\eps_0 - \eps_1}
    \leq O( \ell \eps \delta )
    \leq O \lp(  \frac{k}{n} \; \log n \; \eps \; \delta \rp) \, ,
    \end{align*}
    where in the first inequality we use the fact $\abs{\log(x)} \leq \abs{1 - x}$ for $x \geq 1$, in the second inequality we use our assumption that
    $\max(\eps_0, \eps_1) \leq \eps$ and $\abs{\eps_0 - \eps_1} \leq \delta$, and in the last inequality we use our assumption that $\abs{ \ell - k/n } < \log n \sqrt{k/n}$ and  $k < n / ( \log^2 n \; \eps )$.
    % $$
    % \abs{\ell \log(1 - \eps^2)}
    % \leq O( \ell \eps^2 )
    % \leq O \lp( \frac{k}{n} \eps^2 + \sqrt{ \frac{k}{n} } \log n \; \eps^2 \rp)
    % = O \lp(  \frac{k}{n} \; \log n \; \eps \rp) \, ,
    % $$
    % where 
    % in the first inequality we use the Taylor Expansion of $\log(1-\eps)$,
    % in the second inequality we use our assumption that $\abs{ \ell - k/n } < \log n \sqrt{k/n}$,
    % and in the third inequality we use $k < n / ( \log^2 n \; \eps )$.

    To analyze the second term in \Cref{eq:exp-expansion}, we define the function
    $$
    g_{\ell}(\eps) := \sum_{i=2}^{\infty} \frac{ \lp( \frac{ k}{ n} \; \eps + \ell \; \log(1 - \eps) \rp)^i }{i!}.
    $$
    Then we compute its derivative with respect to $\eps$. In particular, we have
    \begin{align}
    \label{eq:g-derivative}
    g_{\ell}'(\eps) 
    = \sum_{i=2}^{\infty} \frac{ 
    \lp( \frac{k}{n} - \frac{\ell}{1 - \eps} \rp) \; 
    \lp( \frac{ k}{ n} \; \eps + \ell \; \log(1 - \eps) \rp)^{i-1} }{(i-1)!}.
    \end{align}
    The absolute value of the first factor in the denominator can be upper bounded by
    $$
    \abs{ \frac{k}{n} - \frac{\ell}{1 - \eps} }
    \leq
    \abs{ \frac{k}{n} - \ell + O( \eps \ell ) }
    \leq 
    O \lp( \sqrt{ \frac{k}{n} } \log n\rp) \, ,
    $$
    where 
    in the first inequality we approximate $\frac{1}{1 - \eps}$ by $(1 + O(\eps))$ when $\eps$ is sufficiently small,
    in the second inequality we use our assumption that $\ell = \frac{k}{n} \pm O( \sqrt{k/n} \; \log n )$ and that $k < n / (\log^2 n \; \eps )$.
    We then analyze the absolute value of term in the denominator that is raised to its $(i-1)$-th power. We can upper bound it by
    \begin{align*}
    \abs{ \frac{k \eps}{n} + \ell \; \log(1 - \eps) }
    &\leq \abs{ \frac{k \eps}{n} - \ell \eps  } + O( \ell \eps^2 )
    \leq O \lp(  \sqrt{ \frac{k}{n} } \; \log n \; \eps \rp) + O( \frac{k}{n} \eps^2  +  \sqrt{\frac{k}{n}} \; \log n \; \eps^2 )         \\
    &\leq O\lp( \sqrt{ \frac{k}{n} } \; \log n \; \eps \rp) \, ,
    \end{align*}
    where in the first inequality we use the Taylor approximation of $\log(1 - \eps) = - \eps + O(\eps^2)$, in the second inequality we use our assumption that $\abs{ \ell - k/n } < \log n \sqrt{k/n}$, and in the last inequality we use $k < n/( \log^2 n \; \eps )$.
    Notice that $\sqrt{k/n} \; \log n \; \eps < 1/2$ by our assumption $k < n/( \log^2 n \; \eps )$.
    Hence, we conclude that the dominating term in the summation in \Cref{eq:g-derivative} is the one with $i = 2$.
    Therefore, we can upper bound $\abs{g_{\ell}'(\eps)}$ by
    $$
    \abs{g_{\ell}'(\eps)}
    \leq O(1) \; \sqrt{ \frac{k}{n} } \log n \; \sqrt{ \frac{k}{n} } \; \log n \; \eps
    = O\lp(  \; \frac{k}{n} \; \log^2 n \; \eps \rp).
    $$
    It then follows that
    $$
    \abs{ g_{\ell}(\eps_0) - g_{\ell}(\eps_1) }
    \leq O\lp(  \; \frac{k}{n} \; \log^2 n \; \eps \; \delta \rp) \, ,
    $$
    since $\max(\eps_0, \eps_1) < \eps$ and $\abs{\eps_0 - \eps_1} < \delta$.
    Now, for the last term in \Cref{eq:exp-expansion}, we can similarly define
$$
    g^{-}_{\ell}(\eps) := \sum_{i=2}^{\infty} \frac{ \lp( \frac{ k}{ n} \; \eps + \ell \; \log(1 - \eps) \rp)^i }{i!}.
$$
Using an argument almost identical to that of $g_{\ell}(\eps)$, we can similarly show
$$
    \abs{ g_{\ell}^{-}(\eps_0) - g_{\ell}^{-}(\eps_1) }
    \leq O\lp(  \; \frac{k}{n} \; \log^2 n \; \eps \; \delta \rp).
$$
Combining our analysis for the four terms in \Cref{eq:exp-expansion}, we therefore conclude
$$
\abs{f_{ \ell }( \eps_0 ) - f_{\ell}(  \eps_1 )}
\leq O\lp(  \; \frac{k}{n} \; \log^2 n \; \eps \; \delta \rp)
$$
for all $\ell > 0$ such that $\abs{ \ell - k/n } \leq \sqrt{k/n \; \log n \; \eps}$.
    Combining this with \Cref{eq:sublin-prob-diff} we obtain,
    \begin{align*}
        \abs{\Pr(a = l \mid X = 1) - \Pr(a = l \mid X = 0)} &= \frac{1}{2} \exp \left( - \frac{k}{n} \right) \frac{\left( \frac{k}{n} \right)^l}{l!} \abs{f_{l}(\eps_1) - f_{l}(\eps_0)} \\
        &\leq 
        O(1) \; 
        \exp\left(- \frac{k}{n}\right) \frac{(k/n)^{l}}{l!} \; 
        \frac{k}{n} \; \log^2 n \; \eps \; \delta.
    \end{align*}
    We now proceed to lower bound the denominator $\Pr(a = l)$. 
    As in \Cref{lemma:sublin-info-bound}, we begin by lower bounding $f_l(\eps)$.
    \begin{align*}
        f_l(\eps) &= \exp \left( - \frac{k \eps}{n} + l \log (1 + \eps) \right) + \exp \left( \frac{k \eps}{n} + l \log (1 - \eps) \right) \\
        &\geq \exp \left( - \eps + \frac{l \eps}{3} \right) +  \exp \left( \frac{k \eps}{n} - l \eps \right) \\
        &\geq \exp \left( \eps \left( \frac{l}{3} - 1 \right) \right) \\
        &\geq e^{- \eps}  \, ,
    \end{align*}
    where in the first inequality we use $\frac{k}{n} \geq 1$ $\log(1 + x) \geq \frac{x}{3}$ and $\log(1 - x) \geq - x$ for $x \in [0, 1/2]$.
    Recall the identity
    $$
        \Pr(a = l)
        = \frac{1}{2} \exp \left( - \frac{k}{n} \right) \frac{\left( \frac{k}{n} \right)^l}{l!} (f_l(\eps_0) + f_l(\eps_1)).
    $$
    Hence, it follows that
    $$
    \Pr(a = l) 
    \geq 
    \exp(-\eps) \; 
    \exp \left( - \frac{k}{n} \right) \frac{\left( \frac{k}{n} \right)^l}{l!}.
    $$
    Therefore, we can upper bound the summand for $\ell \geq 0$ satisfying
    $\abs{ \ell - k/n } \leq \sqrt{k/n \; \log n \; \eps}$ by
    \begin{align*}
    \frac{ \lp(\Pr(a = \ell \mid X = 1) - \Pr(a = \ell \mid X = 0) \rp)^2}{ \Pr(a = \ell) }        
    &\leq O(1) \; \exp\lp( - \frac{k}{n} \rp) \; \frac{ (k/n)^{\ell} }{ \ell! } \; 
    \frac{k^2}{n^2} \; \log^4 n \; \eps^2 \; \delta^2.
    \end{align*}
    Now, we sum over all $\ell \geq 0$. This gives us
    \begin{align*}
        &\sum_{l = 0}^{\infty} \frac{(\Pr(a = l \mid X = 0) - \Pr(a = l \mid X = 1))^2}{\Pr(a = l)}  \\
        &\leq 
        o(1/n)
        + 
        O(1) \; 
        \sum_{l = \max\lp(0, \frac{k}{n} - \sqrt{k}{n} \; \log n\rp)}^{ \frac{k}{n} + \sqrt{k}{n} \; \log n }
        \exp\lp( - \frac{k}{n} \rp) \; \frac{ (k/n)^{\ell} }{ \ell! } \; 
        \frac{k^2}{n^2} \; \log^4 n \; \eps^2 \; \delta^2 \\
        &\leq o(1/ n) + O \lp(  \frac{k^2}{n^2} \; \log^4 n \; \eps^2 \; \delta^2 \rp) \, ,        
    \end{align*}
where in the first inequality we use the fact that $|a - \lambda| > \sqrt{\lambda} \log n$ with probability at most $o(1/n)$ for $a \sim \PoiD{k/n}$,
and in the  last inequality we use the fact that $ \sum_{\ell} \exp\lp( - \frac{k}{n} \rp) \; \frac{ (k/n)^{\ell} }{ \ell! }$ must be less than one since its summand is exactly the probability mass function of Poisson distribution with mean $k/n$ evaluated at the point $\ell$.    
    % Taking the derivative with respect to $\eps$ gives
    % \begin{align*}
    %     f_l'(\eps) &= \left( \frac{l}{1 + \eps} - \frac{k}{n} \right) \exp \left( - \frac{k \eps}{n} + l \log (1 + \eps) \right) + \left( \frac{k}{n} - \frac{l}{1 - \eps} \right) \exp \left( \frac{k \eps}{n} + l \log (1 - \eps) \right).
    % \end{align*}
    % To present our bound cleanly, we define the quantity 
    % $$
    % b_{\ell} := \abs{\ell - \frac{k}{n}} / \lp( \eps \sqrt{k/n} \rp).
    % $$
    % Using the inequality $\log(x) \leq x - 1$
    % and the bound on $\ell$, we can upper bound the first exponential term by
    % \begin{align*}
    %     \exp \left( - \frac{k \eps}{n} + l \log (1 + \eps) \right) 
    %     \leq \exp \left( - \frac{k \eps}{n} + \left( \frac{k}{n} + b_{\ell} \eps \; \sqrt{\frac{k}{n}} \right) \; \eps  \right)
    %     \leq \exp\left(b_{\ell} \eps \right)
    % \end{align*}  
    % where we use $k \leq \frac{n}{\eps^2}$ in the second inequality. 
    % Similarly, we can upper bound the second exponential term by
    % \begin{align*}
    %     \exp \left(  \frac{k \eps}{n} + l \log (1 - \eps) \right) 
    %     \leq \exp \left(  \frac{k \eps}{n} - \left( \frac{k}{n} + b_{\ell} \; \eps \; \sqrt{\frac{k}{n}} \right) \; \eps  \right)
    %     = \exp \lp( - b_{\ell} \; \sqrt{\frac{k}{n}}\; \eps^2  \rp)  < 1.
    % \end{align*}
    % Besides, the absolute values of the linear terms can be upper bounded by
    % \begin{align*}
    % \abs{\frac{\ell}{1 \pm \eps} - \frac{k}{n}}
    % = \abs{ \ell ( 1 \pm O(\eps) ) - \frac{k}{n} }
    % \leq \lp(1 + O(\eps)\rp) \; b_{\ell} \; \eps \; \sqrt{ \frac{k}{n} }.
    % \end{align*}
    % Overall, we can then upper bound the derivative by,
    % \begin{equation*}
    %     |f_l'(\eps)| \leq \exp( b_{\ell} ) \; \lp(1 + O(\eps)\rp) \; b_{\ell} \; \eps \; \sqrt{ \frac{k}{n} }.
    % \end{equation*}
    % Combining this with \Cref{eq:sublin-prob-diff} we obtain,
    % \begin{align*}
    %     |\Pr(a = l \mid X = 1) - \Pr(a = l \mid X = 0)| &= \frac{1}{2} \exp \left( - \frac{k}{n} \right) \frac{\left( \frac{k}{n} \right)^l}{l!} \left( f_{l}(\eps_1) - f_{l}(\eps_0) \right) \\
    %     &\leq 
    %     \frac{1}{2} \;
    %     \exp\left(- \frac{k}{n}\right) \frac{(k/n)^{l}}{l!} \exp( b_{\ell} ) \; \lp(1 + O(\eps)\rp) \; b_{\ell} \;\sqrt{ \frac{k}{n} } \;  \delta.
    % \end{align*}
    % We now proceed to lower bound the denominator $\Pr(a = l)$. 
    % As in \Cref{lemma:sublin-info-bound}, we begin by lower bounding $f_l(\eps)$.
    % \begin{align*}
    %     f_l(\eps) &= \exp \left( - \frac{k \eps}{n} + l \log (1 + \eps) \right) + \exp \left( \frac{k \eps}{n} + l \log (1 - \eps) \right) \\
    %     &\geq \exp \left( - \eps + \frac{l \eps}{3} \right) +  \exp \left( \frac{k \eps}{n} - l \eps \right) \\
    %     &\geq \exp \left( \eps \left( \frac{l}{3} - 1 \right) \right) \\
    %     &\geq e^{- \eps}  \, ,
    % \end{align*}
    % where in the first inequality we use $\frac{k}{n} \geq 1$ $\log(1 + x) \geq \frac{x}{3}$ and $\log(1 - x) \geq - x$ for $x \in [0, 1/2]$.
    % Recall the identity
    % $$
    %     \Pr(a = l)
    %     = \frac{1}{2} \exp \left( - \frac{k}{n} \right) \frac{\left( \frac{k}{n} \right)^l}{l!} (f_l(\eps_0) + f_l(\eps_1)).
    % $$
    % Hence, it follows that
    % $$
    % \Pr(a = l) 
    % \geq 
    % \exp(-\eps) \; 
    % \exp \left( - \frac{k}{n} \right) \frac{\left( \frac{k}{n} \right)^l}{l!}.
    % $$
    % Therefore, we can upper bound the summand for $\ell \in R_{b}$ by
    % \begin{align*}
    % \frac{ \lp(\Pr(a = \ell \mid X = 1) - \Pr(a = \ell \mid X = 0) \rp)^2}{ \Pr(a = \ell) }        
    % &\leq \exp\lp( - \frac{k}{n} \rp) \; \frac{ (k/n)^{\ell} }{ \ell! } \; \exp(2b_{\ell}) \; b_{\ell} \; \sqrt{ \frac{k}{n} } \; \delta \\
    % &= \exp \lp( 
    % - \frac{k}{n} + \ell \; \log( k/n ) + 2 b_{\ell}
    % + \log(b_{\ell})
    % \rp) \; \frac{1}{ \ell ! }
    % \; \sqrt{ \frac{k}/n } \; \delta.
    % \end{align*}
\end{proof}


We now present the mutual information bound for the last parameter regime.
\begin{lemma}
    \label{lemma:superlearn-info-bound}
    Let $\delta = |\epsa - \epsb|$ and $\eps = \max(\epsa, \epsb)$.
    Let $k >\frac{n}{ 2 \; \log^2 n \; \eps^2}$.
    Then it holds
    \begin{equation*}
    I(X \; : \; (a,b) ) \leq O \left( \frac{\eps^2 \delta^2 k^2 \; \log^2 n }{n^2} \right).
    \end{equation*}
\end{lemma}

We now present the mutual information bound for the last parameter regime.
We are going to use the following facts regarding  KL-divergence and mutual information.
\begin{claim}[Convexity of KL-divergence]
\label{clm:kl-convexity}
Let $w \in (0, 1)$, and $p_1, p_2, q_1, q_2$ be  probability distributions over the same domain.
Then it holds
$$
\KL( w p_1 + (1 - w) p_2 || w q_1 + (1-w) q_2 )
\leq
w  \KL( p_1 || q_1 )
+ (1 - w) \KL( p_2 || q_2 ).
$$
\end{claim}
\begin{claim}[Additivity of KL-divergence]
\label{clm:kl-additive}
Let $w \in (0, 1)$, and $p_1, p_2, q_1, q_2$ be  probability distributions such that $p_1, q_1$ share the same domain and $p_2, q_2$ share the same domain.
Then it holds
$$
\KL( p_1 \otimes p_2 || q_1 \otimes q_2 )
=
\KL( p_1 || q_1 ) + \KL(p_2 || q_2).
$$
\end{claim}
\begin{claim}[Mutual Informtion Identity]
\label{clm:mi-kl-relationship}
Let $X$ be an indicator variable, and $H_0, H_1$ be a pair of distributions.
Let $H$ be the random variable that follows the distribution of $H_0$ if $X = 0$ and $X_1$ if $X = 1$. Then it holds
$$
I(X:H) =  \frac{1}{2} \KL\lp( H_0 : \frac{1}{2} \lp( H_1+H_0\rp) \rp) 
+ \frac{1}{2} \KL\lp( H_1: \frac{1}{2} \lp( H_1+H_0\rp) \rp).
$$
\end{claim}
\begin{proof}[Proof of \Cref{lemma:superlearn-info-bound}]
When $X = 0$, the pair $(a,b)$ is distributed as a even mixture of two distributions that are both product of Poisson distributions: $$
(a,b) \mid (X = 0) \sim
H_0 := 
\frac{1}{2} \lp( 
\PoiD{ \frac{k}{n}+ \eps_0 \; \frac{k}{n} } \otimes
\PoiD{ \frac{k}{n} - \eps_0 \; \frac{k}{n} }
+ 
\PoiD{ \frac{k}{n} - \eps_0 \; \frac{k}{n} }
\otimes 
\PoiD{ \frac{k}{n} + \eps_0 \; \frac{k}{n} } \rp).
$$
Similarly, we have
$$
(a,b) \mid (X = 0) \sim
H_1 := 
\frac{1}{2} \lp( 
\PoiD{ \frac{k}{n}+ \eps_1 \; \frac{k}{n} } \otimes
\PoiD{ \frac{k}{n} - \eps_1 \; \frac{k}{n} }
+ 
\PoiD{ \frac{k}{n} - \eps_1 \; \frac{k}{n} }
\otimes 
\PoiD{ \frac{k}{n} + \eps_1 \; \frac{k}{n} } \rp).
$$
From \Cref{clm:mi-kl-relationship} and \Cref{clm:kl-convexity}, 
we know that it suffices to show that the KL-divergences between $H_0$ and $H_1$ are at most
$ \slearnbound $. We focus on the argument for 
$\KL(H_0 : H_1)$ as the one for $\KL(H_1 : H_0)$ is symmetric.

By the definition of $H_0$ and $H_1$, we have that
\begin{align*}
\KL(H_0:H_1)    
&\leq \frac{1}{2}
\KL \lp(  
\PoiD{ \frac{k}{n}+ \eps_0 \; \frac{k}{n} } \otimes
\PoiD{ \frac{k}{n} - \eps_0 \; \frac{k}{n} }
||
\PoiD{ \frac{k}{n}+ \eps_1 \; \frac{k}{n} } \otimes
\PoiD{ \frac{k}{n} - \eps_1 \; \frac{k}{n} }
\rp) \\
&+ 
\frac{1}{2}
\KL \lp(  
\PoiD{ \frac{k}{n}- \eps_0 \; \frac{k}{n} } \otimes
\PoiD{ \frac{k}{n} + \eps_0 \; \frac{k}{n} }
||
\PoiD{ \frac{k}{n}-\eps_1 \; \frac{k}{n} } \otimes
\PoiD{ \frac{k}{n}+\eps_1 \; \frac{k}{n} }.
\rp) \\
&=
\KL \lp(  
\PoiD{ \frac{k}{n}+ \eps_0 \; \frac{k}{n} }
||
\PoiD{ \frac{k}{n}+ \eps_1 \; \frac{k}{n} }
\rp)
+ 
\KL \lp(  
\PoiD{ \frac{k}{n}- \eps_0 \; \frac{k}{n} }
||
\PoiD{ \frac{k}{n}- \eps_1 \; \frac{k}{n} }
\rp) \, ,
\end{align*}
where in the first line we use \Cref{clm:kl-convexity}, and in the last line we use \Cref{clm:kl-additive}.

Let $\lambda_1 > \lambda_2 > 0$.
Note that we have the following closed form for KL divergence between a pair of Poisson distributions:
$$
\text{KL}( \PoiD{\lambda_1 } || \PoiD{\lambda_2}  )
= \lambda_1 \log( \lambda_1 / \lambda_2 ) + \lambda_2 - \lambda_1
\leq \lambda_1 \frac{ \lambda_1 - \lambda_2 }{ \lambda_2 } + \lambda_2 - \lambda_1
= \frac{ (\lambda_1 - \lambda_2)^2 }{ \lambda_2 } \, ,
$$
where in the first inequality we use the bound $\log(x) \leq x - 1$ for all $x > 0$.
Hence, it follows that
$$
\text{KL}( H_0 || H_1  )
\leq \frac{\lp( \frac{k}{n} \lp( \eps_1 - \eps_0 \rp) \rp)^2}{ \frac{k}{n} (1 + \eps_1) }
\leq O(1) \; \frac{k}{n} \delta^2.
$$
But notice that this is at most
$ O \lp( \slearnbound \rp) $ as long as 
$ k \geq n / ( 2 \log^2 n \eps^2 ) $ which is our assumed parameter regime in this lemma.
\end{proof}


